Causal Support: Modeling Causal Inferences with Visualizations

Analysts often make visual causal inferences about possible data-generating models. However, visual analytics (VA) software tends to leave these models implicit in the mind of the analyst, which casts doubt on the statistical validity of informal visual "insights". We formally evaluate the quality of causal inferences from visualizations by adopting causal support -- a Bayesian cognition model that learns the probability of alternative causal explanations given some data -- as a normative benchmark for causal inferences. We contribute two experiments assessing how well crowdworkers can detect (1) a treatment effect and (2) a confounding relationship. We find that chart users' causal inferences tend to be insensitive to sample size such that they deviate from our normative benchmark. While interactively cross-filtering data in visualizations can improve sensitivity, on average users do not perform reliably better with common visualizations than they do with textual contingency tables. These experiments demonstrate the utility of causal support as an evaluation framework for inferences in VA and point to opportunities to make analysts' mental models more explicit in VA software.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> archived/drafts/background-draft1.tex <==
\section{Background}
\subsection{Visual Representations of Uncertainty}
In communicating the results of statistical analysis, visualization authors commonly represent uncertainty as a range of possible values as has been recommended by numerous experts (e.g., Cumming 2014, Manski 2018). 
However, there is a growing body of work suggesting that lay and expert audiences commonly misinterpret such interval representations of uncertainty (Belia 2005, Soyer 2012, Hoekstra 2014) and that other uncertainty visualization formats such as gradient plots (Correll 2014), violin plots (Correll 2014, Hullman 2015), hypothetical outcome plots (Hullman 2015, Kale 2019), and quantile dotplots (Fernandes 2019) \matt{cite the first bus paper here too (Kay 2016)} lead to more accurate interpretation and performance on various tasks. 
Additional conventional uncertainty representations which are commonly used in statistical workflows include aggregate encodings of distributions such as boxplots, histograms, and densities. \alex{Cites for these static aggregate distributions?} \jessica{There are cites for some of these - maybe Tukey on boxplots, violin plots I think are in a paper called raindrop plots, maybe bean plots, not sure about histogram but worth a look for an early paper} \matt{earliest ref for violins for uncertainty I know of is Spiegelhalter's ``surgical audit'' paper on ``eyeball plots'' (http://www.jstor.org/stable/2680466)}

Importantly, a recent survey of visualization practitioners shows that the most common way of handling uncertainty in visualization authoring is to omit it entirely, opting instead to show only point estimates (Hullman 2020). 
This may be misleading insofar as emphasizing the mean can lead the audience of a visualization to believe that inferences from statistical models are precise with a greater degree of credibility than is warranted (Manski 2018). 
From the perspective of decision theory (von Neumann 1947), omitting uncertainty information from visualizations should lead to suboptimal decision-making since users might be less likely to reason about the space of possible outcomes when considering the utility of alternative courses of action. 

A growing body of work suggests that framing uncertainty as frequencies of events helps people reason in ways that resemble Bayesian update (Gigerenzer 1995, Hoffrage 1998, Micallef 2012, Kim 2019) and improves statistical reasoning more broadly (Chance 2000, Hogarth 2011, Galesic 2009 (study on icon arrays cited in Spiegelhalter review), Hullman 2015, Kay 2016, Kale 2019, Fernades 2019). 
A handful of noteworthy visualization techniques have been developed in this vein. 
For example, icon arrays \alex{original cite?} show proportions, probabilities, and ratios as numbers of discrete graphic objects, often with different colors denoting different groups or different possible outcomes. 
However, traditional icon arrays do not actually convey that the frequencies shown are uncertain. 
Another technique called hypothetical outcome plots (HOPs) (Hullman 2015) can be used to encode uncertainty in icon arrays or other visualized prediction by showing different possible outcomes across frames of an animation. \matt{this point about being able to show two levels of uncertainty simultaneously seems out of place in this paper, especially since we don't study or use it here?}
Because HOPs encode uncertainty over time, turning existing designs into HOPs adds uncertainty information while leaving other spatial encodings unaltered. 
A third technique, quantile dotplots (Kay 2016), shows uncertainty by quantizing a distribution of possible outcomes and representing each quantile as a discrete dot.
More generally, authors may create frequency-based visualziations by displaying a sample of model predictions (e.g., drawn from the posterior distribution of a Bayesian model) in lieu of or in addition to aggregate representations of uncertainty (e.g., confidence intervals).  

In this study, we compare the performance of two frequency-based visualizations, quantile dotplots and HOPs, with two more conventional uncertainty representations, intervals and densities. To our knowledge this is the first direct comparison of HOPs and quantile dotplots in a graphical perception study.

\subsection{Judgments Under Uncertainty}
It is important to distinguish between two types of judgments we investigate in this study: magnitude estimation and decision-making. 
Judgments refer to a broad class of behavioral responses that have been studied in terms of bottom-up processes of perception (e.g., Cleveland and McGill 1984) and top-down processes of heuristics and cognition (e.g., Tversky and Kahneman 1974). 
For instance, in a magnitude estimation task, a user’s performance is a function of both what their visual system enables them to see in a chart and how they subsequently process that information in order to produce a response. 
In contrast, decision-making has conventionally been studied in terms of incentivized choices between alternative courses of action (von Neumann 1947). Thus, decision-making research aims to characterize how well people evaluate alternatives relative to their expected utility in terms of risk preferences under different circumstances (Tversky and Kahneman 1979).

\begin{figure}[ht]
    \centering
    \includegraphics[width=\columnwidth]{figures/llo_explainer-01.png}
    \caption{Linear in log odds (LLO) model with fits in logit (left) and probability units (right). Top: Average response as a function of ground truth for each visualization condition in color vs a range of slopes in gray. Bottom: Predicted fit and raw data from one user.}
    \label{fig:llo_explainer}
\end{figure}

In this study, we base our statistical model of effect size magnitude estimation on a theory of the perception of relative frequencies which posits that the brain represents probabilities on a log odds scale (Zhang 2014). 
In this \textit{linear in log odds (LLO) model} (Fig.~\ref{fig:llo_explainer}),
\matt{I think it's linear \textbf{in} log odds? term introduced in this paper, which should also be cited here: http://www-personal.umich.edu/~gonzo/papers/shapewf.pdf} 
biases in probability judgments are represented by the slope of the linear model, such that slopes less than one reflect a bias toward estimating 50\% probability \matt{depends on where the intercept is though? Honestly this is easier to understand with a viz anyway...}. 
In our study, we frame effect size as a probability judgment by asking users to estimate how many times out of 100 an intervention would produce a better outcome than no intervention, a measure of effect size called \textit{probability of superiority}. 
On this response scale, estimating 50\% corresponds to estimating that there is no effect or no mean difference between predicted outcomes with and without intervention. 
Thus, when the LLO model is applied to estimates of probability of superiority, slopes less than one correspond to a pattern of underestimating effect size.

The pattern of underestimating effect size described by the LLO model is similar and potentially related to an important pattern in decision-making. Prospect theory (Kahneman and Tversky 1979) describes how people incorporate probability information into incentivized decisions such that events with low probabilities are treated as more likely than they are, and events with high probabilities are treated as less likely than they are. 
% \jessica{can we say more about how these things are different? since they seem essentially the same from the description}
Kahneman and Tversky (1979) distinguish between \textit{estimating} the likelihood of of an event $p$ versus \textit{weighting} the probability of an event $\pi(p)$ \matt{not sure I understand the difference. Is $p$ a probability or an event? If an event, don't use $p$, if a probability, is $\pi(p)$ a probability of a probability? See other comments on notation below.} \alex{$p$ is the probability of an event; $\pi(p)$ is the weight assigned to that probability for the purpose of decision-making. I'm borrowing this notation from K \& T, but I agree that we should be internally consistent (FYI, we use $p$ later in the logistic regression specification). I find this whole notion of weighting a little arcane, especially since K \& T sort of punt on it and assume that $\pi(p) = p$ in their analysis. Our results suggest that perceived probability and how probability informs decisions are not the same thing, so it seems important to mention here. I think we should discuss framing around this idea.} \matt{ah hrm, so is a reasonable interpretation something like $p$ is a probability and $\pi(p)$ is a perceived probability? I have seen that framing + notation before (in the cyclical power model). So yeah I'm fine with this notation but I think it needs a clearer explanation.}, suggesting that the later reflects a preference based on the former.
However, recent work in behavioral economics (Khaw 2017) challenges this assertion by attributing biases in decision preferences---often referred to as risk seeking and risk aversion---to perceptual biases in probability estimation.
We investigate whether the patterns of bias in effect size estimates predicted by the LLO model are coupled with the quality of decisions made by the same chart user looking at the same information. \matt{might be worth mentioning the cyclical power model paper somewhere in this para too, since it connects this stuff back to stevens' power law which will be familiar to some in the vis community}

% Regardless of the theoretical relationship between magnitude estimations and decisions, it is important for visualization designers to know how to choose visualization formats that support the intended task of their users. 
% There is practical value in knowing whether the visualization formats which support the most accurate perception of effect size are the same ones that promote the most utility-optimal decisions. \matt{not sure this para does much, could be cut}

==> archived/drafts/background-draft2.tex <==
\section{Background}
\subsection{Visual Representations of Uncertainty}
In communicating the results of statistical analysis, visualization authors commonly represent uncertainty as a range of possible values as has been recommended by numerous experts (e.g.,~\cite{Cumming2014,Manski2018b}). 
However, there is a growing body of work suggesting that lay and expert audiences commonly misinterpret interval representations of uncertainty~\cite{Belia2005,Soyer2012,Hoekstra2014} and that other uncertainty visualization formats such as gradient plots~\cite{Correll2014}, violin plots~\cite{Correll2014,Hullman2015}, hypothetical outcome plots (HOPs)~\cite{Hullman2015,Kale2019-hops}, and quantile dotplots~\cite{Kay2016,Fernandes2018} lead to more accurate interpretation and performance on various tasks. 
Two of these formats show uncertainty as frequencies of events, building on a large body of work suggesting that such frequency framing improves statistical reasoning~\cite{Chance2000,Galesic2009,Gigerenzer1995,Hoffrage1998,Hogarth2011,Hullman2015,Kay2016,Kale2019-hops,Kim2019,Micallef2012,Fernandes2018}:
HOPs~\cite{Hullman2015} encode uncertainty by showing possible outcomes as frames in animation.
Quantile dotplots~\cite{Kay2016} show uncertainty by quantizing a distribution of possible outcomes and representing each quantile as a discrete dot. 
Other conventional uncertainty representations which are commonly used in statistical workflows include aggregate encodings of distributions such as boxplots~\cite{Tukey1977}, histograms~\cite{Pearson1895}, and densities~\cite{Spiegelhalter1999,Barrowman2003}. \jessica{this feels a little out of place, maybe introduce the varieties first then say that research suggests that the more expressive and frequency formats seem better for broader audiences}
% \alex{Cites for these static aggregate distributions?} \jessica{There are cites for some of these - maybe Tukey on boxplots, violin plots I think are in a paper called raindrop plots, maybe bean plots, not sure about histogram but worth a look for an early paper} \matt{earliest ref for violins for uncertainty I know of is Spiegelhalter's ``surgical audit'' paper on ``eyeball plots'' (http://www.jstor.org/stable/2680466)}

% Importantly, a recent survey of visualization practitioners shows that the most common way of handling uncertainty in visualization authoring is to omit it entirely, opting instead to show only point estimates (Hullman 2020). 
% This may be misleading insofar as emphasizing the mean can lead the audience of a visualization to believe that inferences from statistical models are precise with a greater degree of credibility than is warranted (Manski 2018). 
% From the perspective of decision theory (von Neumann 1947), omitting uncertainty information from visualizations should lead to suboptimal decision-making since users might be less likely to reason about the space of possible outcomes when considering the utility of alternative courses of action. 

% A growing body of work suggests that framing uncertainty as frequencies of events helps people reason in ways that resemble Bayesian update~\cite{Gigerenzer1995,Hoffrage1998,Micallef2012,Kim2019} and improves statistical reasoning more broadly~\cite{Chance2000,Galesic2009,Hogarth2011,Hullman2015,Kay2016,Kale2019-hops,Fernandes2018}. 
% A handful of noteworthy visualization techniques have been developed in this vein. 
% For example, icon arrays \alex{original cite?} show proportions, probabilities, and ratios as numbers of discrete graphic objects, often with different colors denoting different groups or different possible outcomes. 
% However, icon arrays do not actually convey that the frequency shown is itself an uncertain estimate.
% Another technique called hypothetical outcome plots (HOPs)~\cite{Hullman2015} can be used to encode uncertainty in icon arrays or any other static visualization by animating between possible estimates. 
% \matt{this point about being able to show two levels of uncertainty simultaneously seems out of place in this paper, especially since we don't study or use it here?} 
% Because HOPs encode uncertainty over time, turning existing designs into HOPs adds uncertainty information while leaving other spatial encodings unaltered. 
% A third technique, quantile dotplots~\cite{Kay2016}, shows uncertainty by quantizing a distribution of possible outcomes and representing each quantile as a discrete dot.
% More generally, authors may create frequency-based visualziations by displaying a sample of model predictions (e.g., drawn from the posterior distribution of a Bayesian model) in lieu of or in addition to aggregate representations of uncertainty (e.g., confidence intervals).  

In this study, we compare the performance of two frequency-based visualizations, quantile dotplots and HOPs, with two more conventional uncertainty representations, intervals and densities. To our knowledge this is the first direct comparison of HOPs and quantile dotplots, \jessica{and by varying whether means are added to each, allows us to investigate the extent to which users of these two frequency visualizations may differ in their tendency to rely on means.} \jessica{can omit that last part for space if needed, I wanted to give a bit more context on why its an interesting comparison}

\subsection{Effect Size}
\jessica{I suspect this section could be one paragraph added to prior section, introduce effect size and describe which vis studies ahve explicitly asked for effect size judgments}
We investigate how design choices impact judgments and decisions from visualized effect size.
We focus on a measure of effect size called probability of superiority (a.k.a. Common Language Effect Size \jessica{(CLES)}~\cite{McGraw1992}), which is the percent of the time that expected outcomes for one group $A$ exceed expected outcomes for another group $B$.
Probability of superiority is a proxy for standardized mean difference $\frac{\mu_A - \mu_B}{\sigma_{A-B}}$~\cite{Coe2002,Cummings2011},
a metric for the difference between two groups relative to uncertainty \jessica{in the mean of each}.
% the mean difference in outcomes between two groups normalized by the variability of the mean difference.
Chart users have an incentive to make accurate judgments of the standardized mean difference in situations where they must choose whether to purchase an intervention or stick with the status quo (e.g.,~\cite{Joslyn2012,Joslyn2013,Hofman2020}). \jessica{could omit the last sentence, it doesnt add much to understanding}
% Effect size judgments require understanding both point estimates and the uncertainty of those estimates in relation to one another.

\subsection{Judgments Under Uncertainty}
\jessica{this may need a more specific title. Something like Biases in Judgment under Uncertainty, though that's still pretty broad. Prospective theory and LLO are in a pretty narrow subspace of judgement under uncertainty lit}
\sout{It is important to} \jessica{Our study} distinguishes between two types of judgments \sout{we investigate in this study}: magnitude estimation and decision-making. 
% Judgments refer to a broad class of behavioral responses that have been studied in terms of bottom-up processes of perception (e.g.,~\cite{Cleveland1984}) and top-down processes of cognition (e.g.,~\cite{Tversky1974}). 
In a magnitude estimation task, a user’s performance is a function of both what their visual system enables them to see in a chart and how they subsequently process that information in order to produce a response. 
In contrast, decision-making is conventionally studied in terms of incentivized choices between alternative courses of action~\cite{vonNeumann1944}, where the aim is to characterize how well people evaluate alternatives relative to their expected utility in different situations~\cite{Kahneman1979,Tversky1981}.
\jessica{not sure this belongs here, seems better in methods. Maybe this section is about probability magnitude estimation only. You may also want to introduce LLO as one example of various models that attempt to describe systematic biases in perceiving how informative data is (pg 25 of the ambuehl and li demand for info paper describes how their model is also equivalent to LLO, so coudl be cut to put it in the more general context first.}
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/llo_explainer-03.png}
    \setlength{\abovecaptionskip}{-10pt}
    \setlength{\belowcaptionskip}{-10pt}
    \caption{Linear in log odds (LLO) model with fits in logit (left) and probability units (right). Top: Responses are biased toward 50\% probability of superiority (underestimation) in all visualization conditions. Bottom: Model of magnitude estimation bias in responses from one user. \jessica{need to be clearer in caption and maybe a figure title that we are demonstrating our modeling approach (otherwise unclear who this user is, how to interpret vis condition). Kind of reads like we are talking about vis conditions we studied in caption rather than hypothetical conditions, which is slightly confusing bc its not clear why we're talking about results in related work.   The purple fits from vis condition part is confusing, it looks like one very thick purple line and one thin one}
    % \idl{I'm confused by $true_{\Pr(S)}$ as it looks like a boolean variable. What if $\Pr(S)_{truth}$ and $\Pr(S)_{response}$?} \alex{I worry about putting truth and response in the subscript, but I could see change `true' to `truth' helping with this confusion.}
    % \idl{It is hard to see the message in Fig 2. Can you add arrows and reference lines to the relevant visual features? I guess we should look at the distance between the actual line and a horizontal line at 50\%, but it took me a long time to figure this out (and I'm not confident if this is correct). Perhaps due to overplotting or the use of less saturated colors, the HOPs and Intervals lines are not really visible in Fig 2.} \alex{Another person was confused about the connection between this figure and JND / PSE (there is none). Neither of the people reviewed the paper understood what this figure is intended to convey.}
    }
    \label{fig:llo_explainer}
\end{figure}

In this study, we model effect size estimation using a \textit{linear in log odds (LLO) model} (Fig.~\ref{fig:llo_explainer}), which is based on a theory that the brain represents probabilities on a log odds scale~\cite{Gonzalez1999,Zhang2012}.
% In this study, we base our statistical model of effect size magnitude estimation on a theory of the perception of relative frequencies which posits that the brain represents probabilities on a log odds scale~\cite{Gonzalez1999,Zhang2012}. 
% In this \textit{linear in log odds (LLO) model} (Fig.~\ref{fig:llo_explainer}), 
\footnote{The linear in log odds model~\cite{Gonzalez1999,Zhang2012} is a special case of the cyclical power model~\cite{Hollands2000} with reference points at probabilities of 0\% and 100\%. This is a modification of Steven's power law~\cite{Stevens1957} to handle proportions.}
% biases in probability judgments are represented by the slope of the linear model, such that slopes less than one reflect a bias toward estimating 50\% probability.
Because we elicit effect size estimates in terms of probability of superiority, such that a response of 50\% corresponds to saying there is no effect, slopes less than one in the the LLO model represent bias toward underestimating effect size (Fig.~\ref{fig:llo_explainer}, blue arrows).
~\footnote{LLO slopes less than one represent bias toward the probability at the intercept $\mathrm{logit^{-1}}(intercept)$ which happens to be close to 50\% in our study.}
% In our study, we frame effect size as a probability judgment by asking users to estimate how many times out of 100 an intervention would produce a better outcome than no intervention (i.e., probability of superiority~\cite{McGraw1992}). 
% On this response scale, estimating 50\% corresponds to saying there is no mean difference between predicted outcomes with and without intervention, so slopes less than one correspond to a pattern of underestimating effect size.
Interestingly, the inverted sigmoid shape of the expected response pattern in the LLO model when slopes are less than one (Fig.~\ref{fig:llo_explainer}, purple curves in right column) resembles a prediction from \textit{prospect theory}~\cite{Kahneman1979}: For the purpose of decision-making, low probabilities are treated as more likely than they are, and events with high probabilities are treated as less likely than they are.
% The pattern of underestimating effect size described by the LLO model seems related to an important pattern in decision-making. 
% Prospect theory~\cite{Kahneman1979} describes how people incorporate probability information into incentivized decisions such that events with low probabilities are treated as more likely than they are, and events with high probabilities are treated as less likely than they are (similar to Fig.~\ref{fig:llo_explainer}, bottom right). 
% \idl{Again it's hard to immediately grasp what you mean by looking at Fig 2. Can you add arrows/highlights in the bottom right panel on the visual features that lead to the statement?  I guess we should look at the gap between the curve and the dotted line?}
Kahneman and Tversky~\cite{Kahneman1979} distinguish between \textit{perceiving} the probability of an event to be $p$ and \textit{weighting} the probability of an event in decision-making as $\mathrm{\pi}(p)$, suggesting that the later reflects a preference based on the former.
However, recent work in behavioral economics~\cite{Khaw2017} challenges this assertion by attributing biases in decision preferences---often referred to as risk seeking and risk aversion---to perceptual biases in probability estimation.
Since we include both a probability estimation and a decision task in our experiment, we can examine whether bias in magnitude estimation is coupled with the quality of decisions made by the same user looking at the same chart. 


==> archived/drafts/discussion-draft1.tex <==
\section{General Discussion}
Our results suggest a handful of high level design guidelines for visualizing effect size.
Of the visualization designs we evaluate,
\begin{wrapfigure}{l}{0.34\columnwidth}
    \vspace*{-3mm}
    \centering
    \includegraphics[width=0.33\columnwidth]{figures/decoupling-01.png}
    \caption{Just-noticeable difference (JND) and point of subjective equality (PSE) vs linear in log odds (LLO) slopes per user. Outliers omitted.}
    \label{fig:decoupling}
\end{wrapfigure}
quantile dotplots seem best suited for perceptual accuracy in estimating effect size.
However, intervals and densities seem best for promoting utility-optimal decisions.
User performance on the decision-making task is most robust to different level of variance with densities.
In the decision-making task, adding means consistently biases users away from the utility-optimal decision threshold, suggesting that decision aids showing effect size probably should not include means.

There seems to be a decoupling of magnitude estimation and decision-making performance in our experiment.
We see this in the fact that different visualization designs lead to the best performance on each task.
A more direct illustration is the fact that an individual user's LLO slope does not clearly predict their JND or PSE (Fig.~\ref{fig:decoupling}).
Many individuals who are poor at magnitude estimation do well on the decision task.
Perhaps this is because we incentivize decisions and not estimation, or because the decision task is easier.
However, that we see this decoupling for estimation and decision tasks based on the same signal suggests that perceptual accuracy may not feed forward directly
into decision-making, but that there are other mitigating factors at play.

We set out to test the hypothesis that chart users rely on distance as a visual proxy for effect size without making this judgment relative to the spatial extent of uncertainty encodings.
In our qualitative analysis of strategies we see that the vast majority of users (357 of 442; 80.8\%) rely on distance between distributions or mean difference to judge effect size.
The results of our quantitative analysis suggests that adding means induces small but reliable biases in magnitude estimation, increasing a tendency to underestimate effect size that we associate with a strategies of looking at \textit{only distance}.
One reason the effect of addings means is negligibly small may be that user already tend to rely on \textit{relative position} as a visual feature, a cue which the mean merely reinforces.
Another reason may be the fact that users are heterogeneous in their strategies and switch strategies frequently.


% \subsection{everything is terrible \jessica{+1!}}
\subsection{Reducing User Behavior to a Monolith}
In graphical perception research, we tend to 
oversimplify
% collectively engage in lazy thinking with respect to 
how people read charts. 
In our qualitative analysis, we see that not everyone uses the same strategies or relies on the same visual properties of charts.
A substantial portion of users don't even make the same judgment in the same way when we show them the same chart.
Rather, strategies and heuristics change over time and on a case-by-case basis, not just depending on visualization design. 
This makes it very hard to both predict how people will read charts and study the impact of design choices.
Thus, it appears that the behavior of the average user may not reflect the experience of very many users and that conventional notations of ranked visualization effectiveness average over a lot of variation and reduce user behavior to a monolith.
% \alex{The key thing here is that conventional notations of ranked effectiveness are averaging over a lot of variation and reducing users to a monolith. In the case of the present study, we thought carefully as visualization experts about strategies users might engage in and how different chart designs might lead to more accurate judgments by promoting better strategies. However, users ended up using a mix of strategies---sometimes even at the same time---suggesting that it is unreasonable to think of graphical perception as a single, consistent process. Our results lay bare the shortcomings of how the field has conceptualized perceptual effectiveness of charts. Making visualization a more robust science will require...[say something hopeful so that we aren't just shitting on the field].}

In light of our findings about heterogeneous patterns in user strategies, we envision a new class of behavioral models for visualization research which attempt to learn the proportion of users adopting a set of predefined strategies such as those we identify in our qualitative analysis.
Related work~\cite{Jardine2020} calculates predicted responses if chart users employ a set of  alternative perceptual proxies for visual comparison and shows these predictions alongside user's actual responses.
Although this approach is similar in essence to what we propose, like the present study it merely describes the correspondence between predicted patterns and user behavior. 
% \jessica{could point to similar other research, eg that jardine franconeri paper, as well as maybe whether we would suggest improving that approach}
What we proposes here is that we should aim to incorporate functions representing predefined strategies into predictive models which estimate the proportion of users employing a given strategy.

In an early pilot study, we attempted to build such a model: a custom Bayesian mixture of alternative strategy functions.
However, because multiple strategies predict similar patterns of responses, we were not able to fit the model due to problems with identifiability.
This suggests that the kind of model we propose will only be feasible if we design experiments such that alternative strategies predict sufficiently different patterns of responses.
The approach of looking at the agreement between proxies and human behavior suffers the same limitation, but there is no analogous mechanism to identifiability in Bayesian models to act as a fail-safe against unwarranted inferences. 
% \jessica{any ideas of how we could do this type of work in a sophisticated away without running into this problem? ie is there some happy medium between the conclusions of the jardine work and what we attempted? maybe they just weren't careful enough in noting the limitations of their method? }
Future work should continue pursuing this kind of strategy-aware behavioral modeling.
% We intend to continue pursing this kind of strategy-aware behavioral modeling in future work, \jessica{I generally prefer framing future work activities generally rather than saying that we intend to do them, it becomes unclear if you are suggesting other people back off, which seems like a bad thing to signal in science} perhaps focusing exclusively on different ways that chart users might be judging distance between distributions.


\subsection{Limitations}
Some of our stimulus design choices may have impacted user strategies and performance. 
For instance, our choice to annotate a decision threshold on charts may have led participants to focus on cumulative probability judgments rather than probability of superiority. 

We faced a trade-off between making means the same size for each visualization condition and balancing the salience of the mean in each condition.
We attempted not to make charts that seemed unnaturally out-of-proportion (i.e., ridiculously large means).
However, the resulting stimuli varied in the salience of added means such that means were only highly salient in the HOPs condition.
Because of this, our estimates of the impact of adding means are probably very conservative.

Perhaps our most consequential design choice was holding axis limits constant across chart stimuli.
While constant axis limits were necessary to study our hypothesis about users relying on distance as a proxy for effect size, one could argue that defaults in visualization software would have rendered our stimuli with less white space such that they would look visually similar but with different axis scales. 
However, in some real-world circumstances, axes scales on charts are not optimized for the data in an individual chart.
For example, this is the case when designers facet small multiples, generate forest plots showing multiple distributions on one axis~\cite{Freiman1978}, or follow the axiom that the axis on a bar chart should always include zero.
In agreement with prior work~\cite{Witt2019,Hofman2020}, we think that the tendency to underestimate effect size may change depending on design choices about axis scale. 
Although, we applied the same axis scale to all stimuli in all conditions, so this limitation does not impact comparisons between visualization conditions in our study.

We didn't show users high and low levels of variance together in a single chart.
Given trade-offs around how many within-subjects comparisons we could make in a set number of trials, we decided to prioritize sampling more levels of ground truth effect size.
Not investigating heterogeneous variances directly may limit the generalizability of our inferences. 
Future work should study distributional comparisons with mixed levels of variance (e.g., in forest plots).

Studying incentives on Mechanical Turk is fundamentally unrealistic because users are trying to optimize their bonus in dollars and cents. 
This may not capture how people respond to visualized data in a crisis situation or when lives, careers, or millions of dollars are at stake.


% \section{Conclusion}
% We present results from a controlled experiment investigating how design choices influence judgments and decisions from visualized effect size. 
% We present nuanced guidelines on the basis of our quantitative results. 
% Our accompanying qualitative analysis yields insights about the strategies that chart users employ when making distributional comparisons.
% \idl{The current conclusion is a bit too short; if you're out of space, perhaps you could cut the conclusion if it is not too different than the intro/discussion.}


==> archived/drafts/discussion-draft3.tex <==
\section{Limitations}
\jessica{agree with idl, this belongs at end of general discussion}
\idl{I’m not sure this needs to be its own section. Can you include it as a subsection somewhere else?}
Since most users seem to not completely understand the statistical judgments they should be doing, our choice to include a decision threshold annotation on charts may have led users to judge effect size as cumulative probability rather than probability of superiority. 
This may have contributed to underestimation bias. 
% \jessica{would make clearer that this assumes that they don't totally understand the statistical judgments they should be doing, otherwise it makes sense to add}

The salience of added means may have varied across uncertainty visualizations, with only the means in the HOPs condition being highly salient.
% We faced a trade-off between making means the same size for each visualization condition and balancing the salience of the mean in each condition.
% In an attempt not to make charts that seemed unnaturally out-of-proportion (i.e., ridiculously large means), we created stimuli that varied in the salience of added means, such that means were only highly salient in the HOPs condition. \jessica{this rationalizing doesn't make sense, I'm not sure what its saying. I would just say something like, The salience of added means may have varied across visualization conditions, with only the means in the HOPs condition being highly salient.} 
Because of this, our estimates of the impact of adding means averaging over visualization conditions are probably very conservative.

We held axis limits constant across chart stimuli in order to study our hypothesis about users relying on distance as a proxy for effect size.
% One could argue that defaults in visualization software would have rendered our stimuli with less white space such that different levels of effect size and variance would differ in their axis scales rather than their visual appearance. 
% However, in some real-world circumstances, axes scales are not optimized for the data in an individual chart.
% For example, this is the case when designers facet small multiples, generate forest plots showing multiple distributions on one axis~\cite{Freiman1978}, or follow the axiom that the axis on a bar chart should always include zero.
In agreement with prior work~\cite{Witt2019,Hofman2020}, we think that the tendency to underestimate effect size may change depending on design choices about axis scale. 
Our choice to hold axis limits constant does not impact comparisons between visualization designs in our study.
% Although, we applied the same axis scale to all stimuli in all conditions, so this limitation does not impact comparisons between visualization designs in our study. \jessica{this is too much and makes me question the decision even more. With limitations its best to state the limitation and move on, not give partial reasons to defend yourself, which reads as weaker than just stating it. I would keep the first sentence, then go right to the In agreement with prior work ...., and keep the Although sentence but reword since the Although is a bit awkward, just say, Our choice to hold axis limits constant does not impact comparisons .... }

% \sout{We never showed low and high variance distributions together in a single chart.
% Given trade-offs around how many within-subjects comparisons we could make in a limited number of trials, we decided to prioritize sampling more levels of ground truth effect size.}
Not investigating effects when distributions with heterogeneous variances are visualized in the same chart may limit the generalizability of our inferences. 
Future work should study distributional comparisons with mixed levels of variance (e.g., in forest plots).

Our choice to incentivize the decision-making task but not magnitude estimation may have contributed to the decoupling of performance on our two tasks.
We cannot disentangle this possible explanation from evidence corroborating a distinction between perceived probability and weight given to probability in decision-making.

Studying incentives on Mechanical Turk is fundamentally unrealistic because users are trying to optimize small monetary bonuses. 
This may not capture how people respond to visualized data in a crisis situation or when lives, careers, or millions of dollars are at stake.

\section{General Discussion}
\jessica{again, part of my expects a sentence intro to section}
\subsection{Canonical Design Guidelines}
\jessica{we need some topic sentences in here. Focus on the big takeaways}
Of the visualization designs we test,
quantile dotplots lead to the least bias in estimating effect size.
Densities and intervals promote the most utility-optimal decisions, with densities performing better at lower variance.
In the decision-making task, adding means slightly but consistently biases users away from the utility-optimal decision rule, suggesting that decision aids showing effect size probably should not include means. 
Note that the optimal visualization design is task dependent.
\alex{We may need some additional nuance when talking about the findings from the decision-making task. I am trying to keep things simpler here than in the results section.}

We set out to test the hypothesis that chart users rely on visual distance between distributions as a proxy for effect size.
The results of our quantitative analysis show that adding means induces small but reliable biases in magnitude estimation, consistent with distance-based heuristics.
Our qualitative analysis of strategies verifies that the majority of users (357 of 442; 80.8\%) rely on distance between distributions or mean difference to judge effect size.
However, from a practical standpoint, the impact of adding means is negligibly small.
This may be because users already tend to rely on \textit{relative position} as a visual feature, a cue which the mean merely reinforces. 
% \jessica{this is a good point}

\subsection{Reducing User Behavior to a Monolith}
\jessica{would probably replace this section with the other thing I was suggesting, which could include mentioning the heterogeneity but the main claim would instead be that people use charts in ways that may not be intended in the absence of training, and that we might need to be mindful of these different types of satisficing or heuristics, and try to intentionally train people out of them, try to model them, and consider possible heterogeneity even in the same user. You coudl consider a more memorable section header, like Uncertainty Visualization Use in Theory vs The World, or something like that. Might be worth rethinking sectioning here. Should we try to think of a more memorable paper title?} 
In graphical perception research, we tend to 
oversimplify how people read charts. 
In our qualitative analysis, we see that not everyone uses the same strategies or relies on the same visual properties of charts.
A substantial portion of users don't even make the same judgment in the same way when we show them the same chart.
Rather, strategies and heuristics change over time and on a case-by-case basis, not just depending on visualization design, making it difficult to both predict how people will read charts and to study the impact of design choices.
Thus, the convention of ranking visualization effectiveness based on the performance of the average user (e.g., Cleveland \& McGill~\cite{Cleveland1984}) may not account for the experience of very many users, instead averaging over a lot of variation and reducing user behavior to a monolith.

\subsection{Toward Better Models of Graphical Perception}
In light of heterogeneity in user strategies, we envision a new class of behavioral models for visualization research which attempt to learn the proportion of users adopting a set of predefined strategies, such as those we identify in our qualitative analysis.
Previous work~\cite{Jardine2020} calculates predicted responses if chart users employ a set of alternative perceptual proxies for visual comparison and compares these predictions to users' actual responses.
Although this approach is similar to what we propose, like the present study it merely describes the correspondence between predicted patterns and user behavior. 
Instead, we propose incorporating functions representing predefined strategies into predictive models which estimate the proportion of users employing a given strategy.

In an early pilot study, we attempted to build such a model: a custom Bayesian mixture of alternative strategy functions.
However, because multiple strategies predict similar patterns of responses, we were not able to fit the model due to problems with identifiability.
This suggests that the kind of model we propose will only be feasible if we design experiments such that alternative strategies predict sufficiently different patterns of responses.
The approach of looking at the agreement between proxies and human behavior~\cite{Jardine2020} suffers the same limitation, but there is no analogous mechanism to identifiability in Bayesian models to act as a fail-safe against unwarranted inferences. 
Future work should continue pursuing this kind of strategy-aware behavioral modeling.

We want to emphasize that the proposed modeling approach is not strictly quantitative, as the definition of strategy functions requires a descriptive understanding of users' visual reasoning.
As such this approach offers a way to formalize the insights of qualitative analysis and represent the gamut of possible user behaviors inside of visualization recommendation and authoring systems.

% \idl{Overall nice work. It seems like a solid study on an important and interesting topic. The paper is almost a page too long right now, I would hope that you could take that space away from sections 3 and 4, and keep sections 5 and 7 thorough, as I feel like they are the more interesting sections. You could probably get away with using Bold words at the start of paragraphs rather than the subsections that you have in section 7 to buy a little space there. You should also add a conclusion that recaps all of the contributions of the work. Also the takeaways from section 7 don’t seem to be hinted at in the introduction; if these are contributions of the work make that clear in the intro.}

\section{Conclusion}
We contribute findings from a mixed design experiment on Mechanical Turk investigating how visualization design impacts judgments and decisions from effect size.
Our results suggest that, among the visualizations we tested, quantile dotplots support the least biased estimation of effect size, whereas densities and intervals support the most utility-optimal decision-making based on effect size.
We discuss how a user’s sense of the signal in a chart may not necessarily be identical when they use the same information for different tasks.
We also find that adding means to uncertainty visualizations induces small but reliable biases consistent with users relying on visual distance between distributions as a proxy for effect size.
In a qualitative analysis of users' visual reasoning strategies, we find that many users switch strategies and do not employ an optimal strategy when one exists.
We discuss ways that canonical characterizations of graphical perception in terms of average performance gloss over the heterogeneity in user behavior, and we propose opportunities to build strategy-aware models of visualization effectiveness which could be used to formalize design knowledge in visualization recommendation and authoring systems beyond context-agnostic rankings of chart types.

==> archived/drafts/discussion-submission.tex <==
\section{General Discussion}
% \jessica{we need some topic sentences in here. Focus on the big takeaways}
The optimal visualization design for conveying effect size seems to be task dependent.
Of the visualization designs we test,
quantile dotplots lead to the least bias in estimating effect size, whereas the visualization design which leads to the least bias in decision-making seems to depend on the variance of distributions relative to axis scale.
On a fixed axis scale, densities without means and quantile dotplots with means perform best at lower variance, while densities without means and intervals without means perform best at higher variance.
No visualization designs we tested completely mitigate bias in decision-making at higher variance.
% densities and intervals promote the most utility-optimal decisions, with densities performing reliably better than intervals at lower variance.
We find that adding means slightly biases users away from the utility-optimal decision criterion in most cases, however, this effect may depend on the ways that variance and axis scale impact the visual appearance of distributions.

In particular, the variance of distributions and choice of axis scale impact whether the visual distance between distributions is a good proxy for effect size.
Because we wanted to measure whether chart users rely on distance as a proxy for effect size, we intentionally set up our experiment so that distance would be a consistent cue for effect size at higher variance and a poor cue for effect size a lower variance (Fig.~\ref{fig:distance_strategy}).
The results of our quantitative analysis show that adding means induces small but reliable biases in magnitude estimation, consistent with distance-based heuristics.
Our qualitative analysis of strategies verifies that the majority of users (357 of 442; 80.8\%) rely on distance between distributions or mean difference to judge effect size.
However, from a practical standpoint, the impact of adding means is negligibly small.
This may be because users already tend to rely on \textit{relative position} as a visual feature, a cue which the mean merely reinforces. 
% \jessica{this is a good point}

\subsection{Limitations}
Since most users seem to not completely understand the statistical judgments they should be doing, our choice to include a decision threshold annotation on charts may have led users to judge effect size as cumulative probability rather than probability of superiority. 
This may have contributed to underestimation bias. 

The salience of added means may have varied across uncertainty visualizations, with only the means in the HOPs condition being highly salient.
Because of this, our estimates of the impact of adding means averaging over visualization conditions are probably very conservative.

We held axis limits constant across chart stimuli in order to study our hypothesis about users relying on distance as a proxy for effect size.
In agreement with prior work~\cite{Witt2019,Hofman2020}, we think that the tendency to underestimate effect size may change depending on design choices about axis scale. 
Our choice to hold axis limits constant does not impact comparisons between visualization designs in our study.

Not investigating effects when distributions with heterogeneous variances are visualized in the same chart may limit the generalizability of our inferences. 
Future work should study distributional comparisons with mixed levels of variance (e.g., in forest plots).

Our choice to incentivize the decision-making task but not magnitude estimation may have contributed to the decoupling of performance on our two tasks.
We cannot disentangle this possible explanation from evidence corroborating Kahneman and Tversky's~\cite{Kahneman1979} distinction between perceived probabilities and decision weights (see Section 4.3).

Studying incentives on Mechanical Turk is fundamentally unrealistic because users are trying to optimize small monetary bonuses. 
This may not capture how people respond to visualized data in a crisis situation or when lives, careers, or millions of dollars are at stake.

\subsection{Satisficing and Heterogeneity}
% \jessica{would probably replace this section with the other thing I was suggesting, which could include mentioning the heterogeneity but the main claim would instead be that people use charts in ways that may not be intended in the absence of training, and that we might need to be mindful of these different types of satisficing or heuristics, and try to intentionally train people out of them, try to model them, and consider possible heterogeneity even in the same user. You coudl consider a more memorable section header, like Uncertainty Visualization Use in Theory vs The World, or something like that. Might be worth rethinking sectioning here. Should we try to think of a more memorable paper title?} 
The visual reasoning strategies that chart users rely on when making judgments from uncertainty visualizations may not be what visualization designers expect. 
We present evidence that, in the absence of training, users satisfice by using suboptimal heuristics to decode the signal from a chart.
We also find that not all users rely on the same strategies and that many users switch between strategies.
Satisficing and heterogeneity in heuristics make it difficult to both anticipate how people will read charts and to study the impact of design choices.
Conventionally, visualization research has characterized visualization effectiveness by ranking visualization designs based on the performance of the average user (e.g.,~\cite{Cleveland1984}).
However, in cases like the present study where users are heterogeneous in their strategies, these \textit{averages may not account for the experience of very many users} and are probably an oversimplification.
Visualization researchers should be mindful of satisficing and heterogeneity in users' visual reasoning strategies, attempt to model these strategies, and try to design ways of training users to employ more optimal strategies.

\subsection{Toward Better Models of Visualization Effectiveness}
Because some users seem to adopt suboptimal strategies or switch between strategies when presented with an uncertainty visualization, models of visualization effectiveness which codify design knowledge and drive automated visualization recommendation and authoring systems should represent these strategies.
We envision a new class of behavioral models for visualization research which attempt to enumerate possible strategies, such as those we identify in our qualitative analysis, and learn how often users employ them to perform a specific task when presented with a particular visualization design.
Previous work~\cite{Jardine2020} demonstrates a related approach by calculating expected responses based on a set of alternative perceptual proxies for visual comparison and comparing these expectations to users' actual responses.
Like the present study, this work describes the correspondence between expected patterns and user behavior. 
Instead, we propose incorporating functions representing predefined strategies into predictive models which estimate the proportion of users employing a given strategy.

In an early pilot study, we attempted to build such a model: a custom Bayesian mixture model of alternative strategy functions.
However, because multiple strategies predict similar patterns of responses, we were not able to fit the model due to problems with identifiability.
This suggests that the kind of model we propose will only be feasible if we design experiments such that alternative strategies predict sufficiently different patterns of responses.
The approach of looking at the agreement between proxies and human behavior~\cite{Jardine2020} suffers the same limitation, but there is no analogous mechanism to identifiability in Bayesian models to act as a fail-safe against unwarranted inferences. 
Future work should continue pursuing this kind of strategy-aware behavioral modeling.

We want to emphasize that the proposed modeling approach is not strictly quantitative, as the definition of strategy functions requires a descriptive understanding of users' visual reasoning.
As such this approach offers a way to formalize the insights of qualitative analysis and represent the gamut of possible user behaviors inside of visualization recommendation and authoring systems.

% \idl{Overall nice work. It seems like a solid study on an important and interesting topic. The paper is almost a page too long right now, I would hope that you could take that space away from sections 3 and 4, and keep sections 5 and 7 thorough, as I feel like they are the more interesting sections. You could probably get away with using Bold words at the start of paragraphs rather than the subsections that you have in section 7 to buy a little space there. You should also add a conclusion that recaps all of the contributions of the work. Also the takeaways from section 7 don’t seem to be hinted at in the introduction; if these are contributions of the work make that clear in the intro.}

\section{Conclusion}
We contribute findings from a mixed design experiment on Mechanical Turk investigating how visualization design impacts judgments and decisions from effect size.
Our results suggest that visualization designs which support the least biased estimation of effect size do not necessarily support the best decision-making.
% , among the visualizations we tested, quantile dotplots support the least biased estimation of effect size, whereas densities and intervals support the most utility-optimal decision-making based on effect size.
We discuss how a user’s sense of the signal in a chart may not necessarily be identical when they use the same information for different tasks.
We also find that adding means to uncertainty visualizations induces small but reliable biases consistent with users relying on visual distance between distributions as a proxy for effect size.
In a qualitative analysis of users' visual reasoning strategies, we find that many users switch strategies and do not employ an optimal strategy when one exists.
We discuss ways that canonical characterizations of graphical perception in terms of average performance gloss over possible heterogeneity in user behavior, and we propose opportunities to build strategy-aware models of visualization effectiveness which could be used to formalize design knowledge in visualization recommendation and authoring systems beyond context-agnostic rankings of chart types.

==> archived/drafts/intro-draft1.tex <==
%% \section{Introduction} %for journal use above \firstsection{..} instead
% Problem exposition
\alex{I'm planning to revise/rewrite the intro based on your comments here, probably after we have a chance to discuss the paper as a whole.}

New computing technologies and an increasingly interconnected world have led to a proliferation of data-intensive probabilistic modeling and prediction. \jessica{not sure what the increasingly interconnected world part means} 
Both in organizational settings (e.g., data science for business intelligence) and in the public domain (e.g., data journalism), predictions are often presented as point estimates. 
A recent survey and interview study of visualization designers finds that presenting uncertainty is often seen as obfuscating the “signal” or message that is conveyed by a visualization (Hullman 2020). 
Visualization practitioners also worry that presenting uncertainty will undermine users’ trust in the process through which estimates or predictions are made and then visualized. 
Ironically, omitting uncertainty information from technical communications leads to ``incredible certitude'' (Manski 2018), the unwarranted implication that error is minimal or not important. 
Insofar as probabilistic modeling is used to inform decision-making, both at an individual level (e.g., whether or not to vote Westwood 2018) and an institutional level (e.g., policy decisions Manski 2018), misleading users about the degree of certainty in predictions can be profoundly harmful.

\matt{Dunno how well this [that we should show people uncertainty] follows from the previous paragraph ... you seem more to be setting up that people don't use it because they don't trust it, yet a solution to people not using it because they don't trust it is not to tell them to use it... because they won't}
\alex{Possible issues with hook. Maybe we should tweak or rewrite?}
\jessica{yes I would just go right from the 'things are often presented as point estimates' to 'A common suggestion is that ....' and integrate a sentence or two about why uncertainty can be beneficial. But then jump right into the heuristics piece}

% The plot thickens: visualizing uncertainty may not be enough
A common suggestion is that reports of point estimates should be supplemented with uncertainty information, for example, by showing intervals in which possible values of that estimate could fall (Cumming 2005; Cumming 2014; Manki 2018). 
However, there are reasons to think that simply presenting uncertainty information alongside point estimates won't work. A large body of work on heuristics and biases has shown that people often try to avoid or discount uncertainty information (Tversky and Kahneman 1974; other cites in JDM). Within visualization research, there is some evidence that people discount uncertainty when presented with means and intervals, focusing excessive attention on means (Hullman 2015).
\jessica{I wonder if there is anything else? Might be worth searching.}
\jessica{I would now go into reasons why overelying on means can be bad, before getting into our contributions. After establishing that means can be bad for certain judgments, I might introduce the idea of different encodings for uncertainty making it easier/harder to focus on means }

% Effect size
In this study, we investigate how the salience of the mean in uncertainty visualizations impacts judgments of effect size and incentivized decisions based on effect size. 
\alex{In this study, we investigate how design choices in uncertainty visualizations may affect the strategies people use to make judgments and decisions.}
We focus on \jessica{a proxy for} the standardized mean difference, a measure of effect size which combines both signal and noise into a standard quantification of the difference between two groups on a continuous outcome (Coe 2002; others): \jessica{explain probability of superiority, also known as Common Language Effect Size [cite is from McGraw et al I think]}. \matt{don't we acually focus on probability of superiority?} 
Chart users have an incentive to make accurate judgments of the standardized mean difference in situations where they must choose whether to purchase an intervention or stick with the status quo (e.g., Dan and Jake study, Joslyn). 
In essence, effect size judgments require understanding both point estimates and the uncertainty of those estimates in relation to one another.

% Framing Research Questions
Discounting uncertainty and focusing instead on means is particularly undesirable when users make judgments and decisions about effect size. 
Although the mean difference between two groups may serve as a good heuristic for effect size when the variance of a distribution is high, we expect that focusing attention on means will lead to underestimates of effect size when distributions with relatively low variance are shown on the same axis scale. 
Imagine a user views charts of predictions with mixed levels of variance. 
For distributions where prediction uncertainty is high, larger mean differences correspond to larger effect sizes. 
However, for distributions where prediction uncertainty is relatively low, a mean difference that looks small on a chart might represent a large and reliable effect. \jessica{I lean toward moving some of this up to where you mention heuristics}
Thus, \textit{we hypothesize that chart users will underestimate effect size when the mean is highly salient and uncertainty in predictions is low relative to other predictions mapped to the same axis scale}. \jessica{Now that I think about it I worry that this same axis scale thing we did may be another thing that makes our results hard to generalize - often people will just scale axes to the data in the chart. I suspect maybe if we hadn't done this, errors from using mean difference would be higher in the low variance case, so our results about variance level may be specific to this choice} \alex{The way I talk about this in the results is that charts which are rescaled to match the data domain would more likely resemble the stimuli at high variance, where as the low variance condition reflects the the impact of our choice to fix the axis scale. The low variance results apply in cases where multiple distributions with heterogeneous variances are shown on a common axis.}
We design an experiment to test for this pattern of perceptual bias in effect size judgments, and we examine whether presenting model predictions in ways that de-emphasize point estimates helps to mitigate this bias.

\jessica{would introduce these ideas of uncertainty visualizations differing slightly earlier }
Imagine a continuum of uncertainty visualization formats representing how perceptually difficult it is to decode the mean from a visualization and, thus, to ignore uncertainty. 
At one extreme are hypothetical outcome plots or HOPs (Hullman 2015; Kale 2018) where the mean is only encoded implicitly as the average of a set of predicted outcomes presented across frames of an animation. 
At the other extreme are direct encodings of point estimates presented alongside uncertainty represented as intervals (e.g., error bars) or text (e.g., margin of error). 
In between these two endpoints on the continuum are uncertainty visualizations such as probability densities and quantile dotplots (Kay 2016) where the mean is encoded as the point where the distribution is at its maximum height. 
We suspect that uncertainty visualization formats which emphasize the mean less may lead to the least biased judgments and decisions from effect size information.
Based on the findings of previous work (Hullman, Kay, Kale, Fernandes), we also expect that visualizations that convey probability as frequencies of events will also lead to the least biased judgments.
\jessica{we'll probably need a figure in the paper that shows all four chart conditions with and without means} \alex{I'm thinking this would make for a good teaser figure}


% Contribution statement
We contribute the results of a crowdsourced study investigating lay user’s judgments and decisions from effect size when using different uncertainty visualizations with and without extrinsic means. 
Our findings prescribe nuanced design guidelines about the adding means to visualizations showing effect size. 
\jessica{I guess this is true, but the size of the effects in most cases for means is so incredibly small at times that it calls into question the need for nuanced guidelines. We should spell out somewhere before we go into the results here that the effects are really small, and that they are slightly bigger between visualization conditions}
For example, when visualized estimates with different levels of variance are shown on a common axis---as they often are in forest plots---chart users are biased toward underestimating effect size when means are added to distributions with relatively low variance.
However, adding means to distributions can be beneficial when variance is constant across distributions and uncertainty is encoded using intervals or densities.
In our decision-making task, adding means to uncertainty visualizations seems to exacerbate bias, leading to a slightly lower rate of utility optimal decisions.

The results of our experiment also shed light on the relationship between perceptual bias in effect size estimation and performance in incentivized decisions.
We find a loose coupling between metrics of perceptual bias and metrics of sensitivity and bias in decision-making.
This suggests that the visualization community should not assume that rankings of visual encodings from canonical graphical perception studies which measure magnitude estimation (e.g., Cleveland and McGill 1984) will generalize to decision tasks.
Our results suggest that, of the visualizations we tested, quantile dotplots are optimal for effect size estimation, while intervals and densities \textit{without means} are best for decision tasks. 

==> archived/drafts/intro-draft2.tex <==
%% \section{Introduction} %for journal use above \firstsection{..} instead
A recent survey and interview study of visualization designers finds that presenting uncertainty is often seen as obfuscating the ``signal'' or message that is conveyed by a visualization~\cite{Hullman2020}. 
However, the common practice of omitting uncertainty information visualizations and focusing attention on point estimates leads to ``incredible certitude''~\cite{Manski2018a,Manski2018b}, the unwarranted implication that error is minimal or not important. 
A common suggestion to designers is to present uncertainty information alongside point estimates, for example, by showing intervals in which possible values of that estimate could fall~\cite{Cumming2005,Cumming2014,Manski2018b}. 

However, simply presenting uncertainty alongside point estimates may not lead to the incorporation of uncertainty information into users' judgments. 
A large body of work on heuristics and biases (e.g.,~\cite{Tversky1974,Tversky1981,Kahneman2011}) has shown that people often avoid or discount uncertainty information.
\jessica{suggestion - now say make clear that its possible to ignore uncertainty in favor of means when they are graphically presented. Then, jump to 'Different visualization design choices' paragraph. After that, then introduce distance heuristics, e.g But how might users of visualizations who focus on means judge effect size? Imagine a user viewing a visualization like 'example fig'. Discounting uncertainty may manifest as ... Then do the 'As with any' paragraph. Reason for this - you're jumping in to distance heuristic before setting up the necessary point about how someone can still ignore uncertainty when means are visually distinguishable in an uncertainty vis. it's too quick of a jump and I think readers will be confused.  }
In the context of graphical perception, discounting uncertainty might manifest in using \textit{distance as a proxy for effect size} (e.g, when looking at intervals with means~\cite{Hullman2015}) and failing to judge distance between means relative to the spatial extent of intervals.

As with any heuristic, there are specific cases where using visual distance between means as a proxy for effect size leads to a predictable pattern of bias. In our study, we investigate charts showing various effects on a fixed axis (Fig.~\ref{fig:teaser}) such that when distributions have lower variance, visual distance between means is small regardless of effect size.
Conversely, distances correspond to effect size consistently at relatively higher variance.
Thus, in our study, we expect that adding means to uncertainty visualizations leads users to underestimate effect size at lower variance and that means may reduce this underestimation bias at higher variance.
While this prediction depends on fixing axis limits across charts, it gives us a behavioral signature to look for in order to determine whether users rely on a visual distance heuristic.

Different visualization design choices make the mean more or less salient.
Imagine a continuum of uncertainty visualization designs representing how perceptually difficult it is to decode the mean from a chart. 
At one extreme are hypothetical outcome plots or HOPs~\cite{Hullman2015,Kale2019-hops} where the mean is only encoded implicitly as the average of a set of outcomes presented across frames of an animation.
At the other extreme are direct encodings of point estimates presented alongside uncertainty represented as intervals (e.g., error bars) or text (e.g., margin of error). 
We expect that the salience of the mean in uncertainty visualization design---as well as other factors such as frequency-framing of probabilily~\cite{Hullman2015,Kay2016,Kale2019-hops,Fernandes2018}---influence the degree to which users base judgments of visualized effect size on distance regardless of uncertainty.

% Contribution statement
We contribute a crowdsourced experiment investigating how different uncertainty visualization designs impact lay users' judgments and decisions from effect size.
Our approach involves iterative experimental design and Bayesian modeling, culminating in a preregistered study which enables us to make precise inferences about the impact of visualization design choices. \jessica{the iterative experimental design strikes me as what you do with any experiment. You can mention Bayesian model, but I don't think its necessary. Those were our choices but they don't make us special.} \jessica{As a contribution paragraph, this could be crisper. Eg we contribute the results of a crowdsourced experiment ... Through a pre-registered mixed design study involving XX participants, we contribute findings that can inform how authors make design choices about visualization uncertainty.  [Describe main results that can inform design directly] [Describe meta results, eg different visualizations are most effective for different tasks. People tend to switch strategies and may not get the optimal strategy when one exists]}
% For example, adding means to charts results in less utility-optimal decision-making and a pattern of bias in magnitude estimation resembling reliance on distance as a proxy.
% However, the biasing effect of means on effect size estimates is so small that it is practically neglibible.
% \idl{This example seems too detailed to be in the intro. It took me a while to decode the sentence and gauge the point it serves to illustrate: are you trying to provide an example of "precise inferences"? If so, you might skip the details and simply mention that you find a very small biasing effect in some conditions.}
Our results suggest that quantile doplots lead to the least bias in magnitude estimation, but densities and intervals lead to the least bias in decision-making.
The decoupling of performance on our two tasks suggests that visualization designs which support magnitude estimation are not necessarily best suited as decision aids.
When we add means to uncertainty visualizations, we see patterns of user behavior resembling reliance on visual distance as a proxy for effect size.
In a qualitative analysis of users' strategy descriptions, we find that the majority of users rely on visual distance regardless of uncertainty information, that many switch between strategies, and that very few users employ an optimal strategy when one exists. \jessica{something about discussing implications for design and study of uncertainty vis etc}


==> archived/drafts/method-draft2.tex <==
\section{Method}
We set out to test how different uncertainty visualization designs impacts users’ ability to judge the magnitude of effect size and make incentivized decisions based on effect size. \jessica{this sentence seems a little generic, would make more specific eg we set out to test how the addition of a mean impacted users of four different uncertainty encodings judgments and decisions.} 
Requirements we sought for our task were (1) a defined ground truth for effect size, (2) a realistic incentive structure where utility-optimal decisions were defined assuming risk neutrality, and (3) targeted measurements of the extent to which chart users treat distance as a proxy for effect size. \jessica{This sentence seems uncontextualized here. the targeted measurements part isn't clear. could rephrase as something like 'Our experiment asked participants to make effect size judgments, which we evaluated relative to the ground truth effect size, as well as decisions under realistic incentives that could be evaluated against a utility optimal decision assuming risk neutrality.}

% We set out to test how adding markings encoding the mean to different uncertainty visualization formats impacts users’ ability to judge the magnitude of effect size and make incentivized decisions based on effect size. 
% Requirements we sought for our task were a defined ground truth for both judgments, an incentive structure mirroring real-world decisions, and targeted measurements of the extent to which chart users treat distance as a proxy for effect size. 
% \jessica{to evaluate hypotheses about mean difference heuristics}
% To this end, we showed users visualizations comparing the predicted performance of a team with versus without adding a new player, and we asked them to (1) judge the probability that the team scores more points with the new player than without (i.e., probability of superiority~\cite{McGraw1992}) and (2) decide whether or not to pay to add the new player to their team given an incentive structure were utility-optimal decisions were defined assuming risk neutrality.
% Each participant used one type of uncertainty visualization and completed two blocks of trials, one with means added and one without. 
% We analyzed users’ estimates and decisions under each visualization condition to model biases in effect size judgments.

\jessica{organization in this section could use a major revision - I don't think we're giving enough of the intuition behind the visualization conditions experimental design, overall framing of task, and framework for evaluating decisions early enough to give the reader grounding for making sense of all these details. Check out the Fernandes et al CHI 2018 bus paper - there are parallels where we could set up the overall design and procedure, then talk about the fictional scenario, perhaps the visualizations/conditions, then the utility framework, then model, then participant details (some things may need to change slightly, but I think the general flow would be a lot easier to follow) Things like sampling ground truth, generating stimuli should come after you've laid out the overall design and procedure, framing/scenario, etc. } 

\subsection{Data Collection}
\subsubsection{Task \& Interface}
We set up our task as a fantasy sports game where participants had to decide whether or not to pay to add new players to their team. 
On each trial, we showed participants a chart comparing the predicted number of points scored by their team with the new player added versus without the new player (e.g., Fig.~\ref{fig:teaser}). 
We asked users to estimate the probability that the team would score more points with the new player than without (i.e., probability of superiority \jessica{or Common Language Effect Size}~\cite{McGraw1992}). 
Then we asked them whether or not they wanted to pay to add the new player to their team. 

\textbf{Elicitation:}
A large body of prior work on statistical reasoning (e.g.,~\cite{Gigerenzer1995,Hoffrage1998}) suggests that people \jessica{are able to reason with} \sout{comprehend} probabilities \sout{most effectively} \jessica{more accurately} when they are framed as frequencies. 
As such, we elicited probability of superiority judgments as frequencies by asking, \textit{``How many times out of 100 do you estimate that your team would score more points with the new player than without the new player?''}
We collected responses using text entry inputs for effect size estimates and radio buttons for intervention decisions. \jessica{might want to say the radio button options to make clear that it was forced choice}
% We used text entry HTML inputs to collect their estimates and used Javascript for validation such that only numerical responses between 0 and 100 were accepted. \jessica{don't think you need to say the part about validation, that's considered a given for this type of thing} Intervention decisions were elicited using radio buttons. 

\textbf{Feedback:}
In naturalistic decision-making scenarios, people experience the probabilistic consequences of their chosen course of action (e.g., whether or not a chosen treatment cures a disease).
Therefore, at the end of each trial we provided feedback which told users whether or not their team scored enough points to win an award~\alex{Do we need a screenshot of the feedback div?}.
% At the end of each trial, users clicked a button to request feedback. 
We \jessica{generated this feedback by} simulating an outcome based on whether or not the user chose to pay for the new player. 
% \jessica{say we showed them it and how. Probably would be good to show the experiment interface}
The feedback showed tables breaking down how their account value changed this trial \jessica{confusing wording of prev phrase}, what their running account value was, and how this translated into an expected bonus \jessica{they would earn} in real money. \jessica{is expected bonus cumulative bonus they are guaranteed at that point, or expectation of bonus conditional on continuing to perform that way (its ambiguous)}
Our choice to emphasize probabilistic outcomes, rather than the expected value of decisions, made this feedback a noisy signal for how well participants were doing, mirroring learning conditions about uncertainty information in the real world. 

\textbf{User Strategies:}
To \jessica{supplement our quantitative measures with qualitative descriptions of} \sout{deepen our understanding of} users' visual reasoning, \sout{we elicited strategy descriptions.}
at the end of each of the two block of trials, we asked users, \textit{``How did you use the charts to complete the task? Please do your best to describe what sorts of visual properties you looked for and how you used them.''}
% This question gave us deeper understanding of users' visual reasoning strategies. \jessica{again, motivation first, here could just have a phrase like, To deepen our understanding of users' ..., we }

\textbf{Incentives for Decisions:}
% We framed the decision task as seeking potential gains. 
\jessica{it may be useful to have topic sentences for paragraphs in this section. maybe that means you shorten the motivation earlier on. but reader might appreciate some higher level sense of what they are reading}

\jessica{The participant's goal} in the fantasy sports game \sout{, the participant tried} \jessica{was framed as} \sout{to} winning awards worth \$3.17M each.

We instructed participants \jessica{that} to maximize the value of their fantasy sports account, \sout{ by winning awards, and only pay for the new player if they are worth the cost.%\jessica{user is probably ok, though participant is more conventional.}
} \jessica{they should pay} \$1M to add that player to their team if they thought the new player improved their chances of winning enough. 
On each trial, there were four possible payouts: 
\begin{enumerate}
    \vspace*{-2mm}\item The participant won without paying for the new player (+\$3.17).
    \vspace*{-2mm}\item The participant paid for a new player and won (+\$2.17M).
    \vspace*{-2mm}\item They failed to win without paying for the new player (\$0).
    \vspace*{-2mm}\item The participant paid for the new player and failed to win (-\$1M). 
\end{enumerate}
\vspace*{-2mm} Note that the only way for the user to lose money on a given trial was if they paid for the new player.
~\footnote{In pilot studies, we tested how framing outcomes as winning versus losing awards impacted user behavior and found that participants had greater preference for intervention when it was described as increasing the certainty of gains, consistent with prior work by Tversky and Kahneman~\cite{Kahneman1979,Tversky1981}.
% In pilot studies, we tested gain vs loss framing versions of the task and replicated findings from Tversky and Kahneman (1979, 1981) \jessica{Will these be described?}\alex{Framing effects are out of scope (hence why they are in a footnote), but I thought I should mention that we tried this variation of the task. Do you think we need to describe?} \jessica{a brief description of the findings from T and K is what I was thinking we need, like what's the pattern at a high level that we also saw} 
}

Optimally, participants should have paid to add the new player only when effect size was larger than a certain threshold. 
We set the incentives in our experiment such that the threshold was about 74\% probability of superiority or a Cohen’s d of 0.9, which was the average effect size in a recent survey of studies in experimental psychology~\cite{Schafer2019}.
Participants received base compensation of \$1 plus a bonus of $\$0.08\cdot(account - \$150M)$, where \$0.08 was the exchange rate \jessica{explain for what}, $account$ was the value of their fantasy sports account at the end of the experiment, and \$150M was a cutoff account value chosen to get bonuses in a desirable range. \jessica{These values were carefully chosen so as to [what?] (I feel like we should be giving the reader more guidance in here on why we did all this, though i know we are short on space}  
On average, participants were compensated \$2.24 and took 16 minutes to complete the experiment. \jessica{this doesn't belong here. Put at beginning of results or end of participants section (moving that to be later in this section)}



\subsubsection{Formalizing Utility}
\jessica{This section is hard to follow. Consider changing title to something like 'Evaluating Decisions: Utility Framework' See how we introduced utility in the Fernandes paper, eg 'To improve the likelihood that subjects in our experiments engaged in realistic decision-making, we adapted a paradigm commonly used to study decision-making in behavioral economics and related fields [4, 29, 10]. In this paradigm, subjects make decisions and are financially rewarded or penalized (as
they would be in real decision contexts) according to a utility function. (we should say something to this effect earlier. In general this whole methods section needs more handholding for the reader to make sense of the why behind these things}


In intervention decisions, whether or not a user should intervene depends on both \jessica{the amounts of the monetary rewards (and penalties) they stand to earn} \sout{incentives} and the effect size \jessica{of the team performance with and without the new player}. 
\sout{The} Specifically, \sout{incentives that mattered to} users \jessica{needed to attend to} \sout{in our task were} the value of an award and the cost of adding a new player to their fantasy sports team. 
Effect size described the relative performance of their team with versus without the new player such that effect size determined the probability of winning an award with the new player, given a fixed baseline chance of winning an award without the new player. \jessica{This last phrase is confusing} 
Thus, \textit{the degree of evidence in favor of the decision to intervene was a monotonically increasing function of effect size}. \jessica{is there a way to motivate why we need this directly earlier in the section? I feel like the cleverness of what we did isn't coming through as much as it could bc reader may not understand that all this wasn't arbitrary }
We formalized this problem using a normative decision rule based on maximizing expected utility~\cite{vonNeumann1944}, and we used this formalization to design our task and analyze user performance. 

Let $v$ be the value of an award.
Let $c$ be the cost of adding a new player to the team. 
The utility optimal decision rule is to intervene if:
$$v \cdot \Pr(award|\neg player) < v \cdot \Pr(award|player) - c$$
% \matt{some notational suggestsions: if $p(...)$ is probability and not density, maybe use $\Pr(...)$ or $\mathbb{P}(...)$. Since you use $\sim$ elsewhere for probability statements I would use $\neg$ for ``not''. Don't use * for multiplication in math, it's a code thing (put things beside each other or use $\cdot$ or $\times$; even $\times$ is controversial as some would rather only see it for cross product). Capitalized letters might be confused with random variables, especially $X$, so I would consider not using them (or at least not $X$, which anyway could have a better name...). So maybe: $x\cdot\Pr(award|\neg player)$. Whatever you choose for probability notation I would update previous text to match (e.g. the stuff with $\pi(p)$ in an earlier section, which is currently confusing because of use of $p$ here).} 
where $\Pr(award|\neg player)$ is the baseline probability of winning the award \textit{without} the new player, and $\Pr(award|player)$ is the probability of winning the award \textit{with} the new player.
Assuming a constant ratio between the value of the award and the cost of intervention $k = \frac{v}{c}$, we express the decision rule in terms of the difference between the probabilities of winning the award with versus without a new player: %\matt{is there a missing connecting sentence here or something? equation just drops itself in there. Or maybe just need a colon at the end of the last sentence?}
$$\Pr(award|\neg player) + \frac{1}{k} < \Pr(award|player)$$

This formalization represents a \textit{class of decision problems} where users face an all-or-nothing probabilistic outcome and have the option of paying for an intervention that changes the probability of that outcome. 
Examples include medical decisions about drugs or surgeries that may save someone’s life or cure them of a disease, organizational decisions about hiring personnel to reach a contract deadline, or personal decisions such as paying for education to seek a promotion. \jessica{This would be good to say early in the method section to give ppl more intuition about the task}

In our study, we focused specifically on how users incorporate visualized effect size into this kind of utility judgment by fixing the incentives $k = 3.17$ and the baseline probability of winning the award without the new player $\Pr(award|\neg player) = 0.5$.~\footnote{In pilot studies, we tried manipulating $k$ and $\Pr(award|\neg player)$ and found that changing the incentives of the task had little impact on the effectiveness of different visualization conditions for supporting utility optimal decision-making. In light of prior work showing that MTurk workers do not respond to changes of incentives~\alex{cite?}, we suspect that these manipulations might have an impact in real-world settings which is difficult to measure on crowdsourcing platforms.} 
\jessica{give some intuition for the fixing of incentives, many readers might not understand implications of this versus alternative}
%\matt{put this footnote after the . to avoid it looking like an exponent (after-the-period generally looks better for footnotes anyway and I would suggest using it everywhere.)}

\subsubsection{Visualization Conditions}
\jessica{have you mentioned yet whether vis conditions are between participants or not? seems important context for reader as they read about conditions}
We evaluated \sout{a set of} visualizations \sout{conditions which} \jessica{intended to} span a design space characterized by the visual salience of the mean, expressiveness of uncertainty representation, and discrete versus continuous encodings of probability. 
We showed each of \sout{the following} \jessica{four}
\begin{wrapfigure}{r}{0.34\columnwidth}
    \vspace*{-3mm}
    \centering
    \includegraphics[width=0.33\columnwidth]{figures/stim-intervals-02.png}
    \setlength{\abovecaptionskip}{-5pt}
    \setlength{\belowcaptionskip}{-7pt}
    \caption{``Intervals contain 95\% of the possible numbers of points that could be scored by your team with (top) and without the new player (bottom).''}
    \label{fig:intervals}
    \vspace*{4mm}
    \centering
    \includegraphics[width=0.33\columnwidth]{figures/stim-HOPs-02.png}
    \setlength{\abovecaptionskip}{-5pt}
    \setlength{\belowcaptionskip}{-7pt}
    \caption{``Moving lines represent individual predictions of the number of points that could be scored by your team with (top) and without the new player (bottom).''}
    \label{fig:HOPs}
\end{wrapfigure}
uncertainty visualization formats\jessica{--intervals, hypothetical outcome plots (HOPs), density plots, and quantile dotplots--}  with and without a separate (i.e., extrinsic) vertical line encoding the mean of each distribution.
We expected that adding means would bias effect size estimates toward discounting uncertainty and that this effect would be most pronounced for uncertainty encodings in which the mean is not intrinsically salient. 

% \begin{wrapfigure}{r}{0.34\columnwidth}
%     \vspace*{-5mm}
%     \centering
%     \includegraphics[width=0.33\columnwidth]{figures/stim-intervals-02.png}
%     \setlength{\abovecaptionskip}{-5pt}
%     \setlength{\belowcaptionskip}{-7pt}
%     \caption{``Intervals contain 95\% of the possible numbers of points that could be scored by your team with (top) and without the new player (bottom).''}
%     \label{fig:intervals}
% \end{wrapfigure}

\textbf{Intervals:}
We showed users intervals representing a range containing 95\% of the possible point values that the team could score (Fig.~\ref{fig:intervals}). 
While the middle of the interval implicitly encoded the mean, this uncertainty encoding did not make the mean intrinsically salient. \jessica{you mean without mean added? Maybe say, We chose to test intervals because in the absence of a separate mark for the mean, the mean is not intrinsically encoded, and intervals are not very expressive .. ,}
Intervals were not very expressive of probability density since they only encoded lower and upper bounds on a distribution. 
Numerous studies have shown that intervals are not the most effective uncertainty encoding~\cite{Correll2014,Hullman2015,Kale2019-hops} and that laypeople and scientists alike struggle to interpret them~\cite{Belia2005,Soyer2012,Hoekstra2014,Hofman2020}, yet they remain very common. \jessica{Don't we say this in related work}

% \begin{wrapfigure}{r}{0.34\columnwidth}
%     \vspace*{-6mm}
%     \centering
%     \includegraphics[width=0.33\columnwidth]{figures/stim-HOPs-02.png}
%     \setlength{\abovecaptionskip}{-5pt}
%     \setlength{\belowcaptionskip}{-7pt}
%     \caption{``Moving lines represent individual predictions of the number of points that could be scored by your team with (top) and without the new player (bottom).''}
%     \label{fig:HOPs}
% \end{wrapfigure}

\textbf{Hypothetical Outcome Plots (HOPs):}
We showed users animations in which sequentially displayed strips represent draws from a distribution of possible point values that the team could score (rendered as a static strip plot in Fig.~\ref{fig:HOPs}).
\jessica{Similar to intervals, HOPs do not make the mean intrinsically salient, as it is}
\sout{With HOPs the mean was} implicitly encoded as the average position of an ensemble of strips shown over time \sout{, so the mean is not intrinsically salient.}
\jessica{However,} HOPs \jessica{are more expressive of the underlying distribution than intervals, and} express uncertainty as frequencies of events, so they conveyed an experience-based sense of probability through discrete markings. 
\jessica{again, next part should go in related work only, not both}
Prior work on HOPs~\cite{Hullman2015,Kale2019-hops} suggests they are a relatively effective uncertainty visualization format for supporting effect size judgments among untrained users.

\begin{wrapfigure}{r}{0.34\columnwidth}
    \vspace*{-6mm}
    \centering
    \includegraphics[width=0.33\columnwidth]{figures/stim-densities-01.png}
    \setlength{\abovecaptionskip}{-5pt}
    \setlength{\belowcaptionskip}{-7pt}
    \caption{``The height of the shaded area represents the chances that different numbers of points could be scored by your team with (top) and without the new player (bottom).''}
    \label{fig:densities}
    \vspace*{4mm}
    \centering
    \includegraphics[width=0.33\columnwidth]{figures/stim-QDPs-01.png}
    \setlength{\abovecaptionskip}{-5pt}
    \setlength{\belowcaptionskip}{-7pt}
    \caption{``Each dot represents a 5\% chance that different numbers of points could be scored by your team with (top) and without the new player (bottom).''}
    \label{fig:QDPs}
\end{wrapfigure}

% \begin{wrapfigure}{r}{0.34\columnwidth}
%     \vspace*{-10mm}
%     \centering
%     \includegraphics[width=0.33\columnwidth]{figures/stim-densities-01.png}
%     \setlength{\abovecaptionskip}{-5pt}
%     \setlength{\belowcaptionskip}{-7pt}
%     \caption{``The height of the shaded area represents the chances that different numbers of points could be scored by your team with (top) and without the new player (bottom).''}
%     \label{fig:densities}
% \end{wrapfigure}

\textbf{Densities:} 
We showed users continuous probability densities where the height of the area marking encoded the probability of scoring the corresponding number of points on the x-axis (Fig.~\ref{fig:densities}).
\jessica{Unlike intervals and HOPs,}
Because distributions were symmetrical, the mean was explicitly represented as the point of maximum mark height and was thus intrinsically salient in this uncertainty encoding.
\sout{While} Densities \jessica{were also the most expressive} \sout{showed the most granular expression} of \jessica{the underlying} probability density 
\jessica{function} of any conditions we tested \sout{, prior work found that users interpret probability density more accurately when it is discretized, i.e., quantile dotplots~\cite{Kay2016,Fernandes2018}.
Thus, the expressiveness of densities may not translate into effective use. }

% \begin{wrapfigure}{r}{0.34\columnwidth}
%     \vspace*{-12mm}
%     \centering
%     \includegraphics[width=0.33\columnwidth]{figures/stim-QDPs-01.png}
%     \setlength{\abovecaptionskip}{-5pt}
%     \setlength{\belowcaptionskip}{-7pt}
%     \caption{``Each dot represents a 5\% chance that different numbers of points could be scored by your team with (top) and without the new player (bottom).''}
%     \label{fig:QDPs}
% \end{wrapfigure}

\textbf{Quantile Dotplots:}
We showed users dotplots where each one of 20 dots represented a 5\% chance that the team could score the corresponding number of points on the x-axis (Fig.~\ref{fig:QDPs}).
\jessica{Similar to density plots,} because distributions were symmetrical \jessica{(and dots were stacked),} the mean was explicitly represented as the point of maximum height and was thus intrinsically salient. 
\jessica{Similar to HOPs,} quantile dotplots~\cite{Kay2016} convey uncertainty \sout{as discrete markings which can be counted and thus convey uncertainty} as frequency. \sout{, similar to HOPs.}
\jessica{My edits in here are aimed at 1) using more similar language between sections and 2) making clear the continuums we are talking about in intro to section}

\subsubsection{Sampling the Ground Truth}
We selected levels of ground truth probability of superiority (i.e., effect size) so that samples spanned probabilities between 55\% and 95\%, inclusive. 
This represented a range of ground truth effect size between no effect (i.e., 50\%), where the new player did not improve the team’s performance at all, and a very large effect (i.e., 100\%), where the new player definitely improved performance. 
We sampled these values so that half of them fell above the utility-optimal decision threshold of about 74\% and half of them fell below. 
This guaranteed that each user would see an equal number of trials where they should pay for the new player as where they shouldn’t pay. 
We sampled eight distinct levels of ground truth probability of superiority, four values between 55\% and just below 74\% and four values between just above 74\% and 95\%.
We converted probabilities into log odds units and sampled on this transformed scale using linear interpolation between the endpoints of the two ranges described above. 
Our choice to sample uniformly in log odds units was informed by prior work in perceptual psychology~\cite{Gonzalez1999,Zhang2012} suggesting that the brain represents probability on a log odds scale.  \jessica{motivation first}
\sout{In addition to the eight levels of ground truth we sampled for our analysis,} We \sout{also included} \jessica{added} two attention checks at probabilities of superiority of 50\% and 99.9\%, where the decision task should have been very easy, \jessica{to allow for filtering of participants who were not paying attention.}

\subsubsection{Generating Stimuli}
% \matt{this para could probably be a fair bit shorter (a lot of this is just describing arithmetic you had to do)} 
\jessica{can this section somehow be combined with another? it's pretty short}
\sout{In order} To create our stimuli, \sout{we made a set of assumptions about how the number of points scored by the fantasy sports team were distributed. 
We decided} \jessica{assumed} \textit{equal and independent variances} between the distributions with and without the new player \sout{should have}  $\sigma_{team}^2$ such that
$$\sigma_{diff}^2 = 2\sigma_{team}^2$$
where $\sigma_{diff}^2$ was the variance of the difference between distributions.
We \jessica{tested two levels of variance:} \sout{manipulated variance in distributions by} setting $\sigma_{diff}^2$ to a low value of 5 or a high value of 15. \jessica{These levels produced} \sout{, generating} distributions that looked narrow or wide relative to the width of the chart, \jessica{allowing us to achieve what}. 
We determined the distance between distributions, or mean difference $\mu_{diff}$, using the formula
$$\mu_{diff} = d\cdot\sigma_{diff}$$
where $d$ were ground truth values as standardized mean differences (i.e., Cohen’s d~\cite{Coe2002,Cummings2011}).
The mean number of points scored without the new player was held constant $\mu_{without} = 100$, which corresponds to a 50\% chance of winning the award. 
We calculated mean for the team with the new player $\mu_{with} = \mu_{without} + \mu_{diff}$. \jessica{Remind reader why we are doing all this}

\subsubsection{Experimental Design}
We assigned each user to one uncertainty visualization condition at random, making comparisons of uncertainty encodings between-subjects.
We asked users to make repeated judgments for two blocks of 16 trials each.
In one block, we showed the users visualizations with extrinsic means added, and in the other block there were no extrinsic means. 
We counterbalanced the order of these blocks across participants. 
Each of the 16 trials in a block showed a unique combination of ground truth effect size (8 levels) and variance of distributions (2 levels).
Thus, we manipulated ground truth effect size, level of variance, and whether or not means were added within-subjects.
The order of trials in each block was randomized. 
In the middle of each block, we inserted an attention check trial, such that users always saw the attention check at 50\% probability of superiority with means and saw the attention check at 99.9\% without means.
Including these attention checks, each participant completed 17 trials per block and 34 trials total.
% \jessica{I would reorder things in here to avoid leading with a weird number like 17 - first say we had them do repeated trials split into two blocks  where in each block, 16 trials showed .... In the middle of each block, we inserted ... This created a total of 17 trials per block ( 34 trials total)}

\subsubsection{Participants}
We recruited users through Amazon Mechanical Turk (MTurk).
Workers were located in the US and had a HIT acceptance rate of 97\% or more.
% \alex{Probably want a small table summarizing demographics}. \matt{I would leave that in the supplement? $P(\textit{anyone at vis cares about that}) \approx 0$}.
Based on the reliability of inferences from pilot data, we aimed to recruit 640 users to participate in our experiment after exclusions, 160 participants per visualization condition. 
We calculated this target sample size by assuming that variance in posterior parameter estimates would shrink by a factor of $\frac{1}{\sqrt{n}}$ if we collected a larger data set using the same interface.
Because we based our target sample size on between-subjects comparisons between visualization conditions, our estimates of within-subjects effects (e.g., adding means) were very precise. 
% \jessica{Consider noting in here that our estimates of within subjects effects are very precise since we chose our sample size to also enable relatively good estimates of the between subjects (vis condition) comparisons. } 

\subsubsection{Exclusions}
We recruited 879 participants.
After our preregistered exclusion criterion that users needed to pass both attention checks, we slightly exceeded our target sample size \sout{of} \jessica{with} 643 \jessica{total} participants.
However, we had issues fitting our model for an additional 21 participants, 17 of whom responded with only one or two levels of probability of superiority and 4 of whom had missing data.
Excluding these participants brought our final sample size to 622 (with block order still counterbalanced).
\jessica{So these were non-preregistered exclusions?}

\subsection{Modeling}
\subsubsection{Approach}
Using the brms package for R~\cite{Burkner2020}, we built Bayesian hierarchical models for each response variable, probability of superiority estimates and whether or not the user chooses to intervene. 
Our overall approach was to start with a simple model and add predictors gradually, checking the predictions of each model against the empirical distribution of the data.
This enabled us to compare the fit of increasingly complex models and understand the more complex models in terms of how they differ from the simpler ones \jessica{(i.e.,}  
\sout{We refer to this process as} \textit{model expansion}~\cite{Gabry2019}). 

Our approach \sout{to model expansion} involved starting with a \textit{minimal model}, which had the minimum set of predictors required to answer our research questions, and building toward a \textit{maximal model}, which included all the variables we manipulated in our experiment. 
We specified the minimal and maximal models for each response variable in our preregistration,~\footnote{https://osf.io/9kpmb} and we made our model building workflow transparent by walking through the model expansion process in R Markdown documents which are included in Supplemental Materials.~\footnote{https://github.com/kalealex/effect-size-jdm} \jessica{Awkward wording for that last part - somewhere in results section you can say all of our analyses are documented in supplemental. this is too much detail}

Expanding model specifications gradually helped us to determine priors one-at-a-time through a process of trial and error, as described in our preregistration. 
Each time we added a new kind of predictor to the model (e.g., a random intercept per participant), we honed in on weakly informative priors using prior predictive checks (i.e., visualizing model predictions implied by sampling from the joint distribution of priors)~\cite{Gabry2019}. 
% \matt{again, cite some stuff on prior predictive checks and whatnot. maybe check the Visualization in Bayesian Workflow paper?}
We centered the prior for each parameter on a value that reflected no bias in responses and scaled each prior to avoid predicting responses that were impossible on the response scale. 
As models became more complex, we figured out how narrow priors needed to be in order to guarantee enough regularization for a stable model fit.
Choosing priors by model expansion helped to mitigate difficulties with convergence of the Markov Chain Monte Carlo simulations used to fit Bayesian regression models. \jessica{maybe Matt has thoughts on whether this is too much detail. Seems like we could make more concise}

\subsubsection{Linear in Log Odds Model:}
\jessica{there is extra white space in this section that could be reduced around equations}
We use the following model (presented in Wilkinson-Pinheiro-Bates notation~\cite{Wilkinson1973,Burkner2020,Pinheiro2020}) to make inferences about responses in the probability of superiority estimation task:
% \matt{should make it clear that you are using lmer-style notation (Wilkinson-Pinheiro-Bates notation or whatever you call it, see here: https://stats.stackexchange.com/questions/284913/the-origin-of-the-wilkinson-style-notation-such-as-1id-for-random-effects-in). Should $estimate$ be $\mathrm{logit}(estimate)$? Also $ground\_truth$ and $estimate$ are somewhat ambiguous, especially given that there are two studies. These are the true and perceived probability of superiority right? Might find some pithy names that reflect that.}
\begin{flalign*}
\mathrm{logit}(response_{\Pr(S)}) \sim &\mathrm{Normal}(\mu, \sigma) \\
\mu = &(\mathrm{logit}(true_{\Pr(S)})*trial + means*var|worker) \\ 
    &+ \mathrm{logit}(true_{\Pr(S)})*means*var*vis*order \\
    &+ \mathrm{logit}(true_{\Pr(S)})*vis*trial \\
\mathrm{log}(\sigma) = &(\mathrm{logit}(true_{\Pr(S)}) + trial|worker) \\
    &+ \mathrm{logit}(true_{\Pr(S)})*vis*trial \\ 
    &+ means*order
\end{flalign*}
Where $response_{\Pr(S)}$ is the user's probability of superiority response, $true_{\Pr(S)}$ is the ground truth probability of superiority, $trial$ is an index of trial order, $means$ is an indicator for whether or not extrinsic means are present, $var$ is an indicator for low versus high variance, $vis$ is a dummy variable for uncertainty visualization condition, $order$ is an indicator for block order, and $worker$ is a unique identifier for each participant used to model random effects.
Note that there are submodels for the mean $\mu$ and standard deviation $\sigma$ of user responses.
Both $response_{\Pr(S)}$ and $true_{\Pr(S)}$ are transformed from probabilities of superiority into log odds, making this a linear in log odds (LLO) model.

\textbf{Motivation}:
We model effects on both $\mu$ and $\sigma$ because we noticed that the spread of the empirical distribution of responses varies as a function of the ground truth, visualization design, and trial order.
However, we are most interested in effects on mean response.
The term $\mathrm{logit}(true_{\Pr(S)})*means*var*vis*order$ tells our model that the slope of the LLO model varies as a joint function of whether or not means were added, the level of variance in distributions, uncertainty visualization condition, and block order (i.e., all of these factors are interacted with each other).
This enables us to answer our core research questions, while controlling for order effects.
The term $\mathrm{logit}(true_{\Pr(S)})*vis*trial$ models learning effects, so we isolate the impact of visualization condition.
The random effects terms in both submodels are the result of a process of model expansion %\matt{maybe say ``model expansion'' instead of ``trial and error'' here (and elsewhere), since you've already established that terminology anyway.} 
where we systematically attempted to incorporate as many within-subjects manipulations as possible without compromising model convergence (see Supplemental Materials).

\subsubsection{Logistic Regression}
We use this model to make inferences about intervention decisions: 
% \matt{functions and distributions are typically set in upright type, e.g. $\mathrm{Bernoulli}(p)$ and $\mathrm{logit}(p)$. I would also consider a more direct naming of the outcome variable than $decision$. Perhaps $intervene$?}
\begin{flalign*}
intervene \sim &\mathrm{Bernoulli}(p) \\
\mathrm{logit}(p) = &(evidence*means*var + evidence*trial|worker) \\
    &+ evidence*means*var*vis*order \\
    &+ evidence*vis*trial
\end{flalign*}
Where $intervene$ is the user's choice of whether or not to intervene, $p$ is the probability that they intervene, and $evidence$ is a transformation of the utility-optimal decision rule (see Formalizing Utility): %\matt{I wonder if this goes here or in "formalizing utility"? Also might be good to explain at this point (or wherever the definition of evidence is) \emph{why} logit-transforming it in this way makes sense: e.g., because it basically turns it into a log of an odds ratio for one versus the other where 0 is the decision cutoff and everything is on the real line (right?)}
$$evidence = \mathrm{logit}(\Pr(award|player)) - \mathrm{logit}(\Pr(award|\neg player) + \frac{1}{k})$$ 
This logit-transformation yields a scale which is perceptually uniform in theory~\cite{Gonzalez1999,Zhang2012,Varshney2013} and where zero represents the utility-optimal decision threshold.
All other factors are the same as in the LLO model (above).

\textbf{Motivation}:
The term $evidence*means*var*vis*order$ tells our model that the location and scale of the logistic curve vary as a joint function of whether or not means were added, the level of variance in distributions, uncertainty visualization condition, and block order.
Mirroring an analogous term in the LLO model, this enables us to answer our core research questions, while controlling for order effects.
The term $evidence*vis*trial$ models learning effects.
%\matt{``controls for'' is not great language I think... it carries baggage and tends to imply something more strong about causality in people's minds I think. Maybe ``models learning effects'' instead? Anyway I would try to remove ``controls for'' here and elsewhere}
As with the LLO model, we specify random effects per participant through model expansion by trying to incorporate as many within-subjects manipulations as possible.
In both the LLO model and logistic regression, random effects are limited by identifiability, (i.e., whether we have enough trials per manipulation per participant for the model to estimate random effects parameters per participant).
Adding random effects improves the fit of our models, however, we do not include them if doing so would require us to compromise on fixed effects which are more important for answering our research questions. 


\subsection{Derived Measures}
From our models, we derive estimates for three preregistered~\footnote{https://osf.io/9kpmb} metrics that we use to compare visualization designs.
% (1) In the linear log odds model, slopes measure perceptual bias in effect size estimates (Fig.~\ref{fig:llo_explainer}).
% In the logistic regression model, (2) just-noticable differences measure sensitivity to effect size information for the purpose of decision-making, and
% (3) points of subjective equality measure bias in decision-making (Fig.~\ref{fig:logistic_explainer}).
% Per our preregistration, we compare these metrics for each visualization condition, and for the interaction between the absence/presence of the mean and the level of variance. 
% To provide context for these comparisons, we also preregistered that we would present posterior predictions in the three-way interaction between means, variance, and visualization condition.
% \idl{I feel that the first paragraph of Section 4 should be in the methods section! You might want to elaborate on how you derive the estimates for the three metrics. For the slope of LLO model, you've already mention in Section 2. But for the other two metrics, I do not recall seeing background information (sorry if I missed anything) and have no idea what these refer to and how you derive them from the logit model.}

\textbf{Linear in log odds (LLO) slopes} measure the degree of bias in probability of superiority $\Pr(S)$ estimation (Fig.~\ref{fig:llo_explainer}).
A slope of one indicates unbiased performance, and slopes less than one indicate the degree to which users underestimate effect size.
We measure LLO slopes because they are especially sensitive to the expected pattern of bias in responses, giving us greater power to make statistical inferences than simpler measures like accuracy.
Specifically, LLO slope is the expected increase in a user's logit-transformed probability of superiority estimate $\mathrm{logit}(response_{\Pr(S)})$ for one unit of increase in logit-transformed ground truth $\mathrm{logit}(true_{\Pr(S)})$.
This provides a linear metric describing an exponential relationship.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/logistic_explainer-01.png}
    \setlength{\abovecaptionskip}{-10pt}
    \setlength{\belowcaptionskip}{-10pt}
    \caption{Logistic regression fit for one user. We derive PSE and JND by working backwards from probabilities of intervention to levels of evidence.
    }
    \label{fig:logistic_explainer}
\end{figure}

\textbf{Points of subjective equality (PSE)} measure bias toward or against choosing to intervene in the decision task relative to a utility-optimal and risk-neutral decision rule (see Formalizing Utility).
\jessica{PSEs} describe the level of evidence at which a user is expected to intervene 50\% of the time (Fig.~\ref{fig:logistic_explainer}). 
A PSE of zero is utility-optimal, whereas negative values indicate that users intervene when there is not enough evidence to warrant doing so, and positive values indicate that users intervene too little.
\jessica{could omit next sentence} PSE enables us to measure decision quality against a normative standard.
We calculate PSE as $\frac{-intercept}{slope}$ where $slope$ and $intercept$ come from the logit-transformed linear model within logistic regression.

\textbf{Just noticeable-differences (JNDs)} 
measure sensitivity to effect size information for the purpose of decision-making (Fig.~\ref{fig:logistic_explainer}). 
They describe how much additional evidence for the effectiveness of an intervention a user needs to see in order to increase their rate of intervening from 50\% to about 75\%.
A JND in evidence units is a difference in the log probability of winning the award with the new player.
We chose this scale for statistical inference because units of log stimulus intensity are thought to be approximately perceptually uniform~\cite{Stevens1957,Varshney2013}.
We calculate JND as $\frac{\mathrm{logit}(0.75)}{slope}$ where $slope$ is the same as for PSE.


\subsection{Qualitative Analysis of Strategies}
\jessica{Using the two strategy responses we elicited from each user,} we \sout{wanted to} \jessica{conducted a qualitative analysis to} characterize user's visual reasoning strategies in terms of what heuristics they used in each visualization condition, whether they payed attention to means, and whether they switched strategies.
\sout{We elicited two strategy responses from each user, one at the end of each block of trials (i.e., with and without means added).}

The first author developed a bottom-up open coding scheme for how users described their reasoning with the charts.
Since some responses were uninformative about what visual properties of the chart a user considered (e.g., \textit{``I used the charts to estimate the value added by the new player.''}), we omitted participants for whom both responses were uninformative from further analysis.
Excluding 180 such participants resulted in a final sample of 442 for our qualitative analysis.

We used our open codes to develop a classification scheme for strategies based on whether users mentioned:
Switching strategies;
Judging distance between graphic elements;
Relying on or ignoring means;
Using variance as cue, ignoring variance, or erroneously preferring a high or low level of variance;
Using a real or imagined threshold on the x-axis scale as a reference;
Relying on the area or extent of geometries;
Counting or judging frequencies of graphical markings (applicable to quantile dotplots and HOPs);
or Being confused about the task or charts.
Thus, we generated a spreadsheet of quotes, open codes, and categorical distinctions which enabled us to provide aggregate descriptions of patterns and heterogeneity in user strategies.

==> archived/drafts/method-submission.tex <==
\section{Method}
We tested how adding means to different uncertainty visualizations impacts users’ ability to estimate effect size and make incentivized decisions based on effect size.
\alex{Maybe move some content from 3.3 to here to make what follows more concrete.}
We asked users to estimate a measure of effect size called \textit{probability of superiority} or common language effect size~\cite{McGraw1992}, the percent of the time that expected outcomes for one group $A$ exceed expected outcomes for another group $B$.
Probability of superiority is a proxy for standardized mean difference $\frac{\mu_A - \mu_B}{\sigma_{A-B}}$~\cite{Coe2002,Cummings2011}, the difference between two group means relative to uncertainty about the difference between means.
Using synthetic data, we evaluated bias in effect size estimates compared to a known ground truth.

\alex{In this paragraph, we are saying why we did what we did before we describe what we did.}
We devised our decision task to represent a \textit{class of decision problems} where one faces an all-or-nothing probabilistic outcome and has the option of paying for an intervention that changes the probability of that outcome. 
This class of problems includes medical decisions about treatments that may save someone’s life or cure them of a disease, organizational decisions about hiring personnel to reach a contract deadline, and personal decisions such as paying for education to seek a promotion.
We set up the incentives of our task so that above a certain level of effect size a risk-neutral user should pay for intervention, and below that effect size they should not pay.
In our decision task, users judged the same information as in the estimation task, and we evaluated their intervention decisions compared to a utility-optimal standard.

% \jessica{organization in this section could use a major revision - I don't think we're giving enough of the intuition behind the visualization conditions experimental design, overall framing of task, and framework for evaluating decisions early enough to give the reader grounding for making sense of all these details. Check out the Fernandes et al CHI 2018 bus paper - there are parallels where we could set up the overall design and procedure, then talk about the fictional scenario, perhaps the visualizations/conditions, then the utility framework, then model, then participant details (some things may need to change slightly, but I think the general flow would be a lot easier to follow) Things like sampling ground truth, generating stimuli should come after you've laid out the overall design and procedure, framing/scenario, etc. }


\subsection{Experimental Design \& Procedure}
We assigned each user to one of four uncertainty visualization conditions at random, making comparisons of uncertainty visualizations between-subjects.
On each trial, users made a probability of superiority estimate and an intervention decision.
We asked users to make repeated judgments for two blocks of 16 trials each.
In one block, we showed the users visualizations with means added, and in the other block there were no means. 
We counterbalanced the order of these blocks across participants. 
Each of the 16 trials in a block showed a unique combination of ground truth effect size (8 levels) and variance of distributions (2 levels), making our manipulations of ground truth, variance, and adding means all within-subjects.
The order of trials in each block was randomized. 
In the middle of each block, we inserted an attention check trial, later used to filter participants who did not attend to the task. Users always saw an attention check at 50\% probability of superiority with means and at 99.9\% without means.
Hence, each participant completed 17 trials per block and 34 trials total. 
% \jessica{watch the wordiness! I imagine you could recover at least 10 lines, probably more from eliminating verbosity.}


\subsection{Uncertainty Visualization Conditions}
% \jessica{have you mentioned yet whether vis conditions are between participants or not? seems important context for reader as they read about conditions}
We evaluated visualizations intended to span a design space characterized by the visual salience of the mean, expressiveness of uncertainty representation, and discrete versus continuous encodings of probability. 
As described above, we showed four uncertainty visualization formats---intervals, hypothetical outcome plots (HOPs), density plots, and quantile dotplots---with and without separate (i.e., extrinsic) vertical lines encoding the mean of each distribution.
We expected that adding means would bias effect size estimates toward discounting uncertainty and that this effect would be most pronounced for uncertainty visualizations in which the mean is \textit{not} intrinsically salient. 

\textbf{Intervals:}
We showed users intervals representing a range containing 95\% of the possible outcomes (Fig.~\ref{fig:teaser}, left column). 
In the absence of a separate mark for the mean, the mean was not intrinsically encoded, and the user could only find the mean by estimating the midpoint of the interval.
% While the middle of the interval implicitly encoded the mean, this uncertainty encoding did not make the mean intrinsically salient. \jessica{you mean without mean added? Maybe say, We chose to test intervals because in the absence of a separate mark for the mean, the mean is not intrinsically encoded, and intervals are not very expressive .. ,}
Intervals were not very expressive of probability density since they only encoded lower and upper bounds on a distribution. 
% Numerous studies have shown that intervals are not the most effective uncertainty encoding~\cite{Correll2014,Hullman2015,Kale2019-hops} and that laypeople and scientists alike struggle to interpret them~\cite{Belia2005,Soyer2012,Hoekstra2014,Hofman2020}, yet they remain very common. \jessica{Don't we say this in related work}

\textbf{Hypothetical Outcome Plots (HOPs):}
We showed users animated sequences of strips representing 20 quantiles sampled from a distribution of possible outcomes (Fig.~\ref{fig:teaser}, left center column), matching the data shown in quantile dotplots.
Animations were rendered at \textit{2.5 frames per second with no animated transitions} (i.e., tweening or fading) between frames, looping every 8 seconds. 
We shuffled the two distributions of 20 quantiles using a 2-dimensional quasi-random Sobol sequence~\cite{Sobol1976} to minimize the apparent correlation between distributions.
Like intervals, HOPs did not make the mean intrinsically salient, as means were implicitly encoded as the average position of an ensemble of strips shown over time.
However, HOPs were more expressive of the underlying distribution than intervals and expressed uncertainty as frequencies of events, so they conveyed an experience-based sense of probability. 

\textbf{Densities:} 
We showed users continuous probability densities where the height of the area marking encoded the probabilities of corresponding possible outcomes on the \textit{x}-axis (Fig.~\ref{fig:teaser}, right center column).
Unlike intervals and HOPs, the mean was explicitly represented as the point of maximum mark height because distributions were symmetrical, so means were intrinsically salient.
Densities were also the most expressive of the underlying probability density function among the uncertainty visualizations we tested.
% \sout{, prior work found that users interpret probability density more accurately when it is discretized, i.e., quantile dotplots~\cite{Kay2016,Fernandes2018}. Thus, the expressiveness of densities may not translate into effective use. }

\textbf{Quantile Dotplots:}
We showed users dotplots where each of 20 dots represented a 5\% chance of a corresponding possible outcome on the \textit{x}-axis (Fig.~\ref{fig:teaser}, right column).
Like densities, because distributions were symmetrical and dots were stacked in bins to express this symmetry, the mean was explicitly represented as the point of maximum height and was thus intrinsically salient. 
% \jessica{My edits in here are aimed at 1) using more similar language between sections and 2) making clear the continuums we are talking about in intro to section}


\subsection{Task Scenario \& Interface}
\alex{Move this description of the task into the overview.}
We set up our task as a fantasy sports game where participants decided whether or not to pay to add new players to their team. 
On each trial, we showed participants a chart comparing the predicted number of points scored by their team with a new player added versus without a new player (e.g., Fig.~\ref{fig:distance_strategy}). 
\alex{Merge this description of the questions and elicitation with the paragraph above where we first explain probability of superiority.}
We asked users to estimate the probability that the team would score more points with a new player than without (i.e., probability of superiority~\cite{McGraw1992}). 
Then we asked them whether or not they wanted to pay to add the new player to their team. 

\textbf{Elicitation:}
We elicited effect size judgments based on a large body of prior work on statistical reasoning (e.g.,~\cite{Gigerenzer1995,Hoffrage1998}) suggesting that people reason with probabilities more accurately when they are framed as frequencies.
\alex{Give reasons for approach to elicitation after saying what the question was.}
We asked for probability of superiority judgments as text entry responses to the question, \textit{``How many times out of 100 do you estimate that your team would score more points with the new player than without the new player?''}
\alex{Make separate paragraphs for estimation and decision questions, mirroring overview.}
We elicited intervention decisions using radio buttons indicating that the user would either \textit{``Pay for the new player,''} or \textit{``Keep [their] team without the new player.''}

\textbf{Feedback:}
\alex{Describe feedback more concisely as a Monte Carlo simulation.}
At the end of each trial we told users whether or not their team scored enough points to win an award.
We generated this feedback by simulating an outcome based on whether or not the user chose to pay for a new player. 
Feedback consisted of two tables, one showing how the user's account value changed on this trial, and the other showing their current total account value and how this translated into a cumulative bonus they would earn in real money. 
% \jessica{is expected bonus cumulative bonus they are guaranteed at that point, or expectation of bonus conditional on continuing to perform that way (its ambiguous)}
Emphasizing probabilistic outcomes, rather than the expected value of decisions, made this feedback a noisy signal for how well participants were doing, mirroring real-world learning conditions for decisions under uncertainty. 

\textbf{User Strategies:}
To supplement our quantitative measures with qualitative descriptions of users' visual reasoning, at the end of each of the two block of trials, we asked users, \textit{``How did you use the charts to complete the task? Please do your best to describe what sorts of visual properties you looked for and how you used them.''}

\textbf{Incentives for Decisions:}
\alex{Borrow language from here when giving an initial description of the decision task.}
The incentives in our decision task mirror real-world decisions with all-or-nothing payouts. The participant's goal was framed as winning awards worth \$3.17M each.

We instructed participants that to maximize the value of their fantasy sports account, they should pay \$1M to add a player to their team if they thought the new player improved their chances of winning enough to be worth the cost. 
On each trial, there were four possible payouts:
\begin{enumerate}[noitemsep,nolistsep]
    \item The participant won without paying for a new player (+\$3.17M).
    \item The participant paid for a new player and won (+\$2.17M).
    \item They failed to win without paying for a new player (\$0).
    \item The participant paid for a new player and failed to win (-\$1M). 
\end{enumerate}
The user could only lose money if they paid for the new player.\footnote{In pilot studies, we tested how framing outcomes as winning versus losing awards impacted user behavior and found that participants had greater preference for intervention when it was described as increasing the certainty of gains, consistent with prior work by Tversky and Kahneman~\cite{Kahneman1979,Tversky1981}.}

Optimally, participants should have paid to add a new player only when effect size was larger than 74\% probability of superiority or Cohen’s d of 0.9, the average effect size in a recent survey of studies in experimental psychology~\cite{Schafer2019}.
\alex{Payout information in a separate paragraph.}
Participants received a \textit{guaranteed base compensation of \$1 plus a bonus} of $\$0.08\cdot(account - \$150M)$, where \$0.08 per \$1M was the exchange rate from account value to real dollars, $account$ was the value of their fantasy sports account at the end of the experiment, and \$150M was a cutoff account value below which they receive no bonus. 
These values were carefully chosen to result in bonuses between \$0 and \$3, such that participants who guessed randomly and experienced unlucky probabilistic outcomes would receive no bonus, and participants who responded optimally would be guaranteed a bonus.


\subsection{Evaluating Utility of Decisions}
\alex{Merge some content from this first paragraph into the overview when motivating the decision task.}
We devised our decision task so that we could define utility-optimal performance for a risk-neutral observer, giving us a normative benchmark against which we could measure bias in decision-making. 
Comparing behavior to a risk-neutral benchmark is a common practice in judgment and decision-making studies~\cite{Baron2008}, used to measure risk preferences~\cite{Weber1994} or attitudes making a person more or less inclined to take action than they should be based on a cost-benefit analysis.
Whether or not a user should decide to intervene depends on both the amount of money they stand to win or lose---specifically, value of an award and the cost of a new player---and the effect size (i.e., the difference in team performance with versus without a new player).  
\alex{This next sentence is redundant with the more formal description of fixing baseline probability below. Omit.}
\sout{Because we fixed the probability of winning an award \textit{without} a new player at 50\% (i.e., a coin flip), effect size corresponded to the probability of winning an award \textit{with} a new player.}
\alex{Be sure that we unpack what we mean by ``class of decision problem'' in the overview. Probably start this section with the following sentence.}
We formalized the class of problem represented by our task using a normative decision rule based on maximizing expected utility~\cite{vonNeumann1944}, which we used to analyze the quality of users' decisions. 

Let $v$ be the value of an award.
Let $c$ be the cost of adding a new player to the team. 
The utility-optimal decision rule is to intervene if
\begingroup
\setlength\abovedisplayskip{3pt}
\setlength\belowdisplayskip{3pt}
    $$v \cdot \Pr(award|\neg player) < v \cdot \Pr(award|player) - c$$
\endgroup
where $\Pr(award|\neg player)$ is the probability of winning an award \textit{without} a new player, and $\Pr(award|player)$ is the probability of winning an award \textit{with} a new player.
Assuming a constant ratio between the value of the award and the cost of intervention $k = \frac{v}{c}$, we express the decision rule in terms of the difference between the probabilities of winning an award with versus without a new player: 
\begingroup
\setlength\abovedisplayskip{2pt}
\setlength\belowdisplayskip{2pt}
    $$\Pr(award|\neg player) + \frac{1}{k} < \Pr(award|player)$$
\endgroup

The threshold level of effect size above which one should intervene depends on the incentive ratio $k$ and the probability of a payout without intervention $\Pr(award|\neg player)$.
In our study, we fixed the incentives $k = 3.17$ and the probability of winning an award without a new player $\Pr(award|\neg player) = 0.5$ so that users would not have to keep track of changing incentives and effect size alone was the signal that users should base decision on.\footnote{In pilot studies, we tried manipulating $k$ and $\Pr(award|\neg player)$ and found that these changes had little impact on the effectiveness of different uncertainty visualizations for supporting utility-optimal decision-making. In light of prior work showing that Mechanical Turk workers do not respond to changes of incentives~\cite{Stoycheff2016}, we suspect that these manipulations might have an impact in real-world settings which is difficult to measure on crowdsourcing platforms.}
This enabled a controlled evaluation of how users translate visualized effect size into a sense of utility.
% \jessica{give some intuition for the fixing of incentives, many readers might not understand implications of this versus alternative}


\subsection{Generating Stimuli}
We generated synthetic data covering a range of effect size such there were an equal number of trials where users should and should not intervene.
Recall that 50\% corresponded to a new player who did not improve the team’s performance at all, 100\% corresponded to a definite improvement in performance, and 74\% was the utility-optimal decision threshold.
% We sample levels of ground truth probability of superiority ranging between 55\% and 95\%, inclusive. 
% Half of the values we sampled fell above the utility-optimal decision threshold of about 74\% and half of them fell below. 
% This guaranteed that each user would see an equal number of trials where they should pay for the new player as where they shouldn’t pay. 
We sampled eight distinct levels of ground truth probability of superiority, four values between 55\% and 74\% and four values between 74\% and 95\%, such that there are an equal number of trials above and below the utility-optimal decision threshold.
Prior work in perceptual psychology~\cite{Gonzalez1999,Zhang2012} suggests that the brain represents probability on a log odds scale.
For this reason, we converted probabilities into log odds units and sampled on this logit-transformed scale using linear interpolation between the endpoints of the two ranges described above. 
We added two attention checks at probabilities of superiority of 50\% and 99.9\%, where the decision task should have been very easy, to allow for excluding participants who were not paying attention.

To derive the visualized distributions from ground truth effect size, we made a set of assumptions.
We assumed \textit{equal and independent variances} for the distributions with and without a new player $\sigma_{team}^2$ such that $\sigma_{diff}^2 = 2\sigma_{team}^2$ 
where $\sigma_{diff}^2$ was the variance of the difference between distributions.
We tested two levels of variance, setting the standard deviation of the difference between distributions $\sigma_{diff}$ to a low value of 5 or a high value of 15. 
These levels produced distributions that looked relatively narrow or wide compared to the width of the chart, making visual distance between distributions an unreliable cue for effect size such that at low variance large effect sizes corresponded to distributions that were close together.

We determined the distance between distributions, or mean difference $\mu_{diff}$, using the formula $\mu_{diff} = d\cdot\sigma_{diff}$
where $d$ were ground truth values as standardized mean differences (i.e., Cohen’s d~\cite{Coe2002,Cummings2011}).
The mean number of points scored without the new player was held constant $\mu_{without} = 100$, which corresponded to a 50\% chance of winning the award. 
We calculated mean for the team with a new player $\mu_{with} = \mu_{without} + \mu_{diff}$.
We rendered our chart stimuli using the parameters $\mu_{with}$, $\mu_{without}$, and $\sigma_{team}$ to define the two distributions on each chart.
% \jessica{Remind reader why we are doing all this}
Holding the chance of winning without a new player constant at 50\% (Fig.~\ref{fig:distance_strategy}, blue distributions) is an experimental control that enables us to compare a user's preference for new players across trials using a coin flip gamble as the alternative choice, which is common in judgment and decision-making studies~\cite{Baron2008}.  
% \jessica{these constraints simplify the user's task, might want to motivate why this is good}


\subsection{Modeling}
We wanted to measure how much users underestimate effect size in their probability of superiority responses, how much they deviate from a utility-optimal criterion in their decisions, and how sensitive they are to effect size for the purpose of decision-making.
To measure underestimation bias, we fit a linear in log odds model~\cite{Gonzalez1999,Zhang2012} to probability of superiority responses, and we derive \textit{slopes} describing users' responses as a function of the ground truth (Fig.~\ref{fig:llo_explainer}).
To measure bias and sensitivity to effect size in decision-making, we fit a logistic regression to intervention decisions, and we derive \textit{points of subjective equality} and \textit{just-noticeable differences} describing the location and scale of the logistic curve as functions of effect size (Fig.~\ref{fig:logistic_explainer}). 
% Following prior work~\cite{Gonzalez1999,Zhang2012}, both models assume that the user's internal representation of probabilities (i.e., probability of superiority and probability of winning) are on a log odds scale.

\subsubsection{Approach}
We used the brms package~\cite{Burkner2020} in R to build Bayesian hierarchical models for each response variable: probability of superiority estimates and decisions of whether or not to intervene. 
We started with simple models and gradually added predictors, checking the predictions of each model against the empirical distribution of the data.
This process of \textit{model expansion}~\cite{Gabry2019} enabled us to understand the more complex models in terms of how they differ from simpler ones. 

We started with a \textit{minimal model}, which had the minimum set of predictors required to answer our research questions, and built toward a \textit{maximal model}, which included all the variables we manipulated in our experiment. 
We specified the minimal and maximal models for each response variable in our preregistration.\footnote{
We include an anonymized preregistration in Supplemental Materials for review. There is a version with author names on OSF.
% https://osf.io/9kpmb
} 

Expanding models gradually helped us determine priors one-at-a-time. 
Each time we added a new kind of predictor to the model (e.g., a random intercept per participant), we honed in on weakly informative priors using prior predictive checks~\cite{Gabry2019}.
% (i.e., visualizing model predictions implied by sampling from the joint distribution of priors)
We centered the prior for each parameter on a value that reflected no bias in responses.
We scaled each prior to avoid predicting impossible responses and to impose enough regularization to avoid issues with convergence in model fitting. 
We documented priors and model expansion in Supplemental Materials.\footnote{
[Github URL redacted for review]
% https://github.com/kalealex/effect-size-jdm
}

\subsubsection{Linear in Log Odds Model:}
% \jessica{there is extra white space in this section that could be reduced around equations}
We use the following model (Wilkinson-Pinheiro-Bates notation~\cite{Wilkinson1973,Burkner2020,Pinheiro2020}) for responses in the probability of superiority estimation task: 
% \matt{put group effects last in each submodel?}
\begingroup
\setlength\abovedisplayskip{3pt}
\setlength\belowdisplayskip{3pt}
    \begin{flalign*}
    \setlength\abovedisplayskip{0pt}
    \setlength\belowdisplayskip{0pt}
    \mathrm{logit}(response_{\Pr(S)}) \sim &\mathrm{Normal}(\mu, \sigma) \\[-2pt]
    \mu = &\mathrm{logit}(true_{\Pr(S)})*means*var*vis*order \\[-2pt]
        +& \mathrm{logit}(true_{\Pr(S)})*vis*trial \\[-2pt] 
        +& \big(\mathrm{logit}(true_{\Pr(S)})*trial + means*var\big|worker\big) \\[-2pt]
    \mathrm{log}(\sigma) =         &\mathrm{logit}(true_{\Pr(S)})*vis*trial \\[-2pt] 
        +& means*order \\[-2pt]
        +& \big(\mathrm{logit}(true_{\Pr(S)}) + trial\big|worker\big)
    \end{flalign*}
\endgroup
% \jessica{I would reduce space between lines slighly}
% \jessica{Pr(S) seems like slightly weird notation, like treating superiority as an event?} \alex{Probability of superiority as an event makes sense given how we elicited the judgment: ``How many times out of 100?''}
Where $response_{\Pr(S)}$ is the user's probability of superiority response, $true_{\Pr(S)}$ is the ground truth probability of superiority, $trial$ is an index of trial order, $means$ is an indicator for whether or not extrinsic means are present, $var$ is an indicator for low versus high variance, $vis$ is a dummy variable for uncertainty visualization condition, $order$ is an indicator for block order, and $worker$ is a unique identifier for each participant used to model random effects.
Note that there are submodels for the mean $\mu$ and standard deviation $\sigma$ of user responses.

\textbf{Motivation}:
We apply a logit-transformation to both $response_{\Pr(S)}$ and $true_{\Pr(S)}$, changing units from probabilities of superiority into log odds, because prior work suggests that the perception of probability should be modeled as linear in log odds (LLO)~\cite{Gonzalez1999,Zhang2012}.
% \jessica{shouldn't we motivate the log transform here?}
We model effects on both $\mu$ and $\sigma$ because we noticed in pilot studies that the spread of the empirical distribution of responses varies as a function of the ground truth, visualization design, and trial order.
However, we are most interested in effects on mean response.
The term $\mathrm{logit}(true_{\Pr(S)})*means*var*vis*order$ tells our model that the slope of the LLO model varies as a joint function of whether or not means were added, the level of variance, uncertainty visualization, and block order (i.e., all of these factors interacted with each other).
This enables us to answer our core research questions, while controlling for order effects.
The term $\mathrm{logit}(true_{\Pr(S)})*vis*trial$ models learning effects, so we isolate the impact of uncertainty visualizations.
In both submodels, we added within-subjects manipulations as random effects predictors as much as possible without compromising model convergence.
% The random effects terms in both submodels are the result of a process of model expansion where we systematically attempted to incorporate as many within-subjects manipulations as possible without compromising model convergence (see Supplemental Materials).

\subsubsection{Logistic Regression}
We use this model to make inferences about intervention decisions: 
% \matt{functions and distributions are typically set in upright type, e.g. $\mathrm{Bernoulli}(p)$ and $\mathrm{logit}(p)$. I would also consider a more direct naming of the outcome variable than $decision$. Perhaps $intervene$?}
\begingroup
\setlength\abovedisplayskip{3pt}
\setlength\belowdisplayskip{3pt}
    \begin{flalign*}
    intervene \sim &\mathrm{Bernoulli}(p) \\[-2pt]
    \mathrm{logit}(p) = &evidence*means*var*vis*order \\[-2pt]
        +& evidence*vis*trial \\[-2pt]
        +&\big(evidence*means*var + evidence*trial\big|worker\big)
    \end{flalign*}
\endgroup
Where $intervene$ is the user's choice of whether or not to intervene, $p$ is the probability that they intervene, and $evidence$ is a logit-transformation of the utility-optimal decision rule (see Section 3.4):
\begingroup
\setlength\abovedisplayskip{2pt}
\setlength\belowdisplayskip{2pt}
    $$evidence = \mathrm{logit}(\Pr(award|player)) - \mathrm{logit}(\Pr(award|\neg player) + \frac{1}{k})$$
\endgroup
This gives us a uniformly sampled scale of evidence where zero represents the utility-optimal decision threshold.
All other factors are the same as in the LLO model (see Section 3.6.2).

\textbf{Motivation}:
We logit-transform our evidence scale because internal representations of probabilities are thought to be on a log odds scale~\cite{Gonzalez1999,Zhang2012}, such that linear changes in log odds appear similar in magnitude.
% This evidence scale is perceptually uniform in theory~\cite{Gonzalez1999,Zhang2012,Varshney2013}. \jessica{unpack perceptually uniform in theory (especially the in theory part, what should the reader get from that statement?)} 
The term $evidence*means*var*vis*order$ tells our model that the location and scale of the logistic curve vary as a joint function of whether or not means were added, the level of variance, uncertainty visualization, and block order.
Mirroring an analogous term in the LLO model, this enables us to answer our core research questions, while controlling for order effects.
The term $evidence*vis*trial$ models learning effects.
As with the LLO model, we specify random effects per participant through model expansion by trying to incorporate as many within-subjects manipulations as possible.
% In both the LLO model and logistic regression, random effects are limited by identifiability, (i.e., whether we have enough trials per manipulation per participant for the model to estimate random effects parameters per participant).
% Adding random effects improves the fit of our models, however, we do not include them if doing so would require us to compromise on fixed effects which are more important for answering our research questions. 


\subsection{Derived Measures}
From our models, we derive estimates for three preregistered metrics that we use to compare visualization designs. 
% \jessica{reading the first part of this section, I felt like I was lacking an understanding of the measures we care about. Can we motivate these at least in a sentence or two earlier in section, at least in terms of what broad types of things we hope to learn, if not the specific measures? Without an idea of what measures we care about the model specs are hard to care about, it reads like a bunch of minute details without much context}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/llo_explainer-04.png}
    % \setlength{\intextsep}{-20pt}
    \setlength{\abovecaptionskip}{-10pt}
    \setlength{\belowcaptionskip}{-10pt}
    \caption{Linear in log odds (LLO) model: fits for average user of quantile dotplots and intervals compared to a range of possible slopes (top); predictive distribution and observed responses for one user (bottom).
    }
    \label{fig:llo_explainer}
\end{figure}

\begin{figure}[b]
    \vspace{-2mm}
    \centering
    \includegraphics[width=\columnwidth]{figures/logistic_explainer-01.png}
    % \setlength{\intextsep}{-20pt}
    \setlength{\abovecaptionskip}{-10pt}
    \setlength{\belowcaptionskip}{-10pt}
    \caption{Logistic regression fit for one user. We derive point of subjective equality (PSE) and just-noticeable difference (JND) by working backwards from probabilities of intervention to levels of evidence.
    }
    \label{fig:logistic_explainer}
\end{figure}


\textbf{Linear in log odds (LLO) slopes} measure the degree of bias in probability of superiority $\Pr(S)$ estimation (Fig.~\ref{fig:llo_explainer}).
A slope of one indicates unbiased performance, and slopes less than one indicate the degree to which users underestimate effect size.\footnote{LLO slopes less than one represent bias toward the probability at the intercept, $\mathrm{logit^{-1}}(intercept)$, which is close to $\Pr(S) = 0.5$ in our study.}
We measure LLO slopes because they are very sensitive to the expected pattern of bias in responses, giving us greater statistical power than simpler measures like accuracy.
Specifically, LLO slope is the expected increase in a user's logit-transformed probability of superiority estimate, $\mathrm{logit}(response_{\Pr(S)})$, for one unit of increase in logit-transformed ground truth, $\mathrm{logit}(true_{\Pr(S)})$.
Using a linear metric (i.e., slope in logit-logit space) to describe an exponential response function in probability units comes from a theory that the brain represents probabilities on a log odds scale~\cite{Gonzalez1999,Zhang2012}.
The LLO model~\cite{Gonzalez1999,Zhang2012} can be thought of as a generalization of the cyclical power model~\cite{Hollands2000} that allows a varying intercept or a modification of Stevens' power law~\cite{Stevens1957} for proportions.
% We can think of the LLO model~\cite{Gonzalez1999,Zhang2012} as a modification of Steven's power law~\cite{Stevens1957} to handle proportions or as a special case  of the cyclical power model~\cite{Hollands2000} with reference probabilities of 0\% and 100\% \matt{I would more say that LLO can be thought of as a *generalization* (not special case) of the cyclical power model that allows the intercept to vary, where the cyclical power model is itself based on Stevens' power law (also note Stevens' not Steven's)}.

\textbf{Points of subjective equality (PSEs)} measure bias toward or against choosing to intervene in the decision task relative to a utility-optimal and risk-neutral decision rule (see Section 3.4).
PSEs describe the level of evidence at which a user is expected to intervene 50\% of the time (Fig.~\ref{fig:logistic_explainer}). 
A PSE of zero is utility-optimal, whereas a negative value indicates that a user intervenes when there is not enough evidence, and a positive value indicates that a user doesn't intervene until there is more than enough evidence. 
In our model, PSE is $\frac{-intercept}{slope}$ where $slope$ and $intercept$ come from the linear model in logistic regression.

\textbf{Just noticeable-differences (JNDs)} 
measure sensitivity to effect size information for the purpose of decision-making (Fig.~\ref{fig:logistic_explainer}). 
They describe how much additional evidence for the effectiveness of an intervention a user needs to see in order to increase their rate of intervening from 50\% to about 75\%.
A JND in evidence units is a difference in the log probability of winning the award with the new player.
We chose this scale for statistical inference because units of log stimulus intensity are thought to be approximately perceptually uniform~\cite{Stevens1957,Varshney2013}.
In our model, JND is $\frac{\mathrm{logit}(0.75)}{slope}$ where $slope$ is the same as for PSE. 
% \matt{again I'd say "In our model," instead of "We calculate"}

% \vbox{
\subsection{Participants}
We recruited users through Amazon Mechanical Turk.
Workers were located in the US and had a HIT acceptance rate of 97\% or more.
Based on the reliability of inferences from pilot data, we aimed to recruit 640 participants, 160 per uncertainty visualization.
We calculated this target sample size by assuming that variance in posterior parameter estimates would shrink by a factor of roughly $\frac{1}{\sqrt{n}}$ if we collected a larger data set using the same interface.
Since we based our target sample size on between-subjects effects (e.g., uncertainty visualization), our estimates of within-subjects effects (e.g., adding means) were very precise.

We recruited 879 participants.
After our preregistered exclusion criterion that users needed to pass both attention checks, we slightly exceeded our target sample size with 643 total participants.
However, we had issues fitting our model for an additional 21 participants, 17 of whom responded with only one or two levels of probability of superiority and 4 of whom had missing data.
After these non-preregistered exclusions, our final sample size was 622 (with block order counterbalanced). 
All participants were paid regardless of exclusions, on average receiving \$2.24 and taking 16 minutes to complete the experiment.

\subsection{Qualitative Analysis of Strategies}
Using the two strategy responses we elicited from each user, we conducted a qualitative analysis to characterize users' visual reasoning strategies based on heuristics they used with different visualization designs (with and without means) and whether they switched strategies.

The first author developed a bottom-up open coding scheme for how users described their reasoning with the charts.
Since some responses were uninformative about what visual properties of the chart a user considered (e.g., \textit{``I used the charts to estimate the value added by the new player.''}), we omitted participants for whom both responses were uninformative from further analysis.
Excluding 180 such participants resulted in a final sample of 442 for our qualitative analysis.

We used our open codes to develop a classification scheme for strategies based on what visual features of charts users mention, whether they switched strategies, and whether they were confused by the chart or task.
We coded for the following uses of visual features:
\begin{itemize}[noitemsep,nolistsep]
    \item \textbf{Relative position} of distributions
    \item \textbf{Means}, whether users relied on or ignored them
    \item \textbf{Spread} of distributions, whether users relied on variance, ignored it, or erroneously preferred high or low variance
    \item \textbf{Reference lines}, whether users relied on imagined or real vertical lines (e.g., the annotated decision threshold in Fig.~\ref{fig:teaser} \&~\ref{fig:distance_strategy})
    \item \textbf{Area}, whether users relied on the spatial extent of geometries
    \item \textbf{Frequencies}, whether users of quantile dotplots or HOPs relied on frequencies of dots or animated draws
\end{itemize}
Thus, we generated a spreadsheet of quotes, open codes, and categorical distinctions which enabled us to provide aggregate descriptions of patterns and heterogeneity in user strategies.
% }

% \begin{itemize}
%     \vspace*{-5pt}\item \textbf{Relative position} of distributions
%     \vspace*{-5pt}\item \textbf{Means}, whether users relied on or ignored them
%     \vspace*{-5pt}\item \textbf{Spread} of distributions, whether users relied on variance, ignored it, or erroneously preferred high or low variance
%     \vspace*{-5pt}\item \textbf{Reference lines}, whether users relied on imagined or real vertical lines (e.g., the annotated decision threshold)
%     \vspace*{-5pt}\item \textbf{Area}, whether users relied on the spatial extent of geometries
%     \vspace*{-5pt}\item \textbf{Frequencies}, whether users of quantile dotplots or HOPs relied on frequencies of dots or animated draws
% \end{itemize}
% \vspace*{-5pt} Thus, we generated a spreadsheet of quotes, open codes, and categorical distinctions which enabled us to provide aggregate descriptions of patterns and heterogeneity in user strategies.


==> archived/drafts/results-draft1.tex <==
\section{Results}
From our models, we derive estimates for three preregistered~\footnote{https://osf.io/9kpmb} metrics.
(1) In the linear log odds model, slopes  measure perceptual bias in effect size estimates (Fig.~\ref{fig:llo_explainer}).
In the logistic regression model, (2) just-noticable differences measure sensitivity to effect size information for the purpose of decision-making, and
(3) points of subjective equality measure bias in decision-making (Fig.~\ref{fig:logistic_explainer}).
Per our preregistration, we compare these metrics for each visualization condition, and for the interaction between the absence/presence of the mean and the level of variance. 
To provide context for these comparisons, we also preregistered that we would present posterior predictions in the three-way interaction between means, variance, and visualization condition.
% \matt{dunno where, but might be good to have at least one figure with the data in it if that's possible. Might be able to integrate the data into one of the other figures. It might also make the stuff about slopes easier to understand since readers could see it directly on a plot of the data. E.g. an explainer figure that shows some people's raw data with fits on them, annotates the slope, links to a vis of estimates of the slopes, etc...}
\idl{I feel that the first paragraph of Section 4 should be in the methods section! You might want to elaborate on how you derive the estimates for the three metrics. For the slope of LLO model, you've already mention in Section 2. But for the other
two metrics, I do not recall seeing background information (sorry if I missed anything) and have no idea what these refer to and how you derive them from the logit model.}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/logistic_explainer-01.png}
    \caption{Logistic regression model fit for one user. We derive PSE and JND in evidence units by working backwards from probabilities of intervention to levels of evidence.
    }
    \label{fig:logistic_explainer}
\end{figure}

\subsection{Probability of Superiority Judgments}
We report impacts of visualization design on probability of superiority judgments in terms of slopes in the linear in log odds (LLO) model, which measure bias in perceived effect size.
A slope of one indicates unbiased performance, and slopes less than one indicate the degree to which users underestimate effect size.
We preregistered comparisons in terms of LLO slopes because they are especially sensitive to the expected pattern of bias in responses.
However, because the LLO model measures a linear relationship between responses and ground truth on a logit-transformed scale, differences in LLO slopes correspond to \textit{non-linear} differences in predicted response error. 
While LLO slopes give us statistical power, they are difficult to interpret directly,
% we caution that they should not be interpreted directly. \jessica{is there even a way to interpret directly? I doubt readers would even try, so maybe we should say, 'While they give us statistical power they are difficult to interpret directly' instead.}
so we contextualize each result in terms of predicted error.

\begin{figure*}[ht]
    \centering
    \includegraphics[width=\textwidth]{figures/llo_slopes-03.png}
    \caption{Effects of evaluated visualization designs on linear in log odds (LLO) model slopes.
    \idl{As you talk about the right column first in the text, perhaps you could make it the left column as we read from left to right ... I like how you label x-axis with an arrow indicating underestimation bias, but perhaps you could add another label to indicate that the numbers on the x-axis correspond to slopes in the LLO model. Also, the horizontal chart placement makes it difficult to compare low variance with high variance. Have you considered stacking all subplots vertically?}
    }
    \label{fig:llo_slopes}
\end{figure*}

\subsubsection{Perceptual Bias per Visualization Condition}
Users in all uncertainty visualization conditions we tested show a tendency to underestimate effect size (Fig. ~\ref{fig:llo_slopes}, right column).
Quantile dotplots have LLO slopes reliably closer to one ($\mu$: 0.565; 95\% CI: [0.502,  0.630]), indicating less bias than all other visualization conditions, followed by densities ($\mu$: 0.434; 95\% CI: [0.370, 0.496]), HOPs ($\mu$:0.394; 95\% CI: [0.327, 0.461]), and intervals ($\mu$: 0.351; 95\% CI: [0.288, 0.414]), respectively.
% \matt{results are hard to skim as the estimates and intervals run together visually. maybe put brackets around the intervals?}
These LLO slopes correspond to posterior predictions that quantile dotplot users underestimate the true probability of superiority by about 9 percentage points, whereas users of densities, HOPs, and intervals underestimate the ground truth by 12, 14, and 15 percentage points, respectively. 
% \matt{do these have intervals associated with them? are these marginal effects or effects at a particular value? Also I now definitely think we need a plot here showing raw data (or at least fit lines / curves) and how slope and error relate --- it's very abstract.} \alex{These percentage point numbers are just the average error in posterior predictions corresponding to each of the slope estimates listed above. These aren't the values we are using for reliability testing. They are just a way of contextualizing the slope values. Do you think we should report CIs alongside these means? The issue is that LLO slopes are a more sensitive measure (i.e., lower signal-to-noise), but the posterior predictions are better for interpretation. I'm trying to split the difference by reporting both.}

\textbf{Discussion:}
% \alex{Talk about why visualization conditions might be different in terms of choices in study and stimulus design: cognitive load of two tasks may have disadvantaged HOPs users even though HOPs show exactly the information they need to answer both questions; holding the x-axis limits constant across all stimuli is necessary to investigate the impact of the hypothesis that distance is a perceptual proxy for effect size, however, this means that individual charts have unrealisitc amounts of white space particularly at low variance, which may have exacerbated the degree of underestimation in all conditions compared to naturalistic conditions (doesn't undermine comparisons between conditions since this applies to all stimuli).}
The fact that users of quantile dotplots show the least bias on average is not completely surprising considering previous work (e.g.,~\cite{Gigerenzer1995,Hoffrage1998,Kay2016}) showing that frequency-based visualizations are especially effective at conveying probabilities.
However, quantile dotplots are optimized to show cumulative probabilities for a single distribution~\cite{Kay2016}, not necessarily for comparisons between two distributions.
Similar to intervals and densities, users should not be able to decode the ground truth directly by comparing two quantile dotplots, unless the distributions completely overlap or they rely on statistical theory to calculate effect size given the means and variances they are shown.
\idl{Are you trying to argue why quantile dotplots show the least bias but still have a slope less than 1? Could you make it explicit?}
% \jessica{maybe say what you have to do to do the two dist comparison with them correctly?} \alex{I'm actually not even sure what the ``right'' strategy would be. I'm planning to talk about how people are using them in the Stategies section: Counting red dots above threshold (cumulative probability above the average of the other distribution); or Counting the number of red dots which do not overlap with the range of the blue distribution (as a proxy for an overall difference in probability density).} \jessica{makes sense, but i think its safe to say that you can't get the right answer directly from the plot unless in the case where the distributions are identical or they are non overlapping - otherwise you have to rely on statistical theory (And know that the variables are independent and normal) - you would have to basically compute normal distribution function using your estimate of the plotted mean difference divided by the sums of your estimates of the variances of each group }

In contrast, HOPs directly encode probability of superiority by how often the draws from the two distributions change order. 
% \jessica{I would start the new paragraph before this sentence so its all about hops}
We find it surprizing that HOPs users do not perform reliably differently from users of intervals or densities.
Our results are \textit{inconsistent} with some findings from previous  repeated-measures and within-subjects experiments showing that HOPs are more perceptually effective than violin plots and error bars~\cite{Hullman2015,Kale2019-hops}.
However, our results are \textit{consistent} with a large between-subjects experiment where HOPs users perform on par with users of error bars showing a 95\% predictive interval~\cite{hofman2020}.  
One plausible explanation for these contradictory results is that our task may have imposed a high cognitive load, leading users to rely on heuristics.
Our experiment requires users to give responses on two tasks per trial with repeated measures and multiple within-subjects manipulations.
The decision task requires users to reason about an incentive structure where the optimal decision criterion is not immediately obvious.
We speculate that the attentional demands of our experiment may reduce the tendency for participants to think of HOPs in terms of frequencies of events, leading to suboptimal performance.

Given that the optimal visual reasoning strategies for our task are unclear with every visualization condition but HOPs, yet HOPs users perform somewhat poorly, the descriptive evidence of heuristics that users employ under different visualization conditions, which we present below, provides context that can help us understand these results.

% In some real-world circumstances, axes scales on charts are not optimized for the data in an individual chart.
% For example, this is the case when designers facet small multiples, generate forest plots showing multiple distributions on one axis, or follow the axiom that the axis on bar charts should always include zero.
% In our task, we hold the x-axis limits constant in order to investigate our hypothesis that distance is a perceptual proxy for effect size.
% However, this design choice may exacerbate the tendency to underestimate effect size.
% Charts depicting small effect sizes or comparing distributions with low variances have more white space than a visualization designer would usually include in an individual chart.
% In agreement with prior work~\cite{Witt2019,Hofman2020}, we think that the tendency to underestimate effect size may change depending on design choices about axis scale. 
% However, since we applied the same axis scale to all stimuli in all conditions, this limitation does not impact comparisons between visualization conditions in our study.

\subsubsection{Perceptual Bias Induced by the Mean}
We see reliable but very small effects on perceptual bias when adding means to uncertainty visualizations.
When charts show distributions with low variances on the same axis scale as charts showing high variances, adding means to distributions with low variances decreases LLO slopes by 0.032 on average (95\% CI: [-0.044, -0.020]), averaging over visualization conditions (Fig.~\ref{fig:llo_slopes}, left column, bottom row). 
For context, this corresponds to an increase in magnitude estimation error of about 1 percentage point on the probability of superiority scale.

Across levels of variance, the effect of adding means to HOPs is similar (\ref{fig:llo_slopes}, left and center columns, third line).
If we average over variance conditions (not shown), adding means to HOPs reduces LLO slopes by -0.041 (95\% CI: [-0.068,	-0.014]) on average. 
However, because user performance with HOPs is relatively biased without means, and because changes in LLO slope correspond to non-linear changes in predicted error, this difference only increases underestimation error by about 0.1 percentage points on the probability of superiority scale. 
While this effect is reliable and visible in Figure~\ref{fig:llo_slopes}, it is not of practical importance.
% \jessica{this effect is so small we need to emphasize this in first sentence. I question whether we should be referring to this as an effect} \matt{yeah i'd be curious to see an interval on this --- are we talking "close enough to 0 not to care" level of effect size? especially if it's precise that makes this a null effect we can talk about, which even sort of strengthens the result. Either way I wouldn't use "exacerbate" to describe it} \alex{I'm mainly noting this because it is the only case where adding means has the same effect regardless of the level of variance. Something distinct is happening with HOPs users when means are added. Whether or not it is practically important in the aggregate, I think this might be linked heterogeneous strategies and lots of switching among HOPs users.}

If we average over visualization conditions, the impact of adding means at high variance is ambiguous (Fig.~\ref{fig:llo_slopes}, center column, bottom row) because this effect changes directions under different conditions. 
At high variance, adding means increases LLO slopes on average by 0.045 (95\% CI: [0.025, 0.064]) for intervals and 0.041 (95\% CI: [0.016, 0.066]) for densities (Fig.~\ref{fig:llo_slopes}, center column, second and fourth lines).
Although this change in LLO slopes is similar to the HOPs condition, the reduction in predicted error in probability of superiority judgments is about 1.5 percentage points for intervals and 1.1 percentage point for densities.
These are the only cases were adding means reduces perceptual bias (i.e, increases slopes).

\textbf{Discussion:}
Based on our results, adding means to uncertainty visualizations seems unhelpful for users making effect size judgments under most conditions, but it doesn't seem too harmful either.
Adding means lead to changes in performance which are practically negligible in comparison to the impact of different uncertainty encodings.

While we do not want to overstate the importance of this effect, adding means to uncertainty visualizations induces a pattern of behavior consistent with what we expected from the outset of the study:
When variance in distributions is relatively low, users tend to underestimate effect size \textit{more} when means are present;
When variance in distributions is high, users tend to underestimate effect size \textit{less} when means are present, at least for intervals and densities (Fig.~\ref{fig:llo_slopes}, center column, second and fourth lines). 
% \matt{you're talking about an interaction here that you haven't shown estimates of yet (unless I missed it)} \alex{Estimates for the effect of means for intervals and densities are presented in the paragraph immediately before this discussion. Also, shown in the figure.}
This reversal of the effect of extrinsic means depending on the level of variance is consistent with users employing a heuristic where the distance between distributions is used as a proxy for effect size.
To the extent that users pay attention to the mean difference between distributions and underweight uncertainty information, they should err systematically in effect size judgments in approximately the observed pattern.
\idl{I don't understand this paragraph at all ... why should you expect a reversal of the effect when the variance is high?} \alex{That this is not coming through is not good. By trying to simplify the introduction, we may have cut too much about the specific anticipated pattern of behavior. Not sure where to add it back in...}

% \idl{Similar to my previous comment, I feel that the result section should describe the results with the current experimental setup and the limitation/discussion section should discuss how experimental design choices might affect the results.}
% In designing the stimuli for our study there is a trade-off between making means the same size for each visualization condition and balancing the salience of the mean in each condition.
% We also consider realism insofar as we attempt not to make charts that seem unnaturally out-of-proportion (i.e., ridiculously large means).
% However, the resulting stimuli probably vary in the salience of extrinsic means, with the lines encoding the mean being less salient for densities and quantile dotplots than for intervals and HOPs.
% This may contribute to differences in the effect of adding means on LLO slopes for different uncertainty visualization conditions.


\subsection{Intervention Decisions}
We report impacts of visualization design on decision quality in terms of two metrics derived from our logistic regression model: just-noticeable differences (JNDs) and points of subjective equality (PSE).
\idl{Could you make a plot/table for the effect sizes and CIs? Readers might want to compare the results before they decide whether to agree with you interpretation, but currently the numbers are embedded in your narrative ...} \alex{This suggestion kind of runs counter to our overall approach to presenting results. What do you think, Matt and Jessica?}

\subsubsection{Just-Noticeable Differences} 
JNDs describe a user's sensitivity to effect size information for the purpose of making decisions. 
Specifically, they measure how much additional evidence for the effectiveness of an intervention a user needs to see in order to increase their rate of intervening from 50\% to about 75\%.
The level of evidence in favor of intervention in our task is a monotonically increasing function of effect size.
A JND on this evidence scale describes a difference in the log probability of winning the award with the new player.
We chose this scale for statistical inference because units of log stimulus intensity are thought to be approximately perceptually uniform~\cite{Stevens1957,Varshney2013}.
However, since these units are difficult to interpret directly, we provide context by translating these effects into changes in the probability of winning the award with the new player.
As a rule of thumb, smaller JNDs indicate that a user is sensitive to smaller differences in effect size for the purpose of decision-making.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/jnd-01.png}
    \caption{Effects of evaluated visualization designs on just-noticeable differences (JNDs) in the decision task.}
    \label{fig:jnd}
\end{figure}

When we average over factors other than visualization (Fig.~\ref{fig:jnd}), quantile dotplot users have a smaller JNDs (i.e., greater sensitivity) than users in any other visualization condition ($\mu$: 0.431; 95\% CI: [0.387, 0.482]), followed by densities ($\mu$: 0.505; 95\% CI: [0.451,	0.567]), intervals ($\mu$: 0.521; 95\% CI: [0.459, 0.596]), and HOPs ($\mu$: 0.591; 95\% CI: [0.518, 0.683]). 
These JNDs mean that the average user of quantile dotplots requires the probability of winning with the new player to change by about 5.6 percentage points in order to go from intervening 50\% of the time to 75\%, whereas the average user of densities, intervals, and HOPs require changes in probability of about 6.3, 6.4, and 7.2 percentage points, respectively.

We also examine the interaction effect of adding means and level of variance in each visualization condition on JNDs. 
% \alex{not clear to me what the figure should be here since these findings are not super important/interesting}
Adding means to uncertainty visualizations only seems to have a reliable effect for intervals at high variance, where means reduce JNDs by 0.100 on average (95\%: [-0.161,	-0.044]).
This corresponds to a 1.2 percentage point reduction in terms of the probability of winning.
Otherwise, we don't see much of an impact of adding means on JNDs.

However, we see a reliable impact of the level of variance on JNDs.
JNDs are smaller by an average of 0.222 evidence units (95\% CI: [-0.275, -0.175]) when variance is high than when variance is low.
This corresponds to a 2.2 percentage point reduction in terms of the probability of winning.

\textbf{Discussion:}
The effects on JNDs that we report are small enough that they may not be of much practical importance.
For example, the difference in JNDs between quantile dotplots and HOPs---the largest pairwise difference in JNDs between uncertainty visualizations---is 1.6 percentage points in term of the probability of winning. 
This is slightly greater than the impact of adding means to intervals at high variance.
% Unless the specific use case involves showing users an effect size which is \textit{very} close to a decision threshold---above which the user should intervene and below which they should not---visualization designers should probably not base their choice of encodings on these small discrepancies in JNDs. 
The reduction in JNDs between low and high variance is slightly larger, indicating that at high variance users in our task are sensitive to probabilities of winning that are 2.2 percentage points smaller.
We may see an effect of variance because charts in the high variance condition use more space to convey effect size compared to the low variance charts, which have more white space.
This explanation is consistent with the idea that visual distance is a proxy for effect size, and it suggests that \textit{the way visualization designers use white space has an impact the perceived signal in a chart}. \idl{From the beginning of reading this paper, I also suspect the effect of the white space. Most of visualization tools fit the scales based on the domain range of the given data. Thus, the high variance case and the low variance case can be look the same in the real world.}


\subsubsection{Points of Subjective Equality} 
PSE describe users’ bias toward or against choosing to intervene in the decision task relative to a utility-optimal decision strategy.
Specifically, they measure the level of evidence at which a user sees intervening versus not intervening as having equal utility (i.e., the level of evidence at which they intervene 50\% of the time). 
A PSE of zero is utility-optimal, whereas negative values indicate that users intervene when there is not enough evidence to warrant doing so, and positive values indicate that users intervene too little.
Although we present inferential statistics on PSE in log-likelihood units of evidence, we contextualize these effects by translating how far off users are from the utility-optimal decision rule into units of the probability of winning the award.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/pse-11.png}
    \caption{Effects of evaluated visualization designs on points of subjective equality (PSE) in the decision task.}
    \label{fig:pse}
\end{figure}

When we average over factors other than visualization (Fig.~\ref{fig:pse}, right column), intervals are the only uncertainty visualization condition where the average user's PSE is not reliably different from zero ($\mu$: -0.067; 95\% CI: [-0.207, 0.088]). 
For HOPs ($\mu$: -0.198; 95\% CI: [-0.351, -0.028]), densities ($\mu$: -0.280; 95\% CI: [-0.396, -0.157]), and quantile dotplots ($\mu$: -0.337; 95\% CI: [-0.438, -0.228]), respectively, the average user shows increasing levels of bias toward intervening too often.
% Intervals reliably outperform quantile dotplots and densities (but not HOPs) on this metric. 
On average, users of intervals intervene when the probability of winning the award with the new player is 2.3 percentage points below the utility-optimal decision threshold, whereas bias on this scale is 4.6, 5.2, and 6.1 percentage points for users of HOPs, densities, quantile dotplots, respectively.

The interaction effects of adding means and level of variance on PSE in each visualization condition are fairly nuanced (Fig.~\ref{fig:pse}, left and center columns).
Adding means at high variance reliably reduces PSE for intervals ($\mu$: -0.159; 95\% CI: [-0.278, -0.038]) and densities ($\mu$: -0.126; 95\% CI: [-0.247, -0.005]), resulting in biases toward intervening of 3.2 and 2.6 percentage points, respectively, in terms of the probability of winning.
Quantile dotplots are the only condition where the average user is biased toward intervention at both high and low variance.
This means that when extrinsic means are added to quantile dotplots at low variance, they have a uniquely debiasing impact on PSE ($\mu$: 0.256; 95\% CI: [0.091, 0.435]), changing the average user's bias from 3.5 percentage points below the utility-optimal threshold to 0.5 percentage points above and thus eliminating bias toward intervention.
While these highly specific effects stand out as interesting, other effects in this three-way interaction are not reliable and are similarly complex.

When we marginalize across visualization conditions (Fig.~\ref{fig:pse}, bottom row), an overall effect of adding means at high versus low variance becomes clear: \textit{Adding extrinsic means consistently biases PSE away from the utility-optimal decision threshold}.
At \text{high variance} and without means, the average user has a negative PSE ($\mu$: -0.536;	95\% CI: [-0.598, -0.475]), indicating bias toward intervention 9.5 percentage points below the utility-optimal threshold in terms of the probability of winning.
Adding means exacerbates this bias in PSE ($\mu$: -0.106; 95\% CI: [-0.174, -0.039]) by about 2.2 percentage points.
Conversely, at \textit{low variance} and without means, the average user may have a slightly positive PSE ($\mu$: 0.072; 95\% CI: [-0.034, 0.184]), indicating bias against intervention 0.7 percentage points above the utility-optimal threshold.
Similar to the high variance case, adding extrinsic means exacerbates bias in PSE ($\mu$: 0.153; 95\% CI: [0.030, 0.282]) by about 1.7 percentage points.

In Figure~\ref{fig:pse} (left and center columns, top row), we can see that different visualization conditions might lead to the least bias depending on the level of variance.
At \textit{high variance and without means}, intervals lead to the least bias on average ($\mu$: -0.416; 95\% CI: [-0.539, -0.293]), with PSE slightly less biased than quantile dotplots ($\mu$: -0.572; 95\% CI: [-0.673, -0.469]) and HOPs ($\mu$: -0.628; 95\% CI: [-0.759, -0.499]), but not reliably less biased than densities ($\mu$: -0.529; 95\% CI: [-0.642, -0.417]). 
These PSE indicate biases to intervene at probabilities of winning 7.1, 9.3, 10, and 11 percentage points below the utility-optimal threshold for intervals, densities, quantile dotplots, and HOPs, respectively. 
\textit{This suggests that intervals or densities---both without means---make the best decision aids when showing distributions with a single level of variance.}

At \textit{low variance and without means}, densities lead to the least bias on average ($\mu$: -0.030; 95\% CI: [-0.187, 0.134]), with PSE less biased than HOPs ($\mu$: 0.235; 95\% CI: [0.010, 0.494]) and intervals ($\mu$: 0.291; 95\% CI: [0.080, 0.541]), but not reliably less biased than quantile dotplots ($\mu$: -0.209; 95\% CI: [-0.352,	-0.053]).
Note that the direction of bias is \textit{against} intervention for HOPs and intervals, where the average users' PSE are 3.0 and 3.7 percentage points \textit{above} the utility-optimal decision threshold, respectively.
Whereas for densities and quantile dotplots, the direction of bias is \textit{toward} intervention such that the average users' PSE are 0.6 and 3.5 percentage points \textit{below} the utility-optimal decision threshold, respectively.
Thus, \textit{densities without means make the best decision aids when showing distributions with different levels of variance on a common axis}.

\textbf{Discussion}
When we marginalize across factors other than visualization condition, intervals lead to the least biased decision-making. \matt{this is a weird marginalization to judge effectiveness on since you can't draw an interval that is the average of having and not having a mean?} \alex{This was a comparison that we preregistered to look at visualization effectiveness. However, I make the point you are raising in the next paragraph. Would you approach this discussion of effectiveness differently?}
However, this is fairly counterintuitive in that we do not expect degrading the expressiveness of uncertainty encodings to be helpful for decision-making. 
Consider the fact that, based on our results, quantile dotplots seem best suited to probability of superiority judgments and intervals seem worst.
However, when we model decision-quality in terms of PSE, visualization rankings based on average bias reverse such that intervals are best and quantile dotplots are worst.
This seems to suggest that \textit{perceptual effectiveness does not necessarily feed forward into better decision-making} and that visualization researchers should do more to try to understand how information processing is different for decision-making than for estimation.
% should consider magnitude estimation and decision tasks separately. \jessica{not sure about this last piece of advice - it seems non ideal to have to think of them separately since they obviously should be related. maybe we just say researchers should be doing more to try to understand the relationship}
 
Note that while the average user of intervals is less biased the average user of densities when we average over adding means and level of variance, densities without means appear to be as good or better than intervals without means when we look at levels of variance separately.
We think of this as a manifestation of Simpson's Paradox~\alex{cite?}, where the apparent effect depends on how we aggregate model predictions.
We argue that whenever details about the data to be visualized (e.g., levels of variance) are available, designers should incorporate this information into their design choices, rather than always choosing the visual encoding which is most effective when averaging over contextual factors.
% We argue that it is more appropriate to reason about design recommendations in terms of specific visualization designs (e.g., densities/intervals without means) under specific circumstances (e.g., at high/low variance), rather than reasoning about visual forms in the abstract (e.g., bias for densities/intervals after adjusting for manipulations of design and circumstance). \jessica{Here I would also put this a bit differently - if someone is designing a visualization tool that should accomodate any levels of variance, then variance specific suggestions aren't very useful unless they already have detailed information on the distribution over variance levels. I would say this more like, We argue that whenever detailed information about factors like expected variance levels are available, designers should use them.}
Our work demonstrates an approach to experimental design and behavioral modeling capable of separating out and disambiguating these considerations, which we hope will be adopted by future researchers to provide such detailed recommendations.
% The ability to separate out and disambiguate these considerations demonstrates the strengths of our approach to experimental design and behavioral modeling. \jessica{might restate this last part as, 'Our work demonstrates an approach to experimental design and behavioral modeling capable of separating out and disambiguating these considerations, which we hope will be adopted by future researchers to provide such detailed recommendations.'}

While the impact of the mean on decision quality is small, our findings support a more-or-less categorical claim that \textit{means are unhelpful for promoting utility-optimal decisions}.
The one exception in our results is that for quantile dotplots at low variance, adding means reduces bias in decision-making. 
However, our results suggests that densities without means promote similarly unbiased decision-making at low variance.
In realistic use cases where distributions with heterogeneous variances are displayed on a common axis (e.g., forest plots showing multiple estimates on a single scale~\cite{Freiman1978}), designers should prefer to use a consistent uncertainty encoding which supports unbiased decision-making across levels of variance. 
% \jessica{Heterogenous variance is being mentioned bc of the way we scaled axes right? makes sense then to also mention the other realistic circumstance where you have axes scaled independently of the variance in each group like to include 0}
We find that \textit{densities without means promote decisions with the least bias across levels of variance}.

==> archived/drafts/results-draft2.tex <==
\section{Results}
\idl{This section is like a massive wall of text. I know its kind of inevitable when reporting experimental results, but any way to cut this down / make it more readable? Maybe report all the numbers in a table so that you can only comment on the interesting stuff in the text?}
\subsection{Probability of Superiority Judgments}
We report impacts of visualization design on probability of superiority judgments in terms of slopes in the linear in log odds (LLO) model, \sout{which} measuring bias in perceived effect size.
\jessica{Recall that} a slope of one indicates unbiased performance, and slopes less than one indicate the degree to which users underestimate effect size.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/llo_slopes-04.png}
    \setlength{\abovecaptionskip}{-10pt}
    \setlength{\belowcaptionskip}{-10pt}
    \caption{Effects of evaluated visualization designs on linear in log odds (LLO) model slopes.
    \idl{What does ``increases slope'' or ``decreases slope'' mean here? Maybe add to the caption how to interpret the changing slope of the model.}
    }
    \label{fig:llo_slopes}
\end{figure}

We examine the interaction effect on LLO slopes of adding means to each uncertainty visualization condition at low and high variance.
For every uncertainty encoding, adding means at low variance decreases LLO slopes (Fig.~\ref{fig:llo_slopes}, first row).
When we average over visualization conditions, adding means at low variance changes LLO slopes by -0.031 (95\% CI: [-0.044, -0.020]) for the average user (Fig.~\ref{fig:llo_slopes}, second row). 
This corresponds to an increase in magnitude estimation error of about 0.8 percentage points on the probability of superiority scale.
If we similarly average over visualization conditions, the impact of adding means at high variance is ambiguous (Fig.~\ref{fig:llo_slopes}, fourth row) because this effect changes directions for different uncertainty encodings. 
At high variance (Fig.~\ref{fig:llo_slopes}, third row), adding means increases LLO slopes for intervals ($\mu$: 0.045; 95\% CI: [0.024, 0.064]) and densities ($\mu$: 0.039; 95\% CI: [0.014, 0.063]), whereas adding means decreases LLO slopes for HOPs ($\mu$: -0.038; 95\% CI: [-0.071, -0.004]). 
Although these effects seem similar in magnitude, differences in LLO slopes represent changes in the exponent of a power law relationship.
Consequently, the reduction in predicted error for probability of superiority judgments is about 1.5 and 1.0 percentage points for intervals and densities, respectively, whereas the increase in predicted error is 0.3 percentage points for HOPs. \jessica{I would add 'small' or 'very small' in front of one of these mentions of effects since some readers may skim through these numeric heavy paragraphs} 

Users show a tendency to underestimate effect size on our task regardless of visualization design (Fig. ~\ref{fig:llo_slopes}).
When we average over factors other than visualization condition (not shown), LLO slopes are reliably closer to one with quantile dotplots ($\mu$: 0.566; 95\% CI: [0.503,	0.631]) than with densities ($\mu$: 0.436; 95\% CI: [0.372, 0.499]), HOPs ($\mu$: 0.394; 95\% CI: [0.329, 0.460]), and intervals ($\mu$: 0.350; 95\% CI: [0.289, 0.413]) in order of increasing bias.
These LLO slopes correspond to average predicted errors in probability of superiority judgments of 8.9 percentage points for quantile dotplots and 12.4, 14.0, and 14.6 percentage points for users of densities, HOPs, and intervals, respectively. 

\textbf{Discussion:}
Adding means to uncertainty visualizations \jessica{does not appear to help} \sout{seems unhelpful for} users make effect size judgments under most conditions, but it does not \jessica{appear to harm them} \sout{seem too harmful} either.
% Adding means lead to changes in performance which are practically negligible in comparison to the impact of different uncertainty encodings.
While we do not want to overstate the practical importance of this \jessica{small} effect, adding means to uncertainty visualizations induces a pattern of behavior consistent with relying on visual distance between distributions as a proxy for effect size:
When variance in distributions is relatively low, users tend to underestimate effect size \textit{more} when means are present (Fig.~\ref{fig:llo_slopes}, second row); \jessica{should we qualify relatively low, like relative to what}
When variance in distributions is high, users tend to underestimate effect size \textit{less} when means are present, at least for intervals and densities (Fig.~\ref{fig:llo_slopes}, third row). 
% This reversal of the effect of extrinsic means depending on the level of variance is consistent with users employing a heuristic where the distance between distributions is used as a proxy for effect size.
% To the extent that users pay attention to the mean difference between distributions and underweight uncertainty information, they should err systematically in effect size judgments in approximately the observed pattern.
% \idl{I don't understand this paragraph at all ... why should you expect a reversal of the effect when the variance is high?} \alex{That this is not coming through is not good. By trying to simplify the introduction, we may have cut too much about the specific anticipated pattern of behavior. Not sure where to add it back in...}
\jessica{the capitals after : in the previous sentence seem weird to me, is that grammatically correct?}
This is the behavioral signature of the visual distance heuristic that we identified at the outset of the study.

Among the uncertainty encodings we tested, users of quantile dotplots show the least bias on average.
This is not surprising considering previous work (e.g.,~\cite{Gigerenzer1995,Hoffrage1998,Kay2016}) showing that frequency-based visualizations are effective at conveying probabilities.
However, quantile dotplots are optimized to show cumulative probabilities for a single distribution~\cite{Kay2016}, not for comparisons between two distributions.
Similarly with intervals and densities, users should not be able to decode the ground truth directly by comparing two distributions unless the distributions completely overlap, or they rely on statistical theory to calculate effect size analytically from visualized means and variances.

In contrast, HOPs directly encode probability of superiority by how often the draws from the two distributions change order. 
We find it surprising that HOPs users do not perform reliably differently from users of intervals or densities.
Our results are inconsistent with some findings from previous
% repeated-measures and within-subjects 
experiments showing that HOPs are more perceptually effective than violin plots and error bars~\cite{Hullman2015,Kale2019-hops}.
However, our results are \textit{consistent} with
% a large between-subjects 
an
experiment where HOPs users perform on par with users of error bars showing a 95\% predictive interval~\cite{Hofman2020}.
% One plausible explanation for these contradictory results is that our task may have imposed a high cognitive load, leading users to rely on heuristics.
% Our experiment requires users to give responses on two tasks per trial with repeated measures and multiple within-subjects manipulations.
% The decision task requires users to reason about an incentive structure where the optimal decision criterion is not immediately obvious.
% We speculate that the attentional demands of our experiment may reduce the tendency for participants to think of HOPs in terms of frequencies of events, leading to suboptimal performance.
One plausible explanation for these contradictory results are differences in cognitive load between experiments.
Both experiments where HOPs users perform poorly involve incentivized decisions, which require users to reason about an incentive structure where the optimal decision rule is not obvious.
Additionally, our study involved two tasks and multiple within-subjects manipulations.
We speculate that the attentional demands of our experiment may lead HOPs users to rely on suboptimal heuristics, rather than reasoning about frequencies of events.

Given that the optimal visual reasoning strategies for our task are unclear with every visualization condition but HOPs, yet HOPs users perform somewhat poorly, the descriptive evidence of heuristics that users employ under different visualization conditions, which we present \jessica{in Section X} \sout{below}, provides context that can help us understand these results.


\subsection{Intervention Decisions}
We report impacts of visualization design on decision quality in terms of two metrics derived from our logistic regression model: points of subjective equality (PSE) and just-noticeable differences (JNDs).

\subsubsection{Points of Subjective Equality} 
\jessica{Recall that} PSE describes the amount of evidence at which a user sees intervening versus not intervening as having equal utility.
A PSE of zero is utility-optimal, negative PSE indicates intervening too often, and positive PSE indicates not intervening enough.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/pse-11.png}
    \setlength{\abovecaptionskip}{-10pt}
    \setlength{\belowcaptionskip}{-10pt}
    \caption{Effects of evaluated visualization designs on points of subjective equality (PSE) in the decision task.}
    \label{fig:pse}
\end{figure}

The interaction effects on PSE of adding means to each uncertainty visualization condition at low and high variance are fairly nuanced (Fig.~\ref{fig:pse}, first and third rows).
Adding means at high variance reliably reduces PSE for intervals ($\mu$:-0.160; 95\% CI: [-0.277, -0.040]) and maybe for densities ($\mu$:-0.11646489; 95\% CI: [-0.238, 0.002]), resulting in biases toward intervening of 3.2 and 2.4 percentage points, respectively, in terms of the probability of winning.
Quantile dotplots are the only condition where the average user is biased toward intervention at both high and low variance.
This means that when extrinsic means are added to quantile dotplots at low variance, they have a uniquely debiasing impact on PSE ($\mu$:0.252; 95\% CI:	[0.082,	0.435]), changing the average user's bias from 3.6 percentage points below the utility-optimal threshold to 0.3 percentage points above and thus eliminating bias toward intervention.
While these effects stand out as interesting, \jessica{raises question, were they chosen because interesting or because more reliable} other effects in this three-way interaction are not reliable and are similarly complex. \jessica{This paragraph is hard to get much from - too many subtle points to thread together}

When we average over visualization conditions (Fig.~\ref{fig:pse}, second and fourth rows), we see a clear overall effect of adding means at low versus high variance: \jessica{the word versus makes me expect some different effect depending on variance level} \textit{Adding extrinsic means consistently biases PSE away from the utility-optimal decision rule}.
At \textit{low variance} and without means, the average user may have a slightly positive PSE ($\mu$: 0.075; 95\% CI: [-0.034, 0.197]), indicating bias against intervention 0.6 percentage points above the utility-optimal PSE.
Adding means increases this mild bias in PSE ($\mu$: 0.150; 95\% CI: [0.027, 0.281]) by about 1.7 percentage points.
Conversely, at \text{high variance} and without means, the average user has a negative PSE ($\mu$: -0.538;	95\% CI: [-0.599, -0.476]), indicating bias toward intervention 8.3 percentage points below the utility-optimal rule in terms of the probability of winning.
Similar to the low variance case, adding means exacerbates this bias in PSE ($\mu$: -0.105; 95\% CI: [-0.175, -0.036]) by about 2.1 percentage points.

In Figure~\ref{fig:pse} (first and third rows), we \sout{can} see that different visualization designs \sout{lead to} \jessica{result in} the least bias depending on the level of variance.
At \textit{low variance and without means}, densities lead to the least bias on average ($\mu$: -0.033; 95\% CI: [-0.188, 0.127]), with PSE less biased than HOPs ($\mu$: 0.255; 95\% CI: [0.021, 0.531]) and intervals ($\mu$: 0.292; 95\% CI: [0.077, 0.548]), but not quite reliably less biased than quantile dotplots ($\mu$: -0.213; 95\% CI: [-0.360, -0.064]).
Note that the direction of bias is \textit{against} intervention for HOPs and intervals, where the average users' PSE are 3.2 and 3.5 percentage points \textit{above} the utility-optimal decision threshold, respectively.
Whereas for densities and quantile dotplots, the direction of bias is \textit{toward} intervention such that the average users' PSE are 0.6 and 3.6 percentage points \textit{below} the utility-optimal decision threshold, respectively.
% Thus, \textit{densities without means make the best decision aids when showing distributions with different levels of variance on a common axis}.
At \textit{high variance and without means}, intervals lead to the least bias on average ($\mu$: -0.423; 95\% CI: [-0.541, -0.302]), with PSE slightly less biased than HOPs ($\mu$:-0.625; 95\% CI:	[-0.759, -0.496]), maybe less biased that quantile dotplots ($\mu$:-0.5727111; 95\% CI: [-0.676, -0.470]), but not reliably less biased than densities ($\mu$:-0.530; 95\% CI: [-0.643, -0.418]). 
These PSE indicate biases to intervene at probabilities of winning 7.3, 9.4, 10.2, and 11.3 percentage points below the utility-optimal threshold for intervals, densities, quantile dotplots, and HOPs, respectively. 
% \textit{This suggests that intervals or densities---both without means---make the best decision aids when showing distributions with a single level of variance.}

When we average over factors other than visualization (not shown), users of intervals ($\mu$:-0.075; 95\% CI: [-0.213, 0.080]), HOPs ($\mu$: -0.187; 95\% CI: [-0.342, -0.013]), densities ($\mu$: -0.277; 95\% CI: [-0.392, -0.153]), and quantile dotplots ($\mu$: -0.340; 95\% CI: [-0.447, -0.228]), respectively, show increasing levels of bias toward intervening too often. 
These PSE correspond to intervening when the probability of winning the award with the new player is 2.5, 4.4, 5.1, and 6.1 percentage points below the utility-optimal decision threshold for users of intervals, HOPs, densities, quantile dotplots, respectively.

\textbf{Discussion}
While the impact of adding means on decision quality is small, our results support a more-or-less categorical claim that \textit{means are unhelpful for promoting utility-optimal decisions}.
\idl{What is a ``more-or-less categorical claim''?}
The one exception in our results is that for quantile dotplots at low variance, adding means reduces bias in decision-making. 
However, our results suggests that densities without means promote similarly unbiased decision-making at low variance. \jessica{similar to what}
In realistic use cases where distributions with heterogeneous variances are displayed on a common axis (e.g., in faceted small multiples), designers should prefer to use a consistent uncertainty encoding which supports unbiased decision-making across levels of variance. 
We find that at low variance \textit{densities without means} promote decisions with the least bias and that at high variance bias with densities is not reliably different from intervals.

We preregistered comparisons looking at the impact of uncertainty visualization conditions, averaging across other factors (presented above in text).
However, in retrospect these comparisons are not very useful as design guidelines because they correspond to a visual form which cannot be rendered: a visualization both with and without means. \jessica{not sure about this, presumably different authors could choose to highlight or not highlight means}
Our approach to experimental design and behavioral modeling separates out the impact of various uncertainty encodings with and without means and at different levels of variance, providing more concrete and detailed recommendations than averages across these various conditions.

\subsubsection{Just-Noticeable Differences} 
JNDs describe how much additional evidence a user needs to see to go from intervening 50\% of the time to about 75\% of the time.
\jessica{Recall that} as a rule of thumb, smaller JNDs indicate that a user is sensitive to smaller differences in effect size for the purpose of decision-making.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/jnd-01.png}
    \setlength{\abovecaptionskip}{-10pt}
    \setlength{\belowcaptionskip}{-10pt}
    \caption{Effects of evaluated visualization designs on just-noticeable differences (JNDs) in the decision task.}
    \label{fig:jnd}
\end{figure}

We examine the interaction effects on JNDs of adding means to each uncertainty visualization condition at low and high variance (Fig.~\ref{fig:jnd}, first and third rows).
Adding means to uncertainty encodings only seems to have a reliable effect on JNDs for intervals at high \jessica{variance} ($\mu$: -0.105; 95\% CI: [-0.169, -0.049]).
This corresponds to a 1.2 percentage point reduction in terms of the probability of winning.
% Otherwise, we don't see much of an impact of adding means on JNDs.
When we average across visualization designs, we see a reliable impact of the level of variance on JNDs ($\mu$:-0.223; 95\% CI: [-0.277, -0.174]), such that JNDs are smaller \jessica{when} variance is high (Fig.~\ref{fig:jnd}, fourth row) than when variance is low(Fig.~\ref{fig:jnd}, second row).
This corresponds to a 2.2 percentage point reduction in terms of the probability of winning.
When we average over factors other than visualization (not shown), the average user has a smaller JND (i.e., greater sensitivity) with quantile dotplots ($\mu$:0.431; 95\% CI: [0.388, 0.481]) than with densities ($\mu$: 0.502; 95\% CI: [0.447, 0.567]), intervals ($\mu$:0.520; 95\% CI:	[0.458,	0.598]), or HOPs ($\mu$:0.599; 95\% CI: [0.520, 0.696]). 
These JNDs mean that the average user of quantile dotplots requires the probability of winning with the new player to change by about 5.6 percentage points in order to go from intervening 50\% of the time to 75\%, whereas the average user of densities, intervals, and HOPs require changes in probability of about 6.3, 6.4, and 7.3 percentage points, respectively.

\textbf{Discussion:}
The effects on JNDs that we report \jessica{are} so small that they may not be of practical importance.
For example, the difference in JNDs between quantile dotplots and HOPs---the largest pairwise difference in JNDs between uncertainty encodings---is 1.7 percentage points in term of the probability of winning. 
This is slightly greater than the impact of adding means to intervals at high variance and slightly smaller than the impact of level of variance.
In our task, users are sensitive to probabilities of winning that are 2.2 percentage points smaller at high variance than at low variance.
Perhaps this is because our high variance charts use white space more efficiently than our low variance charts.
\begin{wrapfigure}{r}{0.34\columnwidth}
    \vspace*{-4mm}
    \centering
    \includegraphics[width=0.33\columnwidth]{figures/decoupling-02.png}
    \setlength{\abovecaptionskip}{-5pt}
    \setlength{\belowcaptionskip}{-7pt}
    \caption{JND and PSE vs LLO slopes per user. Outliers omitted.}
    \label{fig:decoupling}
\end{wrapfigure}
This explanation is consistent with the idea that visual distance is a proxy for effect size, and it suggests that the way visualization designers scale axes has an impact the perceived signal in a chart. \jessica{does it necessarily mean visual distance? maybe they can just read axis values better}

\subsection{Relationship Between Estimation and Decision}
\idl{How valuable are these figures? Move to supplementary material?}
% There seems to be a decoupling of magnitude estimation and decision-making performance in our experiment.
We find that different visualization designs lead to the best performance on our magnitude estimation and decision-making tasks.
To explore this decoupling of performance across tasks, we investigate how our three derived measures---LLO slopes, PSE, and JND---are related within individual subjects.
Figure~\ref{fig:decoupling} shows that many individuals who are poor at magnitude estimation (i.e., LLO slopes far below one) do well on the decision task (i.e., PSE or JND close to zero). \jessica{might add lower = better annotation to y axis in Fig 11}

\begin{wrapfigure}{r}{0.34\columnwidth}
    \vspace*{-15mm}
    \centering
    \includegraphics[width=0.33\columnwidth]{figures/decoupling-03.png}
    \setlength{\abovecaptionskip}{-5pt}
    \setlength{\belowcaptionskip}{-7pt}
    \caption{JND vs PSE per user. Outliers omitted.}
    \label{fig:jnd-pse}
\end{wrapfigure}

Previous work~\cite{Khaw2017} finds that individual differences in perceptual sensitivity explain biases in decision-making. \jessica{what sort of perception is discussed here? may need to give slighty more context in prior sentence}
We conceptually replicate this finding by comparing JND and PSE within individual users (Fig~\ref{fig:jnd-pse}):
Greater sensitivity to effect size for decision-making (i.e., JNDs close to zero) predicts more utility optimal decisions (i.e., PSE close to zero).
However, that we see decoupling of perceptual bias in effect size estimation (i.e., LLO slopes) from sensitivity to effect size for decision-making (i.e., JNDs) lends credence to Kahneman \& Tversky's~\cite{Kahneman1979} distinction between perceived probability $p$ and how probability is weighted for decision-making $\mathrm{\pi}(p)$. \jessica{this is interesting, but may want to remind reader how JND equates to weighting probability in decisions. perhaps we should use this analogy earlier to help readers get the difference between LLO slope and JND?}
As visualization designers, we should be mindful that perceptual accuracy may not feed forward directly into decision-making, but that there are mitigating factors. \jessica{do we need this last phrase about mitigating factors? it raises more questions for me than it answers}



==> archived/drafts/results-draft2edit.tex <==
\section{Results}
\idl{This section is like a massive wall of text. I know its kind of inevitable when reporting experimental results, but any way to cut this down / make it more readable? Maybe report all the numbers in a table so that you can only comment on the interesting stuff in the text?}
\subsection{Probability of Superiority Judgments}
We report impacts of visualization design on probability of superiority judgments in terms of slopes in the linear in log odds (LLO) model, which measuring bias in perceived effect size.
Recall that a slope of one indicates unbiased performance, and slopes less than one indicate the degree to which users underestimate effect size.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/llo_slopes-04.png}
    \setlength{\abovecaptionskip}{-10pt}
    \setlength{\belowcaptionskip}{-10pt}
    \caption{Effects of evaluated visualization designs on linear in log odds (LLO) model slopes.
    \idl{What does ``increases slope'' or ``decreases slope'' mean here? Maybe add to the caption how to interpret the changing slope of the model.}
    \matt{if the LLo slope figure moved down to this part of the paper you could annotate some of the slope sizes from this figure in that one, or even combine them into something that shows all of it.} \matt{All of these figures MUST indicate clearly and in a way that cant be ignored that the densities are uncertainty in means and not representative of data. From previous experience readers will make that mistake.}
    } 
    \label{fig:llo_slopes}
\end{figure}

We examine the interaction effect on LLO slopes of adding means to each uncertainty visualization condition at low and high variance.
For every uncertainty encoding, adding means at low variance decreases LLO slopes (Fig.~\ref{fig:llo_slopes}, first row).
When we average over visualization conditions, adding means at low variance changes LLO slopes by -0.031 (95\% CI: [-0.044, -0.020]) for the average user (Fig.~\ref{fig:llo_slopes}, second row). 
This corresponds to a very small increase in magnitude estimation error of about 0.8 percentage points on the probability of superiority scale.
If we similarly average over visualization conditions, the impact of adding means at high variance is ambiguous (Fig.~\ref{fig:llo_slopes}, fourth row) because this effect changes directions for different uncertainty encodings. 
At high variance (Fig.~\ref{fig:llo_slopes}, third row), adding means increases LLO slopes for intervals ($\mu$: 0.045; 95\% CI: [0.024, 0.064]) and densities ($\mu$: 0.039; 95\% CI: [0.014, 0.063]), whereas adding means decreases LLO slopes for HOPs ($\mu$: -0.038; 95\% CI: [-0.071, -0.004]). 
Although these effects seem similar in magnitude, differences in LLO slopes represent changes in the exponent of a power law relationship.
Consequently, the small reduction in predicted error for probability of superiority judgments is about 1.5 and 1.0 percentage points for intervals and densities, respectively, whereas the very small increase in predicted error is 0.3 percentage points for HOPs. 
% \jessica{I would add 'small' or 'very small' in front of one of these mentions of effects since some readers may skim through these numeric heavy paragraphs} 

Users tend to underestimate effect size on our task regardless of visualization design (Fig. ~\ref{fig:llo_slopes}).
When we average over factors other than visualization condition (not shown), LLO slopes are reliably closer to one with quantile dotplots ($\mu$: 0.566; 95\% CI: [0.503,	0.631]) than with densities ($\mu$: 0.436; 95\% CI: [0.372, 0.499]), HOPs ($\mu$: 0.394; 95\% CI: [0.329, 0.460]), and intervals ($\mu$: 0.350; 95\% CI: [0.289, 0.413]) in order of increasing bias.
These LLO slopes correspond to average predicted errors in probability of superiority judgments of 8.9 percentage points for quantile dotplots and 12.4, 14.0, and 14.6 percentage points for users of densities, HOPs, and intervals, respectively. 

\textbf{Discussion:}
Adding means to uncertainty visualizations does not appear to help users make effect size judgments under most conditions, but it does not appear to harm them either.
While we do not want to overstate the practical importance of this small effect, adding means to uncertainty visualizations induces a pattern of behavior consistent with relying on visual distance between distributions as a proxy for effect size:
when variance in distributions is low relative to the maximum variance shown on a common axis, users tend to underestimate effect size \textit{more} when means are present (Fig.~\ref{fig:llo_slopes}, second row); 
% \jessica{should we qualify relatively low, like relative to what}
when variance in distributions is higher, users tend to underestimate effect size \textit{less} when means are present, at least for intervals and densities (Fig.~\ref{fig:llo_slopes}, third row). 
This is the behavioral signature of a distance-based heuristic.


Among the uncertainty encodings we tested, users of quantile dotplots show the least bias on average.
This is not surprising considering previous work (e.g.,~\cite{Gigerenzer1995,Hoffrage1998,Hullman2015,Kale2019-hops,Kay2016}) showing that frequency-based visualizations are effective at conveying probabilities.
% However, quantile dotplots are optimized to show cumulative probabilities for a single distribution~\cite{Kay2016}, not for comparisons between two distributions.
% Similarly with intervals and densities, users should not be able to decode the ground truth directly by comparing two distributions unless the distributions completely overlap, or they rely on statistical theory to calculate effect size analytically from visualized means and variances.
However, it is suprising that users do not perform reliably differently with HOPs, the other frequency-based encoding we tested, than with intervals or densities.\footnote{Our results are consistent with a recent experiment where HOPs users perform on par with users of error bars showing a 95\% predictive interval~\cite{Hofman2020}.}
Consider the information formats of these visualizations. 
HOPs directly encode probability of superiority by how often the draws from the two distributions change order, whereas in other conditions users would need to rely on statistical theory to calculate effect size analytically from visualized means and variances.
In Section 5, we present descriptive evidence of heuristics that users employ under different visualization conditions, which helps to explain these results.
\alex{I condensed three paragraphs into one here.}

% In contrast, HOPs directly encode probability of superiority by how often the draws from the two distributions change order.
% We find it surprising that HOPs users do not perform reliably differently from users of intervals or densities.
% Our results are inconsistent with some findings from previous
% % repeated-measures and within-subjects 
% experiments showing that HOPs are more perceptually effective than violin plots and error bars~\cite{Hullman2015,Kale2019-hops}.
% However, our results are \textit{consistent} with
% % a large between-subjects 
% an
% experiment where HOPs users perform on par with users of error bars showing a 95\% predictive interval~\cite{Hofman2020}.
% One plausible explanation for these contradictory results are differences in cognitive load between experiments.
% Both experiments where HOPs users perform poorly involve incentivized decisions, which require users to reason about an incentive structure where the optimal decision rule is not obvious.
% Additionally, our study involved two tasks and multiple within-subjects manipulations.
% We speculate that the attentional demands of our experiment may lead HOPs users to rely on suboptimal heuristics, rather than reasoning about frequencies of events.

% Given that the optimal visual reasoning strategies for our task are unclear with every visualization condition but HOPs, yet HOPs users perform somewhat poorly, the descriptive evidence of heuristics that users employ under different visualization conditions, which we present in Section 5, provides context that can help us understand these results.


\subsection{Intervention Decisions}
We report impacts of visualization design on decision quality in terms of two metrics derived from our logistic regression model: points of subjective equality (PSE) and just-noticeable differences (JNDs).

\subsubsection{Points of Subjective Equality} 
Recall that PSE describes the amount of evidence at which a user sees intervening versus not intervening as having equal utility.
A PSE of zero is utility-optimal, negative PSE indicates intervening too often, and positive PSE indicates not intervening enough.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/pse-11.png}
    \setlength{\abovecaptionskip}{-10pt}
    \setlength{\belowcaptionskip}{-10pt}
    \caption{Effects of evaluated visualization designs on points of subjective equality (PSE) in the decision task.}
    \label{fig:pse}
\end{figure}

The interaction effects on PSE of adding means to each uncertainty visualization condition at low and high variance are fairly nuanced (Fig.~\ref{fig:pse}, first and third rows).
Adding means at high variance reliably reduces PSE for intervals ($\mu$:-0.160; 95\% CI: [-0.277, -0.040]) and maybe for densities ($\mu$:-0.11646489; 95\% CI: [-0.238, 0.002]), resulting in biases toward intervening of 3.2 and 2.4 percentage points, respectively, in terms of the probability of winning.
Quantile dotplots are the only condition where the average user is biased toward intervention at both high and low variance.
This means that when extrinsic means are added to quantile dotplots at low variance, they have a uniquely debiasing impact on PSE ($\mu$:0.252; 95\% CI:	[0.082,	0.435]), changing the average user's bias from 3.6 percentage points below the utility-optimal threshold to 0.3 percentage points above and thus eliminating bias toward intervention.
\jessica{This paragraph is hard to get much from - too many subtle points to thread together}

When we average over visualization conditions (Fig.~\ref{fig:pse}, second and fourth rows), we see that \textit{adding extrinsic means consistently biases PSE away from the utility-optimal decision rule} \matt{this is directly contradicted by the previous sentence about dotplots}.
At \textit{low variance} and without means, the average user may have a slightly positive PSE ($\mu$: 0.075; 95\% CI: [-0.034, 0.197]), indicating \textit{bias against intervention} 0.6 percentage points above the utility-optimal PSE.
Adding means increases this mild bias in PSE ($\mu$: 0.150; 95\% CI: [0.027, 0.281]) by about 1.7 percentage points.
Conversely, at \textit{high variance} and without means, the average user has a negative PSE ($\mu$: -0.538;	95\% CI: [-0.599, -0.476]), indicating \textit{bias toward intervention} 8.3 percentage points below the utility-optimal PSE in terms of the probability of winning.
Adding means exacerbates this bias in PSE ($\mu$: -0.105; 95\% CI: [-0.175, -0.036]) by about 2.1 percentage points.

In Figure~\ref{fig:pse} (first and third rows) \matt{this ``row'' nomenclature is confusing, need a clearer way to refer to subfigures}, we see that different visualization designs result in the least bias depending on the level of variance.
At \textit{low variance and without means}, densities \matt{with means or without? by my reading densities without means and dotplots with means are the least biased? though it's hard to tell because I had to visually marginalize to figure this out, which I probably shouldn't have to do...} lead to the least bias on average ($\mu$: -0.033; 95\% CI: [-0.188, 0.127]), with PSE less biased than HOPs ($\mu$: 0.255; 95\% CI: [0.021, 0.531]) and intervals ($\mu$: 0.292; 95\% CI: [0.077, 0.548]), but not quite reliably less biased than quantile dotplots ($\mu$: -0.213; 95\% CI: [-0.360, -0.064]).
Note that the direction of bias is \textit{against} intervention for HOPs and intervals, where the average users' PSE are 3.2 and 3.5 percentage points \textit{above} the utility-optimal decision threshold, respectively.
Whereas for densities and quantile dotplots, the direction of bias is \textit{toward} intervention such that the average users' PSE are 0.6 and 3.6 percentage points \textit{below} the utility-optimal decision threshold, respectively.
At \textit{high variance and without means}, intervals lead to the least bias on average ($\mu$: -0.423; 95\% CI: [-0.541, -0.302]), with PSE slightly less biased than HOPs ($\mu$:-0.625; 95\% CI:	[-0.759, -0.496]), maybe less biased that quantile dotplots ($\mu$:-0.5727111; 95\% CI: [-0.676, -0.470]), but not reliably less biased than densities ($\mu$:-0.530; 95\% CI: [-0.643, -0.418]). 
These PSE indicate biases to intervene at probabilities of winning 7.3, 9.4, 10.2, and 11.3 percentage points below the utility-optimal PSE for intervals, densities, quantile dotplots, and HOPs, respectively. 

Averaging over factors other than visualization (not shown), users of intervals ($\mu$:-0.075; 95\% CI: [-0.213, 0.080]), HOPs ($\mu$: -0.187; 95\% CI: [-0.342, -0.013]), densities ($\mu$: -0.277; 95\% CI: [-0.392, -0.153]), and quantile dotplots ($\mu$: -0.340; 95\% CI: [-0.447, -0.228]), respectively, show increasing levels of bias toward intervening too often. 
Users of intervals, HOPs, densities, and quantile dotplots, respectively, intervene when the probability of winning the award with a new player is 2.5, 4.4, 5.1, and 6.1 percentage points below the utility-optimal PSE.

\textbf{Discussion}
While the impact of adding means on decision quality is small, our results suggest that \textit{means are unhelpful for promoting utility-optimal decisions}.
The one exception in our results is that for quantile dotplots at low variance, adding means reduces bias in decision-making, however user performance is no less biased when using densities without means at low variance. 
In realistic use cases where distributions with heterogeneous variances are displayed on a common axis (e.g., in faceted small multiples), designers should prefer to use a consistent uncertainty encoding which supports unbiased decision-making across levels of variance. 
We find that at low variance \textit{densities without means} promote decisions with the least bias and that at high variance bias with densities is not reliably different from intervals.

We preregistered comparisons looking at the impact of uncertainty visualization conditions, averaging across other factors (presented above in text).
However, in retrospect these comparisons are not very useful as design guidelines because they correspond to a visual form which cannot be rendered: a visualization both with and without means added at the same time.
% \jessica{not sure about this, presumably different authors could choose to highlight or not highlight means}
Our approach to experimental design and behavioral modeling separates out the impact of various uncertainty encodings with and without means and at different levels of variance, providing more concrete and detailed recommendations than averages across these various conditions.

\subsubsection{Just-Noticeable Differences} 
JNDs describe how much additional evidence a user needs to see to go from intervening 50\% of the time to about 75\% of the time.
Recall that as a rule of thumb, smaller JNDs indicate that a user is sensitive to smaller differences in effect size for the purpose of decision-making.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/jnd-01.png}
    \setlength{\abovecaptionskip}{-10pt}
    \setlength{\belowcaptionskip}{-10pt}
    \caption{Effects of evaluated visualization designs on just-noticeable differences (JNDs) in the decision task.}
    \label{fig:jnd}
\end{figure}

We examine the interaction effects on JNDs of adding means to each uncertainty visualization condition at low and high variance (Fig.~\ref{fig:jnd}, first and third rows).
Adding means to uncertainty encodings only seems to have a reliable effect on JNDs for intervals at high variance ($\mu$: -0.105; 95\% CI: [-0.169, -0.049]).
This corresponds to a 1.2 percentage point reduction in terms of the probability of winning.
Averaging across visualization designs, we see a reliable impact of the level of variance on JNDs ($\mu$:-0.223; 95\% CI: [-0.277, -0.174]), such that JNDs are smaller when variance is high (Fig.~\ref{fig:jnd}, fourth row) than when variance is low(Fig.~\ref{fig:jnd}, second row).
This corresponds to a 2.2 percentage point reduction in terms of the probability of winning.
Averaging over factors other than visualization (not shown), the average user has a smaller JND (i.e., greater sensitivity) with quantile dotplots ($\mu$:0.431; 95\% CI: [0.388, 0.481]) than with densities ($\mu$: 0.502; 95\% CI: [0.447, 0.567]), intervals ($\mu$:0.520; 95\% CI:	[0.458,	0.598]), or HOPs ($\mu$:0.599; 95\% CI: [0.520, 0.696]). 
These JNDs mean that the average user of quantile dotplots requires the probability of winning with the new player to change by about 5.6 percentage points in order to go from intervening 50\% of the time to 75\%, whereas the average user of densities, intervals, and HOPs require changes in probability of about 6.3, 6.4, and 7.3 percentage points, respectively.

\textbf{Discussion:}
The effects on JNDs that we report are so small that they may not be of practical importance.
For example, the difference in JNDs between quantile dotplots and HOPs---the largest pairwise difference in JNDs between uncertainty encodings---is 1.7 percentage points in term of the probability of winning. 
This is slightly greater than the impact of adding means to intervals at high variance and slightly smaller than the impact of level of variance.
In our task, users are sensitive to probabilities of winning that are 2.2 percentage points smaller at high variance than at low variance.
Perhaps this is because our high variance charts use white space more efficiently than our low variance charts.
\begin{wrapfigure}{r}{0.34\columnwidth}
    \vspace*{-4mm}
    \centering
    \includegraphics[width=0.33\columnwidth]{figures/decoupling-02.png}
    \setlength{\abovecaptionskip}{-5pt}
    \setlength{\belowcaptionskip}{-7pt}
    \caption{JND and PSE vs LLO slopes per user. Outliers omitted.}
    \label{fig:decoupling}
\end{wrapfigure}
% This explanation is consistent with the idea that visual distance is a proxy for effect size, and it suggests that the way visualization designers scale axes has an impact the perceived signal in a chart. \jessica{does it necessarily mean visual distance? maybe they can just read axis values better}

\subsection{Relationship Between Estimation and Decision}
\idl{How valuable are these figures? Move to supplementary material?} \matt{are these JND and PSE estimates posterior estimates from the two models?} \alex{Yes, these are average posterior estimates of the derived measures from both models for individual users (i.e., incorporating random effects).}
% There seems to be a decoupling of magnitude estimation and decision-making performance in our experiment.
We find that different visualization designs lead to the best performance on our magnitude estimation and decision-making tasks.
To explore this decoupling of performance across tasks, we investigate how our three derived measures---LLO slopes, PSE, and JND---are related within individual subjects.
Figure~\ref{fig:decoupling} shows that many individuals who are poor at magnitude estimation (i.e., LLO slopes far below one) do well on the decision task (i.e., PSE or JND close to zero). \jessica{might add lower = better annotation to y axis in Fig 11}

\begin{wrapfigure}{r}{0.34\columnwidth}
    \vspace*{-15mm}
    \centering
    \includegraphics[width=0.33\columnwidth]{figures/decoupling-03.png}
    \setlength{\abovecaptionskip}{-5pt}
    \setlength{\belowcaptionskip}{-7pt}
    \caption{JND vs PSE per user. Outliers omitted.}
    \label{fig:jnd-pse}
\end{wrapfigure}

Previous work~\cite{Khaw2017} finds that individual differences in perceptual sensitivity explain biases in decision-making. \jessica{what sort of perception is discussed here? may need to give slighty more context in prior sentence}
We conceptually replicate this finding by comparing JND and PSE within individual users (Fig~\ref{fig:jnd-pse}):
Greater sensitivity to effect size for decision-making (i.e., JNDs close to zero) predicts more utility optimal decisions (i.e., PSE close to zero).
However, that we see decoupling of perceptual bias in effect size estimation (i.e., LLO slopes) from sensitivity to effect size for decision-making (i.e., JNDs) lends credence to Kahneman \& Tversky's~\cite{Kahneman1979} distinction between perceived probability $p$ and how probability is weighted for decision-making $\mathrm{\pi}(p)$. \jessica{this is interesting, but may want to remind reader how JND equates to weighting probability in decisions. perhaps we should use this analogy earlier to help readers get the difference between LLO slope and JND?} \matt{this seems like an overly formal way to talk about the problem. Isn't it just that, just because people might be able to more accurately perceive some value they would need to make a decision, they might not know how to use it to make a better decision? Indeed, they might be employing different strategies? (this connects back to everything you were just talking about in the qual results too)}
As visualization designers, we should be mindful that perceptual accuracy may not feed forward directly into decision-making, but that there are mitigating factors. \jessica{do we need this last phrase about mitigating factors? it raises more questions for me than it answers}



==> archived/drafts/strategies-draft1.tex <==
\section{Visual Reasoning Strategies}

\subsection{Prevalent Strategies}
Using qualitative analysis of participants' reported strategies, we identify a set of prevalent ways that users make judgments of effect size from visual properties of distributional encodings. 
These patterns of visual reasoning give us a vocabulary for discussing the impact of visualization design choices.

\textbf{Distance:}
The majority of users (292 of 442; 66.1\%) rely on a judgment of ``how far to the right'' the red distribution is compared to the blue one.
Sometimes they are more specific about their criteria, e.g., \textit{``I tried to use the chart in five point-increments which I eyeballed between 100 and 150,''} the locations of orthogonal grid lines.
A modest subset of users (35 of 442; 7.9\%) seem to understand that their interpretation of the distance between distributions should be contingent on the spread of the distributions, suggesting that not nearly as many people as we might hope are sensitive to the impact of variance on effect size.
We posit a spectrum of distance-based judgments ranging in intentionality from gist distance estimation to actually comparing the distance between graphical elements to the length of uncertainty encodings or the x-axis.

\textbf{Variance:}
A decent portion of users (87 of 442; 19.7\%) rely on the ``spread'' or ``width'' of the distributions in some way. \jessica{seems to contradict the only 7.9\% above who seem to understand they should use spread?}
However, a non-trivial number of these users (17 of 87; 19.5\%) mention an explicit preference for low variance---interpreting variance as the level of risk or confidence in the data---or a preference for high variance---seeing the possibility of scoring a higher point total with the new player and neglecting the fact the both distributions always had the same variance.
Further, most users who mentioned relying on variance did not explicitly mention using it in combination with distance as a cue for effect size (52 of 87; 59.8\%).

\textbf{Area:}
Some users (81 of 442; 18.3\%) rely on the area of visual markings to judge effect size.
Of these users, some judge the cumulative area across a threshold (42 of 81; 51.9\%) \jessica{what kinds of threshold}, and others judge the overlap in spatial extent between two distributions (31 of 81; 38.3\%).

\textbf{Frequency:}
Some users (95 of 442; 21.5\%) rely on frequencies of graphical markings (i.e., draws in HOPs or dots in quantile dotplots) to judge effect size.
These users mostly are split between judging the frequency of marks across a threshold (68 of 95; 71.6\%) or the frequency of draws changing order in HOPs (19 of 95; 20\%).  \jessica{this last point is informative because the frequency of draws changing order is the best strategy for hops (at least for prob superiority). Do you think its fair to say from what you saw in comments that potentially only 20\% of hops users knew to do this?} 

\textbf{Reference Lines:}
Almost half of users (207 of 442; 46.8\%) rely on vertical reference lines. \jessica{what are vertical reference lines}
Most of these users (160 of 207; 77.3\%) judge cumulative probability using the dotted vertical line marking the threshold to win an award \jessica{is this overlapping with one of the above strategies about area?} in addition to other visual cues such as distance, area, or number of graphical elements.
In addition to the threshold to win, some users (27 of 207; 13\%) imagine partitions of the x-axis or use the grid lines on the chart to support overlap judgments or to anchor judgments of distance.

A substantial number of users (129 of 442; 29.2\%) switch between strategies in the middle of the task or use multiple strategies in combination.
For example, one user of intervals without means said, \textit{``If the red [distribution] was completely past the dotted line then I would buy the new player no matter what. If there were overlaps with blue I would just risk assess to see if it was worth it to me or not.''} 
This user looked at distance to get a rough sense of effect size, but they also paid attention to distribution overlap to triage their sense of utility. \jessica{I can't tell from the quote if its an either or? previous statement suggests it not, but quote seems to imply it is}
We are not necessarily modeling a consistent judgment process within each user. \jessica{are we modeling judgment process really? could be construed more like imposing a relationship on it}
This suggest that the predominant approach to graphical perception (i.e., measuring effectiveness in terms of average accuracy or response time) oversimplifies and wrongly homogenizes the visual reasoning of chart users. \jessica{this point doesn't totally follow for me. what seems more obvious are things like We shouldn't assume that people are consistent in how they read uncertainty visualizations, or that they will use the visualizations in a statistical valid way, and by considering strategies alongside measures of effectiveness we may gain useful information that helps us consider new visualizations. }


\subsection{Impacts of Visualization Design Choices}

\textbf{Intervals:}
A larger portion of users rely on a distance-based judgment of effect size with intervals (85 of 112; 75.9\%) compared to densities (68 of 99; 68.7\%), HOPs (74 of 121; 61.2\%), and quantile dotplots (65 of 110; 59.1\%).
Many users rely on area judgments with intervals (31 of 112; 27.7\%), with the majority of these users (17 of 31; 54.8\%) judging the amount of overlap between distributions. \jessica{might want to remind reader somewhere whether any of these categories are mutually exclusive, i assume not but its easy to wonder}

\textbf{HOPs:}
In our task, HOPs users tend to judge the distance between distributions or the mean difference (100 of 121; 82.6\%) in similar proportion to users of intervals (94 of 112; 83.9\%) and somewhat more than users of densities (80 of 99; 80.8\%) and quantile dotplots (83 of 110; 75.5\%).
This strategy is not mutually exclusive with reasoning about frequencies of draws, which 54 of 121 users (44.6\%) mention.
\jessica{Among} \sout{Many} HOPs users who rely on frequencies, \jessica{the majority} count the number of draws that cross the threshold to win (37 of 54; 68.5\%). \jessica{again I am thinking that somewhere in the paper (maybe we already added something) we need to directly address the extent to which there are better or worse strategies for each vis, perhaps at the beginning of this section. i think otherwise the reader may miss a lot of the nuance in the strategies discussion, like they may think everything is equally valid}
Users tend to switch strategies more with HOPs (48 of 121; 39.7\%) than with intervals (35 of 112; 31.2\%), densities (23 of 99; 23.2\%), and quantile dotplots (23 of 110; 20.9\%).
The vast majority of strategy switching among HOPs users involves relying on the mean as a cue (39 of 48; 81.2\%). \jessica{in both strategies?}
More than half of users who switch strategies and mention means transition between reasoning about frequencies of draws and reasoning about means (23 of 39; 59.0\%).
The high rates of reliance on distance or means and strategy switching among HOPs users help to explain why their performance is lower than expected.
\jessica{curious if there are performance differences if we separate out those who appear to use frequency}

\textbf{Densities:}
As in other conditions, many users of densities (68 of 99; 68.7\%) tend to make judgments of distance. 
As expected, many users (36 of 99; 36.4\%) describe using area as a cue, predominantly judging the area of the curve beyond the threshold to win (19 of 36; 52.8\%) or the area of overlap between distributions (10 of 36; 27.8\%). \jessica{maybe compare area judgments among densities and qdps}
Interestingly, users of densities were more likely to rely on the spread of the distributions as a cue (27 of 99; 27.3\%) compared to intervals (24 of 112; 21.4\%), HOPs (25 of 121; 20.7\%), and quantile dotplots (11 of 110; 10\%).
Fewer users of densities gave informative strategy descriptions (99 of 156; 63.5\%) compared to intervals (112 of 160; 70\%), quantile dotplots (110 of 154; 71.4\%), and HOPs (121 of 152; 79.6\%). 
We speculate that the lack of discrete graphic objects to reference with densities, compared to other conditions (e.g., the upper and lower bounds of intervals, and individual draws/dots in frequency based visualizations) may make it more difficult for users to introspect about their visual reasoning.

\textbf{Quantile Dotplots:}
Users of quantile dotplots tend to rely on the distance between distributions or means (83 of 110; 75.5\%), however they do so less than other visualization conditions (see above under HOPs). \jessica{i would put the numbers again in parentheses then say as noted above}
Many quantile dotplot users count dots (41 of 110; 37.3\%), with the vast majority of these users counting dots across the threshold to win (33 of 41; 80.5\%). 

\textbf{Adding Means:}
Many users (155 of 442; 35.1\%) mention using the mean as a cue for effect size. 
If we split users depending on whether or not they start the task with means, a large\jessica{r} number of users change strategy when we add means to the charts halfway through the task (67 of 218; 30.7\%) \sout{, and fewer} \jessica{than} change strategy when we remove means (23 of 224; 10.3\%). 
This asymmetry in strategy switching suggests that means are somewhat sticky as a visual cue, that users will tend to rely on them if they can. \jessica{explain what you mean in previous sentence in more detail}
Indeed, among users who start with means, we see more users attempting to visually estimate means even after we remove them from charts (44 of 224; 19.6\%) than we see switching strategies. 
However, the extent to which relying on the mean impacts performance should depend on what other strategies a person is switching between.
Among users who rely on means and switch strategies (90 of 442; 20.4\%), many users merely incorporated the mean into judgments of distance (40 of 90; 44.4\%). 
Others switch between relying on means and judging frequency (31 of 90; 34.4\%) or area (11 of 90; 12.2\%).
The facts that (1) many users switch between relying on distance and means and (2) user behavior is very heterogeneous might \jessica{help} explain why the aggregate impact of means on performance is rather small in our results. \jessica{I don't think this can explain all of it, i think people using it implicitly even when it isn't there and the lack of saliency in some of our stimuli are probably bigger reasons, though that is speculation}
% Users give mixed feedback on whether adding means makes the task more or less difficult. Among the users who opted to talk about the utility of the mean, there was no consensus.

\textbf{Discussion:} 
A vast majority of users rely on the distance between distributions or mean difference to judge effect size (357 of 442; 80.8\%).
This is in line with what we expected at the outset of the study and what we attempt to measure using the linear in log odds model.
However, because user behavior is so heterogeneous, quantitative models which don't distinguish between possible strategies are missing critical information about the data generating process underlying user responses.

We envision a new class of behavioral models for visualization research which attempt to learn the proportion of users adopting a set of predefined strategies such as those we identify in our qualitative analysis. \jessica{could point to similar other research, eg that jardine franconeri paper, as well as maybe whether we would suggest improving that approach}
In an early pilot study, we attempted to build such a model as a custom Bayesian mixture of alternative strategy functions.
However, we were not able to fit the model due to multiple strategies predicting similar patterns of results. \jessica{any ideas of how we could do this type of work in a sophisticated away without running into this problem? ie is there some happy medium between the conclusions of the jardine work and what we attempted? maybe they just weren't careful enough in noting the limitations of their method? }
We intend to continue pursing this kind of strategy-aware behavioral modeling in future work, \jessica{I generally prefer framing future work activities generally rather than saying that we intend to do them, it becomes unclear if you are suggesting other people back off, which seems like a bad thing to signal in science} perhaps focusing exclusively on different ways that chart users might be judging distance between distributions.

Other than using distance as a cue, the next most prevalent strategy is judging distance, area, or frequency across the threshold to win, which 160 of 442 users (36.2\%) mentioned.
These users may be confusing cumulative probability with probability of superiority. 
However, cumulative probability is the right cue to pay attention to for the decision task. \jessica{again clearly laying out the right strategy for each task and how it differs by chart to the extent that it can be determined seems useful to ground the discussion throughout the paper}
It seems likely that our use of these two tasks together and the inclusion of the threshold reference line on our stimuli contributed to the tendency for users to judge cumulative probability.



% \begin{itemize}
%     % Overview
%     \item Common heuristics for effect size: gist distance; distance/area/counts across threshold; distribution overlap; variance itself (some people prefer high vs low) 
%     \jessica{I like our title (might remove the Investigating) but I also kind of like a phrase like 'To Gist or Not to Gist: How Uncertainty Visualization Design Choices ...'}
%     % Heterogeneity
%     \item Some users change strategy in the middle of the task, even if they do not mention the mean at all. For example, one user of intervals without means said, \textit{``If the red was completely past the dotted line then I would buy the new player no matter what. If there were overlaps with blue I would just risk assess to see if it was worth it to me or not. Most of the time it was not.''} This user looked at distance to get a rough sense of effect size, but when things seemed close they switched to judging distribution overlap. We are not necessarily modeling a consistent judgment process within each user, which implies that graphical perception research to date has oversimplified and wrongly homogenized ideas about the visual reasoning of chart users.
%     % Means
%     \item Many users changed their strategy when mean were added \alex{give proportion}. However, many of these people merely incorporated the mean into judgments of distance that they were already making \alex{give proportion}. This might explain why the impact of means is rather small in aggregate.
%     \item Some users maintain a strategy of relying on means even after they are removed from the chart. \alex{give proportion of users who started with means, mentioned means, and did not change strategy} Others relied on intrinsic cues to estimate the mean before means were added. \alex{give proportion of users who started without means, mentioned means, and did not change strategy}
%     \item Other times (less common) removing the mean derails a user because they become so reliant on the mean that they find the task confusing otherwise.
%     \item Users gave mixed feedback on whether means made the task more or less confusing. No clear agreement.
%     % with HOPs
%     \item Many HOPs users are estimating gist distance and mean difference rather than thinking about frequencies of events. \alex{Give proportions for each} \jessica{curious if there are performance differences if we separate out those who appear to use frequency}
%     \item When means are added in the second block, HOPs users often switch strategies from frequency-based reasoning to looking at the mean difference. \alex{Give proportion of switching and proportion of strategy-switchers who mention using the mean}
%     % with QDPs
%     \item Users of quantile dotplots tend to rely on a mix of distance judgments and counting dots across the threshold to win. They may confusing cumulative probability with probability of superiority, but that may be a better heuristic than what other people are doing.
%     % Thresholds
%     \item The majority of participants use the dotted vertical line marking the threshold number of points to win. Some use it to dichotomize the task, while others describe using it as a reference for cumulative probability judgments based on distance, area, or number of objects on either side.
%     \item Some users imagine partitions of the x-axis other than the provided threshold to support overlap judgments, to dichotomize the task, or as a point of reference used to anchor their judgments.
%     \item A relatively modest subset of users seem to get that their interpretation of the distance \jessica{between distributions} or mean difference should be contingent on the level of variance, suggesting that not nearly as many people as we might hope are \jessica{sensitive to the impact of variance on effect size (or some other rephrasing that's slightly more direct than what you have} \sout{normalizing to the range of possibilities implied by the uncertainty encodings.}
%     \item A non-trivial portion of participants who mention using variance as a cue for the task state an explicit preference for low or high variance charts, seeing variance as indicating risk, confidence, or the possibility of scoring a higher point total with the new player. Some people \jessica{did we code in a way that we can provide a proportion here?} don't understand what the spread of the distribution means.
% \end{itemize}

==> archived/drafts/strategies-draft2.tex <==
\section{Visual Reasoning Strategies}
% \idl{What if insert a figure summarizing the count of the strategies? I know it will be really challenging given that there is not enough room. But I believe it will be effective to convey the stat.}
\idl{It would be nice to have a figure which visually shows all of the different strategies.}
\subsection{Prevalent Strategies}
Using qualitative analysis of reported strategies, we identify prevalent ways that users judge effect size from distributional comparisons.
These visual reasoning patterns form a vocabulary for discussing how users employ the markings on charts and the impacts of visualization design choices \jessica{on their interpretations}. \jessica{could omit prev sentence, or somehow combine with first to make more concise}
The strategies are not mutually exclusive.

\jessica{some missing info here about how you classify users as doing something - in either of their strategy responses? What if its in one only, do you still say things like 'most users'?}

\textbf{Only Distance:}
The majority of users (275 of 442; 62.2\%) rely on ``how far to the right'' the red distribution is compared to the blue one \textit{without mentioning that they incorporate the variance of distributions into their judgments}.
Most of these users \jessica{describe} making a gist estimate of distance between distributions (190 of 275; 69.1\%), with others \jessica{saying the} rely on the mean difference specifically (126 of 275; 45.8\%).
Some users rely on both gist distance and mean difference (36 of 275; 13.1\%).
Strategies which involve only the distance between distributions should result in a large bias toward underestimating effect size. \jessica{do we see this in general}

\textbf{Distance Relative to Variance:}
A modest subset of users (35 of 442; 7.9\%) seem to understand that interpretations of distance between distributions should depend on the spread of the distributions, suggesting that few are sensitive to the impact of variance on effect size.
If users \sout{actually} estimate standard deviation and mean difference between distributions, they could use this information to calculate effect size analytically.
However, we think it is \jessica{far} more likely that these users judge the distance between distributions relative to the spatial extent of uncertainty encodings, which should result in underestimation bias which is similar to but less pronounced than judgments of only distance. 

\textbf{Cumulative Probability:}
A substantial number of users (160 of 442; 36.2\%) estimate the cumulative probability of winning the award with and/or without the new player.
This strategy involves judging the distance, proportion of area, or frequency of markings across the threshold number of points to win (e.g., area to the right of dashed line in Fig.~\ref{fig:teaser}).
These users may be confusing cumulative probability of winning the award, which is the best cue in the decision task, with probability of superiority (i.e., probability that team does better with the new player than without), which is what we ask for in the estimation task. 
% \idl{Can you give an example of what the cumulative probability strategy looks like and how it is different from probability of superiority? You might use a concrete stimulus in Fig. 1}
% However, cumulative probability is the best cue to pay attention to for the decision task.
However, since the probability of winning is a monotonically increasing function of probability of superiority, this strategy results in milder underestimation bias than distance-based strategies. \jessica{this last sentence is hard to parse - can we say for sure it will be milder? maybe we need to qualify eg. this strategy should theoretically .... }
% Our use of two tasks together and the inclusion of an annotated threshold on our stimuli contributed to the tendency for users to judge cumulative probability.

\textbf{Distribution Overlap:}
A small proportion of users (31 of 442; 7.0\%) \jessica{describe} judging the overlap between distributions.
While this seems similar to distance-based strategies, users conceptualize it differently, describing their strategy in terms of area rather than the gap between distributions.
For example, one user of HOPs said they use the charts \textit{``only to see how much of an overlap [there is] between the two areas,''} suggesting that they imagine the contours of distributions over the sets of animated draws.
% \idl{How is this strategy different from `distance relative to variance'?}
This strategy probably results in an underestimation bias similar to judging distance relative to variance. 

\textbf{Frequency of Draws Changing Order:}
This strategy is only relevant to the HOPs condition, where only a handful of users employed it (19 of 121; 15.7\%).
It involves judging the number of animated frames in which that the draws from the two distributions switch order.
This is the best way to estimate probability of superiority from HOPs.
The fact that only 15.7\% of HOPs users employ this strategy helps to explain why the performance of HOPs users is worse than expected.

\textbf{Switching Strategies:}
A substantial number of users (129 of 442; 29.2\%) switch between strategies in the middle of the task.
For example, one user of intervals without means \jessica{described a mix of \textit{cumulative probability} and \textit{distribution overlap}} said, \textit{``If the red [distribution] was completely past the dotted line then I would buy the new player no matter what. If there were overlaps with blue I would just risk assess to see if it was worth it to me or not.''} 
\sout{This user looked at distance past threshold (i.e., \textit{cumulative probability}) to judge effect size, but on trials where distributions were close, they relied on \textit{distribution overlap} to triage their sense of utility. }
% \jessica{I can't tell from the quote if its an either or? previous statement suggests it not, but quote seems to imply it is}
While \sout{this is} more of a meta-strategy, we consider switching to be a very important pattern in our results because it suggests that judgment processes involved in graphical perception are not consistent within each user.
% We are not necessarily modeling a consistent judgment process within each user. \jessica{are we modeling judgment process really? could be construed more like imposing a relationship on it}
% This suggest that the predominant approach to graphical perception (i.e., measuring effectiveness in terms of average accuracy or response time) oversimplifies and wrongly homogenizes the visual reasoning of chart users. \jessica{this point doesn't totally follow for me. what seems more obvious are things like We shouldn't assume that people are consistent in how they read uncertainty visualizations, or that they will use the visualizations in a statistical valid way, and by considering strategies alongside measures of effectiveness we may gain useful information that helps us consider new visualizations. }


\subsection{Visual Features that Users Rely On}
\jessica{I think you could probably omit this section, its more interesting as it comes up below with the chart types} \alex{Maybe we can describe these visual features in the method section when we talk about the coding process and briefly reiterate them at the top of the next section where we talk about the impact of visualization design choices. We should discuss.}
The strategies we identify operate on a small set of visual features of charts.
We describe each visual feature, the proportion of users who rely on them, and how they are incorporated into strategies.

\textbf{Relative Position:}
The majority of users (292 of 442; 66.1\%) rely on the relative position of the two distributions.
Most users who mention relative position employ an \textit{only distance} strategy (266 of 292; 91.1\%). Fewer judge \textit{distance relative to variance} (26 of 292; 8.9\%).

\textbf{Spread:}
A decent portion of users (87 of 442; 19.7\%) rely on the ``spread'' or ``width'' of the distributions as a proxy for variance. \jessica{there are a lot of places here where I think it would be easier to read if we substituted the percentages right into the sentence, eg Roughly 20\% of users rely on .. About 40\% of these users ....}
Some of these users judge \textit{distance relative to variance} (35 of 87; 40.2\%).
However, a non-trivial portion of these users (17 of 87; 19.5\%) mention a preference for low variance---interpreting variance as the level of risk or confidence in the data---or for high variance---seeing the possibility of scoring more points with the new player and neglecting that both distributions always had the same variance.
A small number of these users rely on a \textit{distribution overlap} strategy (6 of 87; 6.9\jessica{\%}).

\textbf{Area:}
Some users (81 of 442; 18.3\%) rely on the area of visual markings.
Of these users, some judge \textit{cumulative probability} (45 of 81; 55.6\%), and others judge \textit{distribution overlap} (31 of 81; 38.3\%).

\textbf{Frequency:}
Some users (95 of 442; 21.5\%) rely on frequencies of markings (i.e., draws in HOPs or dots in quantile dotplots).
Most of these users employ a \textit{cumulative probability} strategy (70 of 95; 73.7\%).
Some others who rely on frequency are HOPs users employing the \textit{frequency of draws changing order} strategy (19 of 95; 20\%).

\textbf{Reference Lines:}
Almost half of users (207 of 442; 46.8\%) rely on vertical reference lines. 
These reference lines could be the decision threshold annotation, vertical grid lines, or lines that the user imagines.
For example, one user imagined a line to help them judge distance: \textit{``I tried to visualize an invisible line in the middle of the teams to gauge how big of a difference a new player would make.''}
Most users who mentioned reference lines employ a \textit{cumulative probability} strategy (160 of 207; 77.3\%).
Fewer rely on vertical grid lines or imagined lines, rather than the threshold annotation (26 of 207; 12.6\%).


\subsection{Impacts of Visualization Design Choices}
Users rely on strategies and visual features to varying degrees depending on how we design the charts we show them.
Recall that strategies are not mutually exclusive and that users often switch between them.

\textbf{Intervals:}
\jessica{Roughly 75\% (85 of 112) of interval users}
\sout{A larger portion of users} rely on \textit{relative position} as a visual cue for effect size \sout{with intervals (85 of 112; 75.9\%)} \jessica{compared to 69\%} \sout{ than} with densities (68 of 99) \sout{; 68.7\%)}, \jessica{61\% with} HOPs (74 of 121), \sout{; 61.2\%),} and \jessica{59\% with} quantile dotplots (65 of 110). \sout{; 59.1\%).} \jessica{trying to make this easier to read, should try to do more of this in this section so the reader doesn't have to keep scanning between text and ()}
Of intervals users who look at \textit{relative position}, the majority (74 of 85; 87.1\%) employ an \textit{only distance} strategy, while fewer judge \textit{distance relative to variance} (11 of 85; 12.9\%).
In other words, only \jessica{about 10\%} (11 of 112) \sout{ (9.8\%)} of intervals users incorporate variance into their judgments of distance.
Many other intervals users look at \textit{area} (31 of 112; 27.7\%), with the majority of these users (17 of 31; 54.8\%) employing a \textit{distribution overlap} strategy.

\textbf{HOPs:}
The majority of HOPs users (74 of 121; 61.2\%) look at \textit{relative position} to judge effect size.
Of HOPs users who rely on \textit{relative position} as a visual cue, almost none (2 of 74; 2.7\%) use a \textit{distance relative to variance} strategy.  
However, looking at \textit{relative position} is not mutually exclusive with looking at \textit{frequency} of draws, which 54 of 121 (44.6\%) HOPs users rely on as a visual feature.
Among HOPs users who rely on frequencies, the majority (37 of 54; 68.5\%) employ a \textit{cumulative probability} strategy, while fewer (19 of 54; 35.2\%) rely on the optimal strategy of counting the \textit{frequency of draws changing order}.
Users tend to \textit{switch strategies} more with HOPs (48 of 121; 39.7\%) than with intervals (35 of 112; 31.2\%), densities (23 of 99; 23.2\%), and quantile dotplots (23 of 110; 20.9\%).
Among HOPs users who switch strategies, the majority (39 of 48; 81.2\%) rely on the mean as a cue.
Strategy switching that involves the mean is less common for users who rely on \textit{relative position} (22 of 74; 29.7\%) than for users who rely on \textit{frequency} (23 of 54; 42.6\%)
That most HOPs users rely on \textit{relative position}, and that those who do rely on \textit{frequency} are more likely to switch to or from relying on the mean, helps to explain why performance with HOPs is lower than expected.

\textbf{Densities:}
The majority of densities users (68 of 99; 68.7\%) rely on \textit{relative position} as a visual cue.
Of densities users who look at \textit{relative position}, very few (9 of 68; 13.2\%) employ a \textit{distance relative to variance} strategy.
As expected, many densities users (36 of 99; 36.4\%) rely on \textit{area} as a cue, compared to 11 of 110 (10\%) quantile dotplots users.
Among densities users who rely on \textit{area}, more than half (19 of 36; 52.8\%) employ a \textit{cumulative probability} strategy, while fewer (10 of 36; 27.8\%) employ the \textit{distribution overlap} strategy. 
Interestingly, users of densities were more likely to rely on the \textit{spread} of distributions as a cue (27 of 99; 27.3\%) than users of intervals (24 of 112; 21.4\%), HOPs (25 of 121; 20.7\%), and quantile dotplots (11 of 110; 10\%).
% Fewer users of densities gave informative strategy descriptions (99 of 156; 63.5\%) compared to intervals (112 of 160; 70\%), quantile dotplots (110 of 154; 71.4\%), and HOPs (121 of 152; 79.6\%). 
% We speculate that the lack of discrete graphic objects to reference with densities---compared to, e.g., the upper and lower bounds of intervals, and individual draws/dots in frequency-based visualizations---may make it more difficult for users to introspect about their visual reasoning.

\textbf{Quantile Dotplots:}
More than half of quantile dotplots users (65 of 110; 59.1\%) look at \textit{relative position} to judge effect size, a similar proportion to users of HOPs (74 of 121; 61.2\%) and a smaller proportion than users of densities (68 of 99; 68.7\%) and intervals (85 of 112; 75.9\%).
Very few quantile dotplots users who rely on \textit{relative position} (4 of 65; 6.2\%) employ a \textit{distance relative to variance} strategy.
Many quantile dotplots users (41 of 110; 37.3\%) rely on \textit{frequency} as a visual cue by counting dots.
The majority of quantile dotplots users who rely on \textit{frequency} (33 of 41; 80.5\%) employ a \textit{cumulative probability} strategy. 

\textbf{Adding Means:}
Many users (155 of 442; 35.1\%) rely on the mean as a cue for effect size. 
If we split users based on whether or not they start the task with means, more users \textit{switch strategies} when we add means to the charts halfway through the task (67 of 218; 30.7\%) than when we remove means (23 of 224; 10.3\%). 
This asymmetry in strategy switching suggests that means are ``sticky'' as a cue: 
% If a user starts relying on the mean they are less likely to switch to a different strategy than they are to switch from a different strategy to relying on means.
% \jessica{explain what you mean in previous sentence in more detail}
Among users who start with and rely on means (67 of 442; 15.2\%), more attempt to visually estimate means \textit{after we remove them from charts} (44 of 67; 65.7\%) than switch to relying on other cues (23 of 67; 34.3\%). 
However, the impact of adding means on performance depends on what other strategies a user is switching between.
Among users who rely on means and switch strategies (90 of 442; 20.4\%), many just incorporate the mean into judgments of \textit{relative position} (40 of 90; 44.4\%) without relying on other visual cues. 
Others switch between relying on means and \textit{frequency} (31 of 90; 34.4\%) or \textit{area} (11 of 90; 12.2\%).
That many users switch between relying on \textit{relative position} and means, and that strategies are heterogeneous, helps to explain why the average impact of means on performance is small in our results. 
% \jessica{I don't think this can explain all of it, i think people using it implicitly even when it isn't there and the lack of saliency in some of our stimuli are probably bigger reasons, though that is speculation}
% Users give mixed feedback on whether adding means makes the task more or less difficult. Among the users who opted to talk about the utility of the mean, there was no consensus.


==> archived/submission/1_intro.tex <==
%% \section{Introduction} %for journal use above \firstsection{..} instead

% \alex{Hook: unpack the relationship between visualization and causal inference. What is the utility of an external representation?}
Data analysts engaged in sensemaking~\cite{Card1999,Pirolli2005,Russell1993,Grolemund2014} infer the compatibility of different causal explanations with their data.
During exploratory analysis or provisional statistical modeling, analysts implicitly or explicitly compare their data to patterns they expect as logical consequences of hypothesized data generating processes~\cite{Andrienko2018,gelman2003,gelman2004exploratory,Hullman2020,hullman2020theories}.
Visualizations play a critical role in causal inference both because externalization reduces cognitive load~\cite{Cox1999} and because human capabilities for inference rely heavily on sensory expectations (e.g., mental imagery) and comparisons between expectations and experiences~\cite{Breedlove2020,Kale2019adaptation}.
% \jessica{I think we can probably improve this first paragraph - the sensemaking reference was a little weird (I expected Pirolli and Card) and I wonder if we should be citing something more canonical like the visual analytics book, which I'm guessing mentions causality. Also would add Andrienko 2018 paper about model building in EVA to the list of things we cite in second paragraph, maybe also Buja et al 2009. Currently feels biased, in a way I like of course, but still potentially biased} \alex{I'll circle back and re-write this.}

% \alex{Talk about the ways in which causal inference can be error prone. Motivate why it is important to model causal inferences with visualizations. We need an evaluative approach to better integrate generative models into visual data analysis software.}
% Despite the potential for visualizations to support causal inferences, 
Data analysts and software designers need to anticipate how human capabilities for causal inference may be error prone.
For instance, perceptual biases such as underestimation of sample size (e.g.,~\cite{Kim2019}) contribute to errors in causal inferences insofar as perceived associations seem to be the basis for causal inferences~\cite{Anderson1995,Xiong2019}.
% Beyond perceptual biases, 
Analysts also err in their causal interpretations of data when the mapping between a potential causal explanation and an expected pattern in the data is unclear~\cite{Batanero1996,Yen2019}.
%, leading to misinterpretations of the perceived signal in data~\cite{Batanero1996,Yen2019}. 
% \jessica{a little abstract maybe give example}
For example, imagine an analyst trying to detect confounding in experiment results on the effectiveness of a treatment at preventing disease (Fig.~\ref{fig:teaser} \raisebox{.5pt}{\textcircled{\raisebox{-.6pt} {A}}}). To detect that `gene' is a confounding factor, the analyst must see effects of gene on both treatment effectiveness (i.e., a difference between the top and bottom cells in the right column of table \raisebox{.5pt}{\textcircled{\raisebox{-.6pt} {A}}}) and overall rate of disease (i.e., a difference between the top and bottom rows of \raisebox{.5pt}{\textcircled{\raisebox{-.6pt} {A}}}). %\jessica{maybe refer to specific cells in A to establish for reader where to look in vis?} 
Attributing these signals in the data to confounding requires the analyst to know what they are looking for, 
% rather than assuming they will passively detect the appropriate visual patterns as insights.
rather than passively detecting the appropriate patterns.

How well do visualizations that commonly appear in visual analytics software support causal inferences? 
Does the ability to interactively filter or aggregate data help analysts discover causal relationships?
In order to answer these questions, we need to compare analysts' causal inferences against a benchmark that is roughly `normative', in the sense that it captures important aspects of good causal inference.
% In order to answer these questions, we need a benchmark for how much analysts should believe a causal explanation based on their data. \jessica{bc its unclear how much we should believe any bayesian model is 'normative', might be worth being a little more nuanced here, something like, in order to answer these qs we need to be able to compare analysts inferences against a benchmark that we believe captures important aspects of good causal inference. (its a small change but might be worth doing this trhoughout paper so its clear we aren't claiming normative is uncontestable/complete} 
% \textit{In order to answer these questions and evaluate model-based interpretations of data more broadly, we need a benchmark for how much analysts should believe a causal explanation based on their data.} \jessica{could skip italics and the second part about model-based interpretations more broadly might be better left for related work and  discussion - I don;t know that the reader will get it in the intro, though I understand why its relevant }
% \jessica{would drop normative from prior sentence}

% \alex{Talk about what we did and what we found}
In this study, we adopt causal support, a model from mathematical psychology~\cite{Griffiths2005}, as a benchmark for evaluating causal inferences from visualizations. 
% \sout{and investigate the research questions above using toy problems involving count and proportion data.} \jessica{simplified instead of toy?}
\textit{Causal support} models one's belief in a set of alternative data generating processes as a Bayesian update.
% , based on the likelihood of the data under each alternative model and a prior encoding initial belief in each alternative.
We posit causal support is a good normative model for three reasons. 
(1) Causal support has numerous proprieties of valid statistical inference in light of the analyst's prior knowledge. It captures the fact that belief in evidence from the data should be stronger as sample size increases. It accounts for unknown unknowns about the space of possible models, such that causal support assigns no posterior probability to models that the analyst does not explicitly consider. 
(2) Prior work~\cite{Griffiths2005} shows through a system of experiments that causal support accounts for otherwise hard-to-explain patterns in human causal inferences. For example, causal support correctly predicts that subjective belief in a causal relationship varies as a function of the potential to detect that relationship in a given data set.
% We posit causal support is normative because:
% \yifan{super minor: might flow better without the bullets?}
% \begin{enumerate}
%     \vspace{-7pt}\item As a Bayesian model of structure learning, causal support has numerous proprieties of valid statistical inference in light of the analyst's prior knowledge. It captures the fact that belief in evidence from the data should be stronger as sample size increases. It accounts for unknown unknowns about the space of possible models, such that causal support assigns no posterior probability to models that the analyst does not explicitly consider.
%     \vspace{-7pt}\item Prior work~\cite{Griffiths2005} shows through a system of experiments that causal support accounts for otherwise hard-to-explain patterns in human causal inferences. For example, causal support correctly predicts that subjective belief in a causal relationship varies as a function of the potential to detect that relationship in a given data set.
% \end{enumerate}
% \vspace{-8pt}
% In addition to being a statistically valid model for structure learning, causal support accounts for otherwise hard-to-explain patterns in human causal inferences~\cite{Griffiths2005}, making it an ideal normative model.
% \yifan{maybe add a line to justify the use causal support? E.g., it best map to human cognition and is statistically sound or something---this combo is actually very particular to the line of work by Tenenbaum and Griffith, that human cognition can be modeled by Bayesian methods.}
(3) Since causal support is \textit{extensible to any generative model} 
% regardless of form or parameterization 
(i.e., models that produce predictions and can assign likelihood to data), this evaluation approach can be applied in a wide range of visual analytics applications to evaluate the quality of causal inferences. 
% \jessica{maybe be clearer that its an ideal normative model if we are comfortable assuming that bayesian inference is a good benchmark}
% \jessica{might to clarify the 'any generative model' part so its less abstract}

% \alex{Unpack contributions}
We contribute two experiments using causal inference problems involving count and proportion data to (1) study the utility of causal support for gaining insight into inferences from visualizations and (2) evaluate how well visualizations common in visual analytics (VA) software support causal inferences.
We compare three common visual encodings for count and proportion data---bar charts, icon arrays, and text tables as a baseline---and we investigate how the ability to interactively aggregate or cross-filter data in bar charts impacts causal inferences. 
In Experiment 1, we ask participants to differentiate whether a treatment is effective by allocating probability across two different data-generating processes.
We find that chart users' causal inferences are far from normative with all visualizations we tested, and that interacting with visualizations can improve sensitivity to signal in predictable ways. 
Ultimately, however, no visualization reliably outperforms text tables. 
We also see that chart users are more sensitive to evidence against a treatment effect than evidence in favor of one, suggesting an unequal weighting of falsifying versus verifying evidence.
In Experiment 2, we replicate the main findings Experiment 1 but with a task where we ask participants to detect confounding in data sets by allocating probability across four alternative data-generating processes. 
The models in this second experiment demonstrate how casual support can be extended to study complex causal inferences across many models. 
% We see similar results as in Experiment 1, suggesting common VA tools do not promote causal inferences which are appropriately sensitive to sample size or evidence that verifies causal effects.
% We point to opportunities to improve support for causal inferences by explicitly incorporating alternative models and their predictions into VA software. \yifan{This last sentence seems a little loose/speculative from the main ideas/narrative?.}

==> archived/submission/2_related-work.tex <==
\section{Related Work}
\subsection{Visualization for casual inference}
Much of the psychology and statistics literature on visual aids for causal reasoning focuses on contingency tables (e.g.,~\cite{Anderson1995,Batanero1996,Cheng1997,Greenland1999,Griffiths2005,Sobel1995}).
% Much of the literature on visual aids for causal reasoning comes out of psychology and statistics, focusing primarily on contingency tables (e.g.,~\cite{Anderson1995,Batanero1996,Cheng1997,Greenland1999,Griffiths2005,Sobel1995}).
Contingency tables support causal inferences by using layout to encode conditional probabilities, the same way trellis plots afford grouping by factors during visual data analysis~\cite{Tukey1977,Becker1996}.
Whether or not a factor seems to be \textit{collapsible}---whether or not patterns the data seem to change depending on whether the data are grouped by that factor---can be a visual signal for reasoning about causal relationships such as confounding~\cite{Greenland1999}.
However, empirical research on interpretation strategies for contingency tables~\cite{Batanero1996} suggests that analysts often misinterpret signals like collapsability because they don't ascertain the mapping between visual signals like collapsability and hypothesized causal relationships.
% However, empirical research on interpretation strategies for contingency tables~\cite{Batanero1996} suggests that most misinterpretations result from ambiguity about precisely how signals like collapsability map to hypothesized causal relationships. \jessica{last sentence not totally clear - so you are saying that collapsibility is an imperfect proxy for causal relationship ?} \alex{There are two aspects of this. First, non-colapsibility is not a guarantee that there is a causal relationship for reasons detailed in Greenland et al. (1999). Second, Batanero et al. (1996) found strategic errors in how people map between observations about contingency tables and specific causal explanations. The first thing is about the nuances of a statistically valid interpretation. The second thing is about cognitive difficulties reasoning about counterfactual patterns that would indicate evidence for a causal relationship.}
Tools like Tableau support exploration of collapsability by enabling analysts to interactively control how data are aggregated.
We investigate whether the ability to interactively control data aggregation improves the quality of causal inferences, showing how strategic errors in causal reasoning impact the use of interactive visualizations.
% In this study we investigate how the ability to interactively control how data are aggregated influences the quality of causal inferences, shedding some light on whether interactive visual analytics can ameliorate strategic errors in causal reasoning. \jessica{this last sentence seems not completely tied to the point about how they find it difficult - why might interaction help that? }

Research on visual analytics (VA) employs a broader range of representations to support causal reasoning, including parallel coordinates~\cite{Wang2016,Wang2018}, bar charts~\cite{Yen2019}, ``diff bar charts'' showing counterfactual outcomes under different conditions as layered bars~\cite{Xie2020preprint}, and novel techniques using animation to show event sequences (e.g.,~\cite{Elmqvist2003,Jin2020,Kadaba2007}).

Some of these interfaces also incorporate directed acyclic graphs (DAGs) as interfaces to models and visualizations (e.g.,~\cite{Wang2016,Wang2018,Xie2020preprint,Yen2019}).
DAGs are a visual tool for causal reasoning which has garnered attention in recent years~\cite{Pearl2018}. 
DAGs encode hypothesized relationships among variables (e.g.,~Fig.\ref{fig:teaser}\raisebox{.5pt}{\textcircled{\raisebox{-.8pt} {B}}}), making causal relationships and the assumptions they entail explicit and in some cases testable~\cite{Bareinboim2016,Pearl2009,Pearl2014,Pearl2015}.
% Judea Pearl and colleagues demonstrate how DAGs can be used to solve thorny problems in causal inference such as formalizing generalizability of scientific findings~\cite{Bareinboim2016,Pearl2014,Pearl2015}.
In this study, we use DAGs to present alternative causal explanations for data sets that we ask participants to judge as a way of making these alternatives and the differences between them explicit (Figs.~\ref{fig:dags-e1-explainer}~\&~\ref{fig:dags-e2-explainer}).

VA systems frequently use interaction techniques such as cross-filtering linked views of data (e.g.,~\cite{Wang2016,Wang2018}) and click- or drag-and-drop-based chart construction (e.g.,~\cite{stolte2002polaris,Xie2020preprint,Yen2019}).
The most similar prior research to our study\footnote{Also, see unpublished formative work from the second author: 
\\ \texttt{URL redacted for anonymous review}
% \\ \url{https://logical-interactions.github.io/causal2020/}
} tests whether constructing charts by clicking on variables versus dragging variables onto a DAG makes a difference in analysts' ability to differentiate between different kinds of causal relationships~\cite{Yen2019}, specifically identifying mediating variables.
Although they do not find an effect of interaction method on causal inferences, the authors provide a detailed strategy analysis extending evidence from psychological studies~\cite{Batanero1996} that analysts struggle to reason about the exact set of visual signals they should look for to verify or falsify a causal relationship.
We extend this line of work by studying whether the ability to (un)facet charts or cross-filter coordinated multiple views impacts the quality of untrained analysts' causal inferences. %\jessica{could consider saying something about how we provide minimal training so can also speak to how attuned people seem to be about what to look for. though maybe not} \alex{Definitely worth mention in discussion I think. Maybe a little out of place here?}

% \jessica{probably want to cite some of the ottley et al and others classic bayesian reasoning stuff at least if we use icon arrays. I can imagine vis reviewers bringing that up}
Previous work in visualization~\cite{Micallef2012,Ottley2016} and risk communication~\cite{Galesic2009,Spiegelhalter1999} suggests that icon arrays can improve Bayesian inferences.
This may be in part because of cognitive benefits of framing probabilities as frequencies of events~\cite{Gigerenzer1995,Hoffrage1998,Hullman2015,Kay2016}.
% However, the performance improvements associated with these visualizations seem to depend on the use of text in the display~\cite{Micallef2012}, the chart user's spatial ability~\cite{Ottley2016}, and the strategies users rely on~\cite{Kale2021}.
We compare icon arrays to text tables and bar charts since these visualizations represent very different parts of the design space for showing count data and are also easy to create in visual analytics software like Tableau.


\subsection{Modeling causal reasoning}
In the present study, we draw on and extend a model of causal reasoning called causal support, first proposed by Griffiths and Tenenbaum~\cite{Griffiths2005}.
\textit{Causal support} formulates causal inferences as a Bayesian update on the log odds of a finite set of causal explanations given some observed data. 
Mathematically, causal support has similar properties to a Chi-squared test (i.e., Are the data in each cell of a contingency table likely generated by the same process?), which prior work analogizes to the kind of comparisons between data and model predictions that analysts visualize in ``model checks''~\cite{gelman2003,gelman2004exploratory,hullman2020theories} such as QQ-plots.
However, unlike a Chi-squared test, causal support relies on Monte Carlo simulations to assign likelihoods under alternative causal explanations, making causal support extensible to any finite set of generative causal models.
For instance, Pacer and Griffiths extend causal support to handle continuous data~\cite{Pacer2011} and event streams~\cite{Pacer2015}.

Previous cognitive models of causal inference explored in psychology share more in common with parameter estimation than statistical inference per se, a subtle but important distinction.
One such model \textit{delta p} posits that that people judge differences in conditional proportions of observed events when making causal inferences about count data~\cite{Anderson1995}.
Another such model \textit{causal power} posits that people judge the magnitude of effect size when making causal inferences~\cite{Cheng1997}. 
Both of these predecessors and alternatives to causal support make the assumption that causal inferences are fundamentally a perceptual judgment.
The difference between them is that causal power rescales delta p to apportion the posited signal for causal inferences based on the potential to detect any signal whatsoever within the observed data.
In contrast, causal support assumes that the signal for causal inferences depends on the possible data generating models that the analyst has in mind and represents these alternative models explicitly.
This makes causal support more flexible, with higher predictive validity for human judgments than delta p, causal power, and even Chi-squared~\cite{Griffiths2005}. 
Causal support models structure learning in a way that reflects analysts' natural tendency to dichotomize, for better or worse, reasoning about whether or not causal relationships exist rather than how strong they are.

==> archived/submission/3_e1-method.tex <==
% \begin{figure*}[th!]
%     \centering
%     \includegraphics[width=\textwidth]{figures/vis-conditions_all.png}
%     % \setlength{\intextsep}{-20pt}
%     \setlength{\abovecaptionskip}{-10pt}
%     \setlength{\belowcaptionskip}{-10pt}
%     \caption{Visualization conditions evaluated in our study.
%     }
%     \label{fig:vis-conds}
% \end{figure*}

\section{Experiment 1}
% Our first experiment addresses the research question: 
\textit{How well do different visualization designs that are common in visual analytics (VA) software support causal inferences?} 
We evaluate visualizations of count data including text contingency tables, icon arrays, grouped bar charts, bars that users can interactively aggregate, and linked bars that users can interactively cross-filter.
% We compare encodings of count data using text contingency tables as a baseline. We also evaluate icon arrays, grouped bar charts, bars that users can interactively aggregate, and linked bars that users can interactively cross-filter.
In Experiment 1, we investigate chart users' ability to infer whether a treatment prevents a disease.
By asking chart users about a treatment effect in count data, we build on the task and structural equation models used by Griffiths and Tenenbaum~\cite{Griffiths2005} to propose and validate causal support.
% We chose to ask chart users about a treatment effect in count data in order to build on the task and structural equation models used by Griffiths and Tenenbaum~\cite{Griffiths2005} to propose, operationalize, and validate causal support.
% \jessica{should we briefly motivate count data?}
Count data are also ideal for evaluating bar charts. \jessica{Do you need the previous sentence? not sure exactly what you mean.}
The design requirements for supporting our causal inference task with count data are that visualizations should express both the \textit{proportion} of people with disease and \textit{sample size}.
% Considering these design requirements, we ruled out evaluating some additional visualization conditions such as pie charts and heatmaps, which are common ways of encoding proportions in VA but which don't encode sample size.
Based on these requirements, we ruled out testing visualizations such as pie charts and heatmaps, which are common ways of encoding proportions but which don't encode sample size.
% \jessica{maybe also motivate why treatment effect in count data is reasonable given visual analytics settings?}


\subsection{Method}
We set out to study how well different visualizations support causal reasoning by using \textit{causal support} as a benchmark for causal inferences.


\subsubsection{Task scenario}
% In our task,
Participants played the role of an analyst hired by a company to interpret samples of data on the effectiveness of experimental treatments at preventing various diseases. %\jessica{could describe the simulated elsewhere since its a little ambiguous whether you mean we told them simulated}
We showed participants visualizations of the number of people in each sample who did or did not receive \textit{treatment}, get a \textit{disease}, and have a \textit{gene} known to cause the disease.
% in 50\% of people who have it.
% 2x2 contingency tables where rows encoded whether or not people in the sample had a gene known to cause cancer in 30\% of people who have it, columns encoded whether or not the same people received immunotherapy, and each cell of the table layout contained a visualization showing how many of those people did and did not develop cancer.

We asked participants to judge the underlying causal relationships in the data, rating their degree of belief that treatment protects against disease by allocating probability across the two DAGs in Figure~\ref{fig:dags-e1-explainer}.

\noindent
\textbf{Question \& Elicitation.}
We asked participants the following question: 
\begin{quote}
    \vspace{0mm}
    \textit{\textbf{How much do you believe in each of the causal explanations described below?} Imagine you have 100 votes to allocate across the two possible explanations. Split your 100 votes between explanations based on your degree of belief. For example, if you think one explanation is twice as likely as the other, you might give 67 votes (roughly two thirds) to that explanation and 33 votes (roughly one third) to the other. Assume no other explanations are possible.}
\end{quote}
\vspace{-3pt}
\noindent
Participants responded with two complementary probabilities. We used form validation to make sure their responses were both numbers between 0 and 100 that summed to 100.
Following prior work on eliciting Dirichlet distributions~\cite{Chalone1987,OHagan2006} (i.e., probabilities allocated across alternatives), when participants gave their first response, we imputed what the second response would need to be in order for their responses to sum to 100. This imputed value and a corresponding prompt, \textit{``Adjust your responses until both numbers reflect your beliefs.''}, were both highlighted with the same color to indicate this imputation.
We elicited probabilities as ``votes out of 100'' because \textit{frequency framing} tends to reduce bias in probability estimates~\cite{Gigerenzer1995,Hoffrage1998,OHagan2006}.
Participants received no feedback on their responses.
We combined these subjective probabilities ($\mathit{response_A}$ and $\mathit{response_B}$) into an estimate of perceived causal support, which we compared to our normative benchmark. 
% \yifan{maybe you should also mention that they were not given feedback on the correctness of their response during the experiment? As a reader i would find it relevant}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/explainer-dag-01.png}
    % \setlength{\intextsep}{-20pt}
    \setlength{\abovecaptionskip}{-10pt}
    \setlength{\belowcaptionskip}{-18pt}
    \caption{DAGs representing possible causal explanations participants were asked to consider in Experiment 1.
    }
    \label{fig:dags-e1-explainer}
\end{figure}

\noindent
\textbf{Payment.}
Participants received a \textit{guaranteed reward of \$2 for participating} plus a bonus of \$0.25 for every trial where their estimate of the probability of causal explanation A was within 5 votes of the ground truth derived from our model of causal support.


\begin{wrapfigure}{r}{0.4\columnwidth}
    \vspace*{-4mm}
    \centering
    \includegraphics[width=0.4\columnwidth]{figures/vis-conditions_text.png}
    \setlength{\abovecaptionskip}{-7pt}
    \setlength{\belowcaptionskip}{-7pt}
    \caption{Text tables.}
    \label{fig:text}
    
    \vspace*{4mm}
    \centering
    \includegraphics[width=0.4\columnwidth]{figures/vis-conditions_icons.png}
    \setlength{\abovecaptionskip}{-7pt}
    \setlength{\belowcaptionskip}{-7pt}
    \caption{Icon arrays.}
    \label{fig:icons}
    
    % \vspace*{3mm}
    % \centering
    % \includegraphics[width=0.4\columnwidth]{figures/vis-conditions_bars.png}
    % \setlength{\abovecaptionskip}{-5pt}
    % \setlength{\belowcaptionskip}{-7pt}
    % \caption{Bar charts.}
    % \label{fig:bars}
    
    % \vspace*{3mm}
    % \centering
    % \includegraphics[width=0.4\columnwidth]{figures/vis-conditions_aggbars.png}
    % \setlength{\abovecaptionskip}{-12pt}
    % \setlength{\belowcaptionskip}{-12pt}
    % \caption{Aggregating bars.}
    % \label{fig:aggbars}
    
    % \vspace*{3mm}
    % \centering
    % \includegraphics[width=0.4\columnwidth]{figures/vis-conditions_filtbars.png}
    % \setlength{\abovecaptionskip}{-5pt}
    % \setlength{\belowcaptionskip}{-7pt}
    % \caption{Cross-filter bars.}
    % \label{fig:filtbars}
\end{wrapfigure}
% \yifan{The text in these figures are pretty hard to read without zooming in, and the reader might want to actually read.} 
% \jessica{should we make the figure one figure with labeled panels so that we don't have to deal with the separate captions splitting things?}

\subsubsection{Visualization conditions}
Our visualizations show the number of people with and without disease in each cell of a 2x2 contingency table faceted by treatment and gene, with the exception of cross-filter bars which use a different layout.
We aimed to test visualizations of count data similar to what an analyst could produce using visual analytics software like Tableau.

\noindent
\textbf{Text.}
The text condition showed the number of people with disease as a fraction of the total number of people in each cell of the faceted table (Fig.~\ref{fig:text}).
Text tables, which have been studied in prior psychology research on causal support, served as a baseline comparison for other visualizations.

\noindent
\textbf{Icon arrays.}
Icon arrays showed counts of people with and without disease as filled and open circles, respectively (Fig.~\ref{fig:icons}). 
We set the number of dot columns to minimize the aspect ratio on each trial, similar to how analysts might create roughly square icon arrays in Tableau.
Icon arrays express both proportion and sample size as natural frequencies, which prior work suggests should aid in statistical reasoning (e.g., ~\cite{Galesic2009, Gigerenzer1995,Hoffrage1998}).

\noindent
\textbf{Bars.}
Grouped bar charts showed counts of people with and without disease using a length/position encoding on a common scale (Fig.~\ref{fig:aggbars}, top only).
On each trial, we set the $y$-axis scale to the maximum count of the data in view, allowing scales to change from trial to trial as they do when users load a new data set in Tableau. %We made the same design choice with the axis scales in every variation of bar charts (see below). 
Grouped bar charts are ubiquitous for showing count data.

\begin{wrapfigure}{r}{0.4\columnwidth}
    \vspace*{-7mm}
    \centering
    \includegraphics[width=0.4\columnwidth]{figures/vis-conditions_aggbars.png}
    \setlength{\abovecaptionskip}{-12pt}
    \setlength{\belowcaptionskip}{-12pt}
    \caption{Aggregating bars.}
    \label{fig:aggbars}
\end{wrapfigure}

\noindent
\textbf{Aggregating bars.}
Aggregating bars were similar to grouped bar charts (above), however, users could interactively control data aggregation by clicking on the table headers to toggle faceting by treatment or gene (Fig.~\ref{fig:aggbars}).
We designed this interaction to roughly mirror Tableau's shelf interactions, where users control faceting by direct manipulation of table headers.
% Interactive faceting might assist in causal inferences because whether or not data looks the same when collapsing over and grouping by a factor is a statistically valid signal as to whether that factor has a causal effect~\cite{Greenland1999}.
Interactive faceting may facilitate causal inferences by enabling users to explore whether ``collapsing''~\cite{Greenland1999} over a factor changes patterns in the data.

\noindent
\textbf{Cross-filtering bars.}
Three grouped bar charts show the number of people with and without treatment, the gene, and disease, respectively (Fig.~\ref{fig:filtbars}).
We linked these bar charts such that clicking on one bar cross-filtered the rest of the data in view.
When users apply a filter (e.g., to only show data for people who received treatment), the corresponding axis label becomes bold, and 
% to signal which filters the user has applied.Additionally, 
gray bars persist in the background 
% behind the filtered bars 
so that chart users do not need to rely on working memory to compare filtered and unfiltered views. 
Users ``reset filters'' by clicking a button below the charts.
% Unlike our other visualizations, cross-filtering bars did not use a two-way table layout. 
% We implemented three linked bar charts to 
Filterbars emulate coordinated multiple views such as analysts might create in a Tableau dashboard.
Interactive cross-filtering might assist in causal inferences because conditioning the data in view based on a specific event is analogous to Pearl's \textit{do operator} (e.g.,~$\mathrm{do}(\mathit{treatment}=\mathrm{yes})$), a notation for expressing and reasoning with counterfactual interventions in a causal networks~\cite{Pearl2018}.

\begin{figure}[h]
    \vspace*{-3mm}
    \centering
    \includegraphics[width=\columnwidth]{figures/vis-conditions_filtbars-big.png}
    \setlength{\abovecaptionskip}{-5pt}
    \setlength{\belowcaptionskip}{-7pt}
    \caption{Cross-filter bars. 
    % \alex{Need to shrink cursor to match aggbars}
    }
    \label{fig:filtbars}
\end{figure}


\subsubsection{Modeling causal support}
We operationalized the ground truth for causal inferences using Griffiths and Tenenbaum's \textit{causal support}, a Bayesian cognition model that estimates the posterior log odds of a set of possible data generating models given a data set.
In Experiment 1, we defined causal support:
\begingroup
\setlength\abovedisplayskip{3pt}
\setlength\belowdisplayskip{3pt}
    \begin{flalign*}
    \setlength\abovedisplayskip{0pt}
    \setlength\belowdisplayskip{0pt}
    \mathit{causal\_support_A} &= \log \bigg( \frac{\Pr(\mathit{model_A}|\mathit{data})}{\Pr(\mathit{model_B}|\mathit{data})} \bigg) \\
    &= \log \bigg( \frac{\Pr(\mathit{data}|\mathit{model_A})}{\Pr(\mathit{data}|\mathit{model_B})} \bigg) + \log \bigg( \frac{\Pr(\mathit{model_A})}{\Pr(\mathit{model_B})} \bigg)
    \end{flalign*}
\endgroup
where $\mathit{data}$ is a data set, and models $\mathit{model_A}$ and $\mathit{model_B}$ correspond to causal explanations A and B (Fig.~\ref{fig:dags-e1-explainer}).
Thus, we calculated causal support for explanation A ($\mathit{causal\_support_A}$) by adding together a log likelihood ratio for how strongly a data set corresponds with each generative model
and a log ratio of the prior probability for each model. \jessica{We assume equal prior probability per model to simplify the communication of the prior to participants.}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/causal-support-parameterization_final.png}
    \setlength{\intextsep}{-20pt}
    \setlength{\abovecaptionskip}{-10pt}
    \setlength{\belowcaptionskip}{-17pt}
    \caption{Causal support model, used to calculate normative baseline and to generate data for stimuli. Each formula gives probability of disease $\mathit{Ds}$ or no disease $\neg \mathit{Ds}$ contingent on a person having the gene $G$ or no gene $\neg G$ and treatment $T$ or no treatment $\neg T$.
    }
    \label{fig:parameterization}
\end{figure}

\jessica{part of what might be confusing here is that we sort of imply a dataset is getting generated in all this, but its not exactly clear how many datasets and what we define prior to sampling to get data}

To calculate the likelihood of each model $\Pr(\mathit{data}|\mathit{model_A})$ and $\Pr(\mathit{data}|\mathit{model_B})$ \jessica{given what? there has to be some type of input right?}, we parameterized a set of structural equations for each of the eight possible outcomes in our task (Fig.~\ref{fig:parameterization}). 
These structural equations had three parameters: $\Pr(\mathcal{D}|G)$ the probability of getting disease given that one has the gene; $\Pr(\mathcal{D})$ the base rate of disease due to unexplained causes; and $\Pr(\neg \mathcal{D}|T)$ the probability that treatment prevents disease.
% These structural equations had three parameters: $\textcolor{r}{\Pr(\mathcal{D}|G)}$ the probability of getting disease given that one has the gene; $\textcolor{b}{\Pr(\mathcal{D})}$ the base rate of disease due to unexplained causes; and $\textcolor{g}{\Pr(\neg \mathcal{D}|T)}$ the probability that treatment prevents disease.
We estimated log likelihood of each causal explanation using Monte Carlo integration to marginalize over possible parameter values. \jessica{maybe we should first say what parameter values we considered; these first few sentences where we jump into explaining are kind of abstract. Is there a higher level description we could give first of process like, We define distributions of values for these parameters, then we repeatedly sample from these distributions (to ensure the data we show participants are not especially extreme samples), etc (my exact words are probably wrong, but somethings like this } 
Specifically, we drew 10,000 uniformly distributed samples for each parameter on the interval $[0, 1]$, passed these samples through the formulae in Figure~\ref{fig:parameterization}) to get probabilities for each possible outcome in the data set, \jessica{What is a possible outcome and what is the dataset?} used these probabilities to calculate 10,000 likelihood estimates for the data set, \jessica{what is the dataset? how many datasets did we make?} and then averaged over these likelihoods.
This Monte Carlo integration enabled us to estimate the likelihood of each data set \jessica{can we lay out our goals explicitly at the beginning of this section - how many datasets did we want to create, and how much variation did we want in the key parameters?} that we showed participants under each alternative data generating model without necessarily estimating the parameters themselves. \jessica{reader might not get the point of this last part, if there's another way to explain might help}
% \jessica{Doing so provides a more realistic representation of uncertainty inherent in data samples (or something like that to motivate?)}
% \jessica{have we mentioned what the parameter values were set to or say these are in supplemental material and make clear we set each to a single value?}
%\jessica{so there is no added uncertainty through sampling here, or is there?} \alex{We run 10000 simulations, so the log likelihoods we get are probably pretty accurate.}
Under $\mathit{model_A}$ we sampled all three parameters uniformly in our Monte Carlo simulation, representing the assumptions that there is a treatment effect and that both gene and unobserved factors cause disease. %\jessica{this part is still a little unclear maybe bc im unclear on parameter values we set}
\jessica{should the prev sentence be said earlier? reading above I was lacking a sense of what we wanted in our datasets}
Under $\mathit{model_B}$ we sample $\Pr(\mathcal{D}|G)$ and $\Pr(\mathcal{D})$ uniformly, but we fix $\Pr(\neg \mathcal{D}|T)$ at zero representing an assumption of no treatment effect. 
% Under $\mathit{model_B}$ we sample $\textcolor{r}{\Pr(\mathcal{D}|G)}$ and $\textcolor{b}{\Pr(\mathcal{D})}$ uniformly, but we fix $\textcolor{g}{\Pr(\neg \mathcal{D}|T)}$ at zero representing an assumption of no treatment effect. 
%\jessica{can we motivate this at all or say why we don't think this is a critical choice that could eg explain why ppls inferences are so far off from causal support?}
Thus, we simulated alternative hypothetical data generating processes in order to calculate their relative compatibility with the data. \jessica{this seems like a useful sentence for providing high level description of what we are doing, should it go earlier?}

% \yifan{Would be good to provide more intuitive description rather than just relying on the math. Also I'm a little confused by the math---isn't it Pr(m\_a|D) = Pr(D|m\_A)Pr(m\_A) / (Pr(D|m\_A)Pr(m\_A) + Pr(D|m\_B)Pr(m\_B))? and not Pr(m\_a|D) = Pr(D|m\_A)Pr(m\_A) /Pr(D|m\_B)Pr(m\_B) as suggested?} \alex{This is a really great question! I'm just following the math from G\&T, equation 9. However, I'm not sure why the update formula is posed as an an odds ratio rather than as probabilities. I tried to clean up the notation, and I provide a more intuitive description of Bayesian structure learning in the last sentence of this paragraph.}
% Note causal support is a likelihood for Bayesian structure learning. \jessica{have we defined this latter part?}
% Full Bayesian inference incorporates a prior assigning probability to each model---$\Pr(model_A)$ and $\Pr(model_B)$, respectively---in addition to log likelihood. 
% \begingroup
% \setlength\abovedisplayskip{3pt}
% \setlength\belowdisplayskip{3pt}
%     $$\log \bigg( \frac{\Pr(model_A|D)}{\Pr(model_B|D)} \bigg) = \log \bigg( \frac{\Pr(D|model_A)}{\Pr(D|model_B)} \bigg) + \log \bigg( \frac{\Pr(model_A)}{\Pr(model_B)} \bigg)$$
% \endgroup
Following Griffiths and Tenenbaum~\cite{Griffiths2005}, we assume a uniform prior across possible data generating models to be normative. 
Since there were only two alternative explanations in Experiment 1, we calculated ground truth causal support using the \textit{log prior ratio} ($\mathit{lpr_A}$), %\yifan{maybe add a paren around lpr to make it more readable? also later for lrr.}
\begingroup
\setlength\abovedisplayskip{3pt}
\setlength\belowdisplayskip{3pt}
    \begin{flalign*}
    \setlength\abovedisplayskip{0pt}
    \setlength\belowdisplayskip{0pt}
    \mathit{lpr_A} &= \log \bigg( \frac{\Pr(\mathit{model_A})}{\Pr(\mathit{model_B})} \bigg) = \log \bigg( \frac{0.5}{0.5} \bigg) = 0
    \end{flalign*}
\endgroup
% \yifan{why not squeeze them into one line to save space?}
which factors out of the formula for causal support, making the likelihood itself the normative posterior for Experiment 1.
In Experiment 2, where there are four alternative causal explanations, the prior will not factor out of the normative update in the same way.
One can think of the prior as encoding a systematic bias in belief allocation across a finite set of alternative causal explanations.
We assume uniform priors in defining causal support because we want our benchmark to reflect no \textit{a priori} bias towards any particular causal explanation.\footnote{Uniform priors follow a convention of psychometric models that assume guessing responses are informed by the number of response alternatives~\cite{Kingdom2010}.} 

\jessica{this chunk on priors makes me think we need more structure in this section. Like, define causal support as you do in the beginning, maybe then put this prior part, maybe with other things we decided related to our goals for hte datasets we create. Then we have a subsection called Dataset Generation Process or something like that which is just the order in which we did what steps.}
% \jessica{if there's any way to evaluate this assumption of uniform (though I'm not sure there is), we might mention we later explore it here. Its clearly an assumption we are making so we may want at least a brief motivation as well}
% \jessica{Also might help readability slightly to capitalize Experiment 1 Experiment 2. But up to you}
% For this reason, we directly compared participant responses to causal support, but applying this method with more than two alternative models requires adding a log ratio of priors (see Experiment 2).
% In summary, combining causal support and a uniform prior provided us with a normative estimate for the posterior log odds of explanation A rather than explanation B (Fig.~\ref{fig:dags-e1-explainer}), which is a transformation of the probability of a treatment effect given the data that we presented on each trial. \jessica{this explanation might be a little hard for readers to grasp, especially second sentence}


% \begin{algorithm}[H]
%   \caption{
%       Monte Carlo simulation to calculate causal support in Experiment 1. Algorithm for Experiment 2 is similar.
%   }
%   \label{alg:monte_carlo}
% \begin{algorithmic}[1]
%     \Input contingency table counts for no disease vs disease given no gene vs gene and no treatment vs treatment as a (8,1) vector $C$, Monte Carlo iterations $m$, set of parameters to fix at zero $\theta_0$
%     \Output log likelihood of data generating process with parameters $\theta_0$ fixed at zero $\mathit{log\_lik}$
%     \item \textcolor{purple}{\texttt{\textbf{\# Monte Carlo simulation to calculate likelihood}}} \setcounter{ALC@line}{1}
%     \SubAlgorithm{monte\_carlo}{($C$, $m$, $\theta_0$):}
%         \STATE \hspace{\algorithmicindent} Parameters corresponding to each possible DAG arrow in Fig.~\ref{fig:dags-e1-explainer}: \\
%         \hspace{\algorithmicindent} $\theta_\mathcal{P} = \{$ \textcolor{red}{\texttt{\ \ \ \ \# initialize parameters}} \\
%         \hspace{2\algorithmicindent}  $\Pr(\mathcal{D})$, \textcolor{red}{\texttt{\ \ \ \# p disease due to unknown causes}} \\
%         \hspace{2\algorithmicindent} $\Pr(\mathcal{D}|G)$, \textcolor{red}{\texttt{\ \# p disease due to gene}} \\
%         \hspace{2\algorithmicindent} $\Pr(\neg \mathcal{D}|T)$ \textcolor{red}{\texttt{\# p no disease due to treatment}} \\
%         \hspace{\algorithmicindent} $\}$ \setcounter{ALC@line}{3}
%         \For{parameter $\theta \in  \theta_\mathcal{P}$} \textcolor{red}{\texttt{\ \# assign parameters}} \setcounter{ALC@line}{4}
%             \If{$\theta \in \theta_0$} Fix parameter at zero: $\theta = \mathrm{Zeros(}m\mathrm{)}$ \setcounter{ALC@line}{5}
%             \Else{} Uniformly sample probabilities: $\theta = \mathrm{Random(}0,1,m\mathrm{)}$ \setcounter{ALC@line}{6}
%             \EndIf{}
%         \EndFor{}
%         \STATE \hspace{\algorithmicindent} Calculate probabilities corresponding to contingency table: \\
%         \hspace{\algorithmicindent} $\mathcal{P} = [$ \textcolor{red}{\texttt{\ \# probability of each possible outcome}} \\
%         \hspace{2\algorithmicindent} $\big(1 - \Pr(\mathcal{D})\big)$, \\ %\textcolor{green}{\texttt{\# $\Pr(\neg\mathcal{D} \mid \neg G, \neg T)$}} \\
%         \hspace{2\algorithmicindent} $\Pr(\mathcal{D})$, \\
%         \hspace{2\algorithmicindent} $\big(1 - \Pr(\mathcal{D})\big) + \Pr(\mathcal{D}) \cdot \Pr(\neg \mathcal{D}|T)$, \\
%         \hspace{2\algorithmicindent} $\Pr(\mathcal{D}) \cdot \big(1 - \Pr(\neg \mathcal{D}|T)\big)$, \\
%         \hspace{2\algorithmicindent} $\big(1 - \Pr(\mathcal{D} \mid G)\big) \cdot \big(1 - \Pr(\mathcal{D})\big)$, \\
%         \hspace{2\algorithmicindent} $\Pr(\mathcal{D} \mid G) + \Pr(\mathcal{D}) - \Pr(\mathcal{D} \mid G) \cdot \Pr(\mathcal{D})$, \\
%         \hspace{2\algorithmicindent} $\big(\Pr(\mathcal{D} \mid G) + \Pr(\mathcal{D}) - \Pr(\mathcal{D} \mid G) \cdot \Pr(\mathcal{D})\big) \cdot \Pr(\neg \mathcal{D}|T) +$ \\ \hspace{3\algorithmicindent} $\big(1 - \Pr(\mathcal{D} \mid G)\big) \cdot \big(1 - \Pr(\mathcal{D})\big)$, \\
%         \hspace{2\algorithmicindent} $\big(\Pr(\mathcal{D} \mid G) + \Pr(\mathcal{D}) - \Pr(\mathcal{D} \mid G) \cdot \Pr(\mathcal{D})\big) \cdot \big(1 - \Pr(\neg \mathcal{D}|T)\big)$ \\
%         \hspace{\algorithmicindent} $]$
%         \STATE \hspace{\algorithmicindent} \Return average log likelihood of data: \\
%         \hspace{\algorithmicindent} $\mathit{log\_lik} = \sum_{i \in \{1,...,m\}}{\sum{\big(C \cdot \log(\mathcal{P})\big)}} - \log(m)$
%     \EndSubAlgorithm{} \setcounter{ALC@line}{9}
%     \item \textcolor{purple}{\texttt{\textbf{\# Main: causal support calculation}}}
%     \STATE Run Monte Carlo simulations to get likelihood of data given each causal explanation in Fig.~\ref{fig:dags-e1-explainer}: \\
%     $\mathit{log\_lik}_A = \textsc{monte\_carlo}(C, 10000, \{\})$ \\
%     $\mathit{log\_lik}_B = \textsc{monte\_carlo}(C, 10000, \{\Pr(\neg \mathcal{D}|T)\})$
%     \STATE \Return causal support for explanation: \textcolor{red}{\texttt{\ \# Bayesian update }}\\
%     $\mathit{causal\_support}_A = \big(\mathit{log\_lik}_A - \mathit{log\_lik}_B\big) + \big(\log(0.5) - \log(0.5)\big)$
% \end{algorithmic}
% \end{algorithm}

\begin{algorithm}[H]
  \caption{
      Monte Carlo simulation to calculate causal support in Experiment 1. Algorithm for Experiment 2 is similar.
  }
  \label{alg:monte_carlo}
\begin{algorithmic}[1]
    \Input (8, 1) vector of contingency table counts (no disease vs disease, no gene vs gene, no treatment vs treatment) $C$, Monte Carlo iterations $m$, set of parameters to fix at zero $\theta_0$ (i.e., parameters representing DAG arrows to omit from the data generating process)
    \Output \textsc{{monte\_carlo}} returns log likelihood of the given data generating process $\mathit{log\_lik}$; Main returns causal support for the target explanation (Fig.~\ref{fig:dags-e1-explainer}, Explanation A) $\mathit{causal\_support}_A$ 
    \item \textcolor{purple}{\texttt{\textbf{\# Monte Carlo simulation to calculate likelihood}}}
    \SubAlgorithm{monte\_carlo}{($C$, $m$, $\theta_0$):} \\
        \STATE \hspace{\algorithmicindent} Parameters corresponding to each DAG arrow in Fig.~\ref{fig:dags-e1-explainer}: \\
        \hspace{\algorithmicindent} $\theta_\mathcal{P} = \{$ \textcolor{red}{\texttt{\ \ \ \ \ \# initialize parameters}} \\
        \hspace{\algorithmicindent} \hspace{\algorithmicindent}  $\Pr(\mathcal{D})$, \textcolor{red}{\texttt{\ \ \ \# p disease due to unknown causes}} \\
        \hspace{\algorithmicindent} \hspace{\algorithmicindent} $\Pr(\mathcal{D}|G)$, \textcolor{red}{\texttt{\ \# p disease due to gene}} \\
        \hspace{\algorithmicindent} \hspace{\algorithmicindent} $\Pr(\neg \mathcal{D}|T)$ \textcolor{red}{\texttt{\# p no disease due to treatment}} \\
        \hspace{\algorithmicindent} $\}$
        \For{parameter $\theta \in  \theta_\mathcal{P}$} \textcolor{red}{\texttt{\ \# assign parameters}}
            \If{$\theta \in \theta_0$} Fix parameter at zero: $\theta = \mathrm{Zeros(}m\mathrm{)}$
            \Else{} Uniformly sample probabilities: $\theta = \mathrm{Random(}0,1,m\mathrm{)}$
            \EndIf{}
        \EndFor{} \\
        \STATE \hspace{\algorithmicindent} Calculate probabilities corresponding to contingency table: \\
        \hspace{\algorithmicindent} $\mathcal{P} = [$ \textcolor{red}{\texttt{\ \ \ \# p no disease vs p disease given...}} \\
        \hspace{\algorithmicindent} \hspace{\algorithmicindent} $\big(1 - \Pr(\mathcal{D})\big)$, \textcolor{red}{\texttt{\ \ \ \# no treat $\neg T$, no gene $\neg G$}} \\ %\textcolor{green}{\texttt{\# $\Pr(\neg\mathcal{D} \mid \neg G, \neg T)$}} \\
        \hspace{\algorithmicindent} \hspace{\algorithmicindent} $\Pr(\mathcal{D})$, \\
        \hspace{\algorithmicindent} \hspace{\algorithmicindent} $\big(1 - \Pr(\mathcal{D})\big) + \Pr(\mathcal{D}) \cdot \Pr(\neg \mathcal{D}|T)$, \textcolor{red}{\texttt{\ \ \ \ \ \# $T$, $\neg G$}} \\
        \hspace{\algorithmicindent} \hspace{\algorithmicindent} $\Pr(\mathcal{D}) \cdot \big(1 - \Pr(\neg \mathcal{D}|T)\big)$, \\
        \hspace{\algorithmicindent} \hspace{\algorithmicindent} $\big(1 - \Pr(\mathcal{D} \mid G)\big) \cdot \big(1 - \Pr(\mathcal{D})\big)$, \textcolor{red}{\texttt{\ \ \ \ \ \ \ \# $\neg T$, $G$}}\\
        \hspace{\algorithmicindent} \hspace{\algorithmicindent} $\Pr(\mathcal{D} \mid G) + \Pr(\mathcal{D}) - \Pr(\mathcal{D} \mid G) \cdot \Pr(\mathcal{D})$, \\
        \hspace{\algorithmicindent} \hspace{\algorithmicindent} $\big(\Pr(\mathcal{D} \mid G) + \Pr(\mathcal{D}) - \Pr(\mathcal{D} \mid G) \cdot \Pr(\mathcal{D})\big)$ \textcolor{red}{\texttt{\# $T$, $G$}} \\ \hspace{\algorithmicindent} \hspace{\algorithmicindent} \hspace{\algorithmicindent} $\cdot \Pr(\neg \mathcal{D}|T) + \big(1 - \Pr(\mathcal{D} \mid G)\big) \cdot \big(1 - \Pr(\mathcal{D})\big)$, \\
        \hspace{\algorithmicindent} \hspace{\algorithmicindent} $\big(\Pr(\mathcal{D} \mid G) + \Pr(\mathcal{D}) - \Pr(\mathcal{D} \mid G) \cdot \Pr(\mathcal{D})\big)$ \\ \hspace{\algorithmicindent} \hspace{\algorithmicindent} \hspace{\algorithmicindent} $\cdot \big(1 - \Pr(\neg \mathcal{D}|T)\big)$ \\
        \hspace{\algorithmicindent} $]$ \\
        \STATE \hspace{\algorithmicindent} \Return average log likelihood of data: \\
        \hspace{\algorithmicindent} $\mathit{log\_lik} = \sum_{i \in \{1,...,m\}}{\sum{\big(C \cdot \log(\mathcal{P})\big)}} - \log(m)$
    \EndSubAlgorithm{} \\
    \item \textcolor{purple}{\texttt{\textbf{\# Main: causal support calculation}}} \\
    \STATE Run Monte Carlo simulations to get likelihood of data given each causal explanation in Fig.~\ref{fig:dags-e1-explainer}: \\
    $\mathit{log\_lik}_A = \textsc{monte\_carlo}(C, 10000, \{\})$ \\
    $\mathit{log\_lik}_B = \textsc{monte\_carlo}(C, 10000, \{\Pr(\neg \mathcal{D}|T)\})$ \\
    \STATE \Return causal support for explanation A: \textcolor{red}{\texttt{\ \# Bayesian update }}\\
    $\mathit{causal\_support}_A = \big(\mathit{log\_lik}_A - \mathit{log\_lik}_B\big) + \big(\log(0.5) - \log(0.5)\big)$
\end{algorithmic}
\end{algorithm}


\subsubsection{Experimental design \& stimuli}
We manipulated both the visualizations participants used for the task and the data that we showed participants.
We randomly assigned each participant to use one of five visualizations (see Section 3.1.2), making comparisions of visualizations between-subjects.

Our goal was to test each visualization condition on realistic-looking data sets, which spanned
% varied in both the apparent treatment effect and the overall amount of data shown, resulting in trials that span 
a range of ground truth causal support.
The visual attributes of the data which signaled causal support were delta p and sample size.
% We designed our stimuli not only to sample causal support itself but also the visual attributes of the data which signaled causal support for a treatment effect, delta p and sample size. 
\textit{Delta p} described the difference in the proportion of people with disease in each data set depending on whether they received treatment.
Positive values of delta p indicated evidence that the treatment protected against disease; negative values indicated evidence against treatment effectiveness.
\textit{Sample size} was the number of people in each data set we showed participants.

% We randomly assigned each participant to use one of five visualizations (see Section 3.1.2).
% \jessica{this description is a little confusing - are we only interested in vis comparisons, or should we motivate sample size as a condition we vary? Like more motivation of why we choose to vary what we vary and which ones are for realism/getting more robust estimates across vis versus effects we are specifically interested in estimating } 
% Comparisons between visualizations were between-subjects.
% Participants made repeated judgments for 16 trials.

We showed each participant 16 data conditions generated from unique combinations of two factors: \textit{probability that treatment prevents disease} (4 levels: $\{0, 0.1, 0.2, 0.4\}$) and \textit{sample size} (4 levels: $\{100, 500, 1000, 1500\}$). 
\jessica{I think the detail about the data conditions needs to come earlier, before we describe data generation process. Can just be a single sentence, like Our goal was to generate 16 data conditions (which become trials in our experiment) that varied two factors: .... This will give some needed context on our goals in the descdription of the dataset generation. Actually should probably just describe data generation with modeling causal support. Otherwise its very hard to figure out how they go together}
% We generated the data sets shown to participants on each trial using unique combinations of two factors: \textit{probability that treatment prevents disease} (4 levels: $\{0, 0.1, 0.2, 0.4\}$) and \textit{sample size} (4 levels: $\{100, 500, 1000, 1500\}$).
For each of these 16 data conditions, we simulated many data sets using a binomial random number generator to approximate realistic sampling error.
By simulating sampling error, we prevented the count data from appearing contrived.
Because of this sampling error, ground truth causal support was not a deterministic function of the factors used to generate the data.
In order to guarantee that each participant saw trials spanning a consistent range of causal support despite this sampling error, we counterbalanced the presentation of this sampling error across participants within each visualization condition.
% \jessica{in this section it might be useful to motivate why you do some things first more obviously since its pretty technical and some readers may not get it. E.g., be more specific that 'to control how we presented this sampling error', above maybe first point out why it would be somewhat weird not to include sampling error. basically if we have space spell some of these things out a little more}
% In order to control how we presented this sampling error, \jessica{In order to balance how much sampling error was shown across participants,} 
We selected a subset of data sets for each data condition representing 16 quantiles of causal support, and we counterbalanced which quantile was shown for each data condition across participants using a balanced latin square.
% Specifically, we filtered our simulated data sets for each data condition to a subset representing 16 quantiles of causal support, and we counterbalanced which quantile was shown for each data condition across participants using a balanced latin square.
% We used a balanced latin square to sample each pair of data condition and quantile uniformly across participants within visualization condition.
We randomized trial order for each participant.
% These within-subjects data manipulations provide realistic-looking fake data sets that span a range of ground truth causal support.  \jessica{you might consider saying this above so its clear at a high level what the goal is before you describe what you did (Maneesh was very picky about this actually - never say what you did until you've made clear why you had to)}

We presented two additional trials as attention checks.
We chose data sets for these trials that had the minimum and maximum ground truth causal support among our simulated data.
% These data showed clear patterns of treatments that hurt and help \jessica{and maybe say where reader can see them}. \yifan{hurt and help? are you going to talk more about the effects? If so please mention section forward reference, and if not, this is not enough info and we need to either add or remove completely}
We presented these attention checks on the 7th and 13th of 18 total trials, with order randomized.
% \yifan{what happens if they fail the attention checks?}
We used these attention checks for exclusion criteria (see Section 3.1.6).


\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/e1-interactions_final.png}
    % \setlength{\intextsep}{-20pt}
    \setlength{\abovecaptionskip}{-10pt}
    \setlength{\belowcaptionskip}{-17pt}
    \caption{Sensitivity (y-axes) conditioned on two attributes of visual signal for treatment effectiveness (rows, x-axes) and visualizations (columns).
    }
    \label{fig:e1-interactions}
\end{figure*}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/e1-main-effects_slopes.png}
    % \setlength{\intextsep}{-20pt}
    \setlength{\abovecaptionskip}{-10pt}
    \setlength{\belowcaptionskip}{-17pt}
    \caption{Linear in log odds (LLO) slopes per visualization condition.
    }
    \label{fig:e1-slopes}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/e1-main-effects_intercepts.png}
    % \setlength{\intextsep}{-20pt}
    \setlength{\abovecaptionskip}{-10pt}
    \setlength{\belowcaptionskip}{-17pt}
    \caption{LLO intercepts per visualization condition.
    }
    \label{fig:e1-intercepts}
\end{figure}


\subsubsection{Performance evaluation}
We wanted to measure how much participants' causal inferences deviated from our normative benchmark, causal support. 
% \yifan{s/chart user/participant?} nvm it seems to be in other places also

\noindent
\textbf{Perceived causal support.}
We compare participants' responses to causal support on a log odds scale.
This requires transforming responses into \textit{perceived causal support}, a log response ratio ($\mathit{lrr_A}$),
\begingroup
\setlength\abovedisplayskip{3pt}
\setlength\belowdisplayskip{3pt}
    $$\mathit{lrr_A} = \log \bigg( \frac{\mathit{response_A}}{\mathit{response_B}} \bigg)$$
\endgroup
where $\mathit{response_A}$ and $\mathit{response_B}$ were the probabilities participants allocated to causal explanations A and B, respectively, on each trial.
% \jessica{could move next sentence to the below paragraph, since when i first read it i was thinking that's all you were to going to say about lrr} By choosing to model $lrr$ as a function of normative causal support on a log odds scale, we leverage a linear in log odds model to extend causal support from a normative cognitive model into a descriptive one. \jessica{maybe also give some general motivation for why people do log ratios, eg log odds are symmetric around 50\% which helps interpretation? } \alex{That's what the following section is about.}
% \alex{motivation here!}
% We chose the LLO model both for its basis in theoretical models of perception~\cite{Gonzalez1999,Hollands2000,Stevens1957,Zhang2012} and because using a LLO model with causal support as a predictor effectively extends causal support from a normative cognitive model to a descriptive one.

\noindent
\textbf{The linear in log odds model \& causal support.}
By choosing to model $\mathit{lrr_A}$ as a function of normative causal support on a log odds scale, we leverage a linear in log odds (LLO) model to extend causal support from a normative cognitive model into a descriptive one.
Prior work shows that the LLO model accurately describes natural distortions in mental representations of probability~\cite{Gonzalez1999,Hollands2000,Stevens1957,Zhang2012}.
For example, Zhang et al.~\cite{Zhang2012} apply the LLO model to reanalyze data from multiple experiments involving a variety of judgments of probabilities and proportions, finding that the functional relationship between actual and perceived proportions seems to be ubiquitously LLO.
Related literature in visualization~\cite{Kale2021} uses the LLO model to measure perceptual distortions in probabilistic judgments about intervention effectiveness.
Our normative model of causal support itself (see Section 3.1.3) is a LLO model, 
% where we compute causal support as 
a sum of likelihoods and priors in log odds units.

We use a LLO model to measure the correspondence between normative and perceived causal support.
This enables us to estimate participants' \textit{sensitivity} to changes in ground truth causal support and \textit{bias} in perceived causal support. 
% By using a LLO model to describe perceived causal support $lrr$ as a function of normative causal support, we learn (1) \textit{how sensitive chart users are to causal support}---the weight they assign to changes in the ground truth log likelihood ratio of causal explanation A rather than explanation B---and (2) \textit{how biased chart users are in their causal inferences}---the average prior probability of causal explanation A which they appear to add to their judgments in log odds units. \jessica{this section is asking the reader to process a lot of abstract info at once (what is LLO and how does it relate to our study), in a way that makes me have to reread it multiple times. i wonder if there's a slightly more direct way to give an intuition for LLO first, like (if my understanding is correct), At a high level, an LLO model enables estimating \textit{bias} in perceived probability (i.e., when the ground truth is 50\%, what is the users' perceived probaiblity predicted to be), as well as their \textit{sensitivity} to changes in the underlying probabilities (i.e., do their perceived probabilities change less or more than they should with the ground truth probability? ) Then can say how in our study bias is about difference in log likelihood A vs B etc}
From our model, we derive sensitivity and bias per condition as \textit{LLO slopes and intercepts}, respectively.
LLO slopes describe sensitivity to ground truth causal support such that a slope of one indicates ideal sensitivity.
% a one-to-one relationship between participants' responses and our normative benchmark (i.e., ideal sensitivity). 
One can think of slopes as the weight participants assign to changes in the ground truth log likelihood ratio of causal explanation A rather than explanation B.
LLO intercepts describe bias in participants' probability allocations when causal support is zero such that an intercept of 50\% indicates no bias.
One can think of intercepts as the average prior probability that participants allocate to explanation A when there is no signal in the data.

% For ease of interpretation, we apply a logistic transform to intercepts and present them as expected probability assigned to explanation A given no signal in a data set.

\noindent
\textbf{Approach.}
We used the brms package~\cite{Burkner2020} in R to fit Bayesian hierarchical models on perceived causal support.
We adopted a Bayesian workflow called \textit{model expansion}~\cite{Gabry2019}, where we started with a simple model and iteratively added predictors to build up to more complex models, running prior predictive checks, model diagnostics, posterior predictive checks, and leave-one-out cross validation for each version of the model.
% This enabled us to understand increasingly complex models in terms of the simpler models they contain, while also helping us guard against needless complexity. \yifan{not sure if the prev sentence adds much; can trim if out of space?} \jessica{agree}
We centered each prior to reflect a null hypothesis of ideal performance and no bias, and we scaled each prior to be weakly informative while providing sufficient regularization for models to converge.
We provide more details about our modeling workflow in our preregistration\footnote{
We include an anonymized preregistration in Supplemental Materials for review. There is a version with author names on OSF. 
% https://osf.io/vzmhu
} and Supplemental Materials.\footnote{
% https://github.com/kalealex/causal-support
\texttt{Github repo omitted for anonymous review.}
}

\noindent
\textbf{Model specification.}
% \yifan{could you motivate the use of this model? Why is it not as simple as a point to point (two numeric value) comparison? Or something like a variance between the expected and the response? Or directly say some prior work used this model (instead of just citing the work and requiring the reader to research)} \alex{I added the motivation you are looking for above in the first paragraph of this subsection.}
We used the following model (Wilkinson-Pinheiro-Bates notation~\cite{Wilkinson1973,Burkner2020,Pinheiro2020}) to evaluate participants' responses: 
\begingroup
\setlength\abovedisplayskip{3pt}
\setlength\belowdisplayskip{3pt}
    \begin{flalign*}
    \setlength\abovedisplayskip{0pt}
    \setlength\belowdisplayskip{0pt}
    \mathit{lrr_A} \sim &\mathrm{Normal}(\mu_A, \sigma_A) \\[-2pt]
    \mu_A = &\mathit{causal\_support_A}*\mathit{delta\_p}*n*\mathit{vis} \\[-2pt]
        &+ \big(\mathit{causal\_support_A}*\mathit{delta\_p} + \mathit{causal\_support_A}*n\big|\mathit{worker\_id}\big)
    \end{flalign*}
\endgroup
% \yifan{maybe use the notation worker\_id?}
where $\mathit{lrr_A}$ was perceived causal support for a treatment effect based on participant responses, $\mathit{causal\_support_A}$ was our normative benchmark, $\mathit{delta\_p}$ was the difference in the proportion of people with disease given treatment versus no treatment, $n$ was the sample size as a factor, $\mathit{vis}$ was a dummy variable for visualization condition, and $\mathit{worker\_id}$ was a unique identifier for each participant.
% \jessica{the mu is slightly indented above}

We primarily modeled effects on the mean perceived causal support $\mu_A$, but our model also learned the residual standard deviation $\sigma_A$ of perceived causal support.
Both $\sigma_A$ and the random effects in the $\mu_A$ submodel helped account for the empirical distribution, differentiating between response noise and effects of interest.
The term $\mathit{causal\_support_A}*\mathit{delta\_p}*n*\mathit{vis}$ enabled our model to learn how the slope on causal support varies as a function of the visual signal on each trial---operationalized as $\mathit{delta\_p}$ and $n$---as well as visualization condition (i.e., all of these factors interacted with each other).
% We analyze these interacting slope effects to answer our research questions about the quality of causal inferences with different visualizations.

% \noindent
% \textbf{Linear in log odds slopes and intercepts.}
% From our model, we derived \textit{linear in log odds (LLO) slopes and intercepts}, which measured the correspondence between perceived and normative causal support.
% Specifically, \textit{slopes described sensitivity to ground truth causal support} such that a slope of one would mean a one-to-one relationship between the user's responses and our normative benchmark, indicating that participants were perfectly sensitive to the signal in charts when making causal inferences. 
% \textit{Intercepts described bias in users' subjective probability allocations when causal support was zero} such that an intercept of zero indicated no bias.
% For ease of interpretation, we apply a logistic transform to intercepts and present them as expected probability assigned to explanation A given no signal in a data set.

% A slope of one meant there was a one-to-one relationship between the user's responses and our normative benchmark, indicating that participants were perfectly sensitive to the signal in charts when making causal inferences. 
% Slopes less than one meant participants assigned less probability than they should to the most likely causal explanation; slopes greater than one meant participants assigned too much probability to the most likely causal explanation.
% Slopes less than one meant that participants were less confident than they should have been in attributing visual signal to causal explanations, and slopes greater than one meant participants were overconfident.
% In general, LLO slopes less than indicate bias toward the probability at the intercept, or the mean response, which was $avg response_A$ in E1.
% Because the LLO model represents natural distortions in subjective probabilities~\cite{Gonzalez1999,Zhang2012}, \jessica{again consider better motivating the natural part somewhere in this section} LLO slopes and intercepts describe deviance from ground truth causal support with greater statistical power than measures such as accuracy.
% though also we derive average error from our model to help interpret LLO slopes.


\subsubsection{Participants.}
We recruited participants on Amazon Mechanical Turk.
Workers had a HIT acceptance rate of at least 97\% and were located in the US.
We aimed to recruit a total of 400 participants after exclusions using our attention check trials, 80 per visualization condition. %\yifan{I don't remember reading exclusion criterion described anywhere?}
We determined this target sample size using a heuristic power analysis based on pilot data and the assumption that the width of confidence intervals would be inversely proportional to $\sqrt{N}$.
% We determined this target sample size using a heuristic power analysis based on pilot data and the assumption that the confidence intervals estimated from our model would shrink by a factor of about $\frac{1}{\sqrt{n}}$.
% We determined this target sample size by a heuristic power analysis, using data from a pilot study to estimate the magnitude of effect we wanted to reliably detect and assuming that posterior containment intervals (CIs, analogous to frequentist confidence intervals) estimated from our model would shrink by about $\frac{1}{\sqrt{n}}$ depending on sample size.
We recruited a total of 548 participants, and after exclusions we used data from 408 participants in our analysis. 
We slightly overshot our target sample size because we could not anticipate perfectly how many participants would miss our attention checks (see Section 3.1.4).
Although we preregistered that we would exclude participants who failed to allocate at least 50\% subjective probability to the most likely causal explanation on either attention check, this criterion proved too strict and would have excluded 48\% of our sample.
% Originally, we preregistered that we would exclude participants who missed either of two attention check trials (see Section 3.1.4), where we define a ``miss'' as a user failing to allocate more subjective probability to the most likely causal explanation than to any other. However, since one of our attention checks was more difficult than we intended, this criterion proved too strict and would have excluded 48\% of our sample.
Instead, we opted to use only the easier of the two attention checks for exclusions, resulting in the exclusion of 26\% of our sample.
% and leaving us with the final sample we used for data analysis.
All participants were paid regardless of exclusions.
We compensated the average participant \$2.50 for about 9 minutes.
% \jessica{maybe this could be shortened more}

==> archived/submission/4_e1-results.tex <==
\subsection{Results}
We compare chart users' causal inferences to a benchmark called causal support, using a linear in log odds (LLO) model to describe performance in terms of \textit{sensitivity} to the ground truth and \textit{bias} in probability allocations when each causal explanation is equally likely.
% Recall that our evaluation compares chart users' causal inferences to a normative benchmark called causal support using a linear in log odds (LLO) model. This allows us to describe performance in terms of \textit{sensitivity} to the ground truth and \textit{bias} in probability allocations when the ground truth is that each causal explanation is equally likely.

\noindent
\textbf{Sensitivity.}
A LLO slope of one indicates one-to-one correspondence between the ground truth and users' probability allocations.
In all visualization conditions (Fig.~\ref{fig:e1-slopes}), we see slopes far below one, indicating that users are much less sensitive than ideal.
% to the signal in the data.
On average, the only reliable difference between visualization conditions is that filterbars users who do not interact are less sensitive than users in other conditions. 
% The average user of each other visualization is more sensitive to signal than filterbars users who do not interact.
% Otherwise, differences in LLO slopes between visualization conditions are not reliable. 
% \yifan{prob better to call filtbars (Cross)FilterBars? Filt seems a littler too abbreviated to easily parse.}

When filterbars users do not interact with the charts, slopes are approximately zero indicating that users are insensitive to signal.
Performance improves reliably when users interact with the visualization by applying cross-filters to coordinated multiple views.
This is expected because filterbars hide visual signal for the task behind interactions.
% This is expected because filterbars hide the signal in charts behind interactions such that the task is impossible without interacting.

Surprisingly, when aggbars users interact with the charts to group by gene or treatment, this leads to lower sensitivity, though this difference is not reliable. %\yifan{delete on or "group by"/"collapse across"?}
To make sense of this result, we analyze interaction log data to see which variables chart users condition on.
We find that aggbars users group the data by gene almost as often as 
% they group the data by 
treatment.
Compare this to filterbars users, who condition on treatment much more often than gene (see Supplemental Material).
This suggests that interacting with visualizations only improves sensitivity to causal support when users deliberately generate views of the data which show counterfactual predictions that can distinguish competing causal explanations. 
% This finding reassures us that causal support can help us understand how users struggle to use visualizations to evaluate causal hypotheses.
% \jessica{can remove this, but seems maybe we should note that this is expected/good: This observation is reassuring in that it suggests our model is capable of helping us understand where users are struggling to understand how to use a visualization to evaluate causal hypothesis.} 

\noindent
\textbf{Visual signal effects on sensitivity.} %\yifan{not sure how to fix but I was briefly confusing this statistical interaction with vis interactions.}
We examine sensitivity in each visualization as function of attributes of the visual signal for our task.
% We further investigate sensitivity to causal support by examining interactions between visualization conditions and attributes of the visual signal.
In Experiment 1, the signal breaks down into two data attributes, \textit{delta p} and \textit{sample size} (see Section 3.1.4). 
% \jessica{kind of seems like this should go earlier in stimuli generation and then just reference the explanations there}
% \textit{Delta p} describes the difference in the proportion of people with disease in each data set depending on whether they received treatment.
% Positive values of delta p indicate evidence that the treatment protects against disease; negative values of delta p indicate evidence against treatment effectiveness.
% \textit{Sample size} is the number of people in each data set we showed chart users.
% In a ideal observer \yifan{keep the terminology consistent with ``chart user''?},
Normatively, LLO slopes equal one regardless of delta p and sample size, however, our model measures differences in sensitivity depending on these data attributes.

Figure~\ref{fig:e1-interactions} shows that in the conditions where slopes are largest---text, icons, bars, aggbars without interaction, and filterbars with interaction---users are more sensitive to causal support at negative values of delta p (e.g., Fig.~\ref{fig:e1-interactions}, top inset). %\jessica{do we have a figure we can reference so people can see what this looks like?}
The average user in these conditions responds more to evidence against treatment (i.e., falsification) than evidence in favor of a treatment effect (i.e., verification). %\jessica{more compelling suggests they know what they're doing to me}
At positive values of delta p (e.g., Fig.~\ref{fig:e1-interactions}, top inset), LLO slopes are similar across conditions, suggesting that differences in performance between conditions are driven in part by differences in sensitivity to falsifying evidence.

We also see in Figure~\ref{fig:e1-interactions} that users of icons, bars, and aggbars especially are more sensitive to signal when sample size is smaller. 
% However, users of text and filterbars are more consistent in their sensitivity across levels of sample size.
This finding is consistent with prior work showing that chart users tend to underestimate sample size when making inferences with data~\cite{Kim2019}, which may be driven by logarithmic perception~\cite{Varshney2013,Zhang2012}.
Alternatively, we also could interpret this result as a cognitive bias where users are unwilling to be certain even when sample size is large enough to support unambiguous inferences, related to non-belief in the law of large numbers~\cite{Benjamin2016}.
Whatever the reason, we find it somewhat surprising that insensitivity to sample size persists even with icon arrays, which emphasize sample size as the overall number of equal-sized dots.

\noindent
\textbf{Bias.}
Intercepts in the LLO model describe bias in users' probability allocations when ground truth causal support indicates that explanation A (i.e., treatment effect) is just as likely as explanation B (i.e., no treatment effect). 
Under this condition, a normative observer would allocate equal probability to both causal explanations.
% \yifan{nit: just noticed that the use of probability allocation is a little inconsistent. you used belief allocation earlier, and vote allocation; I'm not sure what's the different between subjective probability allocation and ``user's probability allocation''}
We derive expected probability allocated to explanation A based on a logistic transform of LLO intercepts, and compare this to the normative benchmark of 50\%.

With all visualizations except for filterbars, probability allocations are far below 50\% indicating substantial bias (Fig.~\ref{fig:e1-intercepts}). 
On average when causal support is zero, users of text tables, icons, bars, and aggbars allocate too little probability to causal explanation A. %\jessica{can we make clear here whether A is causal or not causal?} 
Users of filterbars, on the other hand, allocate approximately 50\% to explanation A.
% , especially when they interact with the visualization.
We see the most extreme bias of up to 20\% with icons arrays.
% These biases help to account for the high absolute error in users' probability allocations, which is 31 percentage points on average.

Unfortunately, we can only speculate about possible reasons for these biases.
% , connecting them to key differences in the designs of these visualizations.
% Perhaps the especially large bias with icon arrays is related to frequency framing of proportions, such that something about discrete representations of outcomes makes users more cautious about believing in a treatment effect.
% Perhaps the lack of bias with  has to do with the non-tabular layout or the fact that data start aggregated rather than disaggregated by gene and treatment, such that expectations are better calibrated for some reason when users hunt for the signal in charts rather than seeing it in a detailed overview.
We expected that LLO intercepts would indicate average responses near 50\% in the absence of signal for all conditions (i.e., a uniform prior), simply because this follows from the structure of the task. 
Because this pattern of biases across visualizations results from a non-preregistered exploratory comparison, we investigate in Experiment 2 whether these biases replicate for a more complex task.

==> archived/submission/5_e2-method.tex <==
\section{Experiment 2}
In Experiment 2, we evaluate the same visualization designs on a more difficult task. 
We asked participants to detect confounding in the presence of a known treatment effect by allocating probability across four possible ``backdoor paths''~\cite{Pearl2018} (Fig.~\ref{fig:dags-e2-explainer}). %\jessica{have we explained backdoor path? if not cite something and put in ""}
We extend causal support to handle more than two alternative causal explanations,
% by eliciting a Dirichlet distribution (i.e., more than two probabilities that sum to one), 
demonstrating how causal support can be employed in more open-ended analyses.
% \jessica{can cut next sentence since its a little weird to explain resutls first} Experiment 2 replicates the core findings of Experiment 1, pointing to insensitivity to both sample size and verifying evidence as core challenges for causal inference that remain unsolved by common visual analytics tools.


\subsection{Method}
Experiment 2 was the same as Experiment 1 except for the following changes to response elicitation, modeling, and experimental design. %\yifan{s/these changes/changes described below? I thought you were referring to something that you had already described.} \jessica{agree a little confusing}

\subsubsection{Task scenario}
% Again, our participants played the role of an analyst hired by a company to interpret data sets on different treatments, genes, and diseases. \jessica{could omit prev sentence since you said its identical}
We asked participants to judge the influence of a gene on both disease and treatment effectiveness by allocating probability across the four DAGs in Figure~\ref{fig:dags-e2-explainer}.
Participants separately judge each component effect of a potential confounding relationship.

\noindent
\textbf{Question \& Elicitation.}
We asked participants the same question as in Experiment 1, where participants allocated 100 votes (i.e., subjective probability) across alternative causal explanations.
However, in Experiment 2 we elicited a Dirichlet distribution with four alternatives. %\yifan{The citation is just maths---would be great to have a citation that was cogsci study?} \alex{I looked and I could find no cogsci work on Dirichlets! I added the OHagen cite below. It is a more accessible description, but it's just a textbook that doesn't add much substance beyond the Chalone et al. paper.}
Following Chalone et al.~\cite{Chalone1987,OHagan2006} and extending our interface from Experiment 1, 
% we structured the elicitation so that 
each time participants allocated a number of votes between 0 and 100 to an option, the \textit{remaining votes out of 100 were uniformly distributed across unused response options}. 
These imputed responses were highlighted along with a prompt to, \textit{``Adjust your responses until all the numbers reflect your beliefs.''}
Participants iteratively set and adjusted their probability allocations. %\jessica{def need to make terms on this consistent}
We combined the four resulting probabilities into estimates of perceived causal support (i.e., log response ratios), which we compared to our normative benchmark. 
% \alex{I describe the elicitation procedure in terms of votes bc that's what we asked participants for. Although, I tried to make reiterate that votes are subjective probability.}

\noindent
\textbf{Payment.}
In Experiment 2, participants received a \$0.25 bonus for every trial where they responded within 5 percentage points of the ground truth probability of causal explanation D (Fig.~\ref{fig:dags-e2-explainer}).


\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/explainer-dag-04.png}
    % \setlength{\intextsep}{-20pt}
    \setlength{\abovecaptionskip}{-10pt}
    \setlength{\belowcaptionskip}{-20pt}
    \caption{DAGs for possible causal explanations in Experiment 2. %\yifan{would it make sense to join this figure with that of experiment 1's DAG? Also I think the stats folks like to call this a graphical model (rather than a DAG)?} \alex{I'd prefer not to combine these two figures since these are two different sets of explanations per experiment. I'm pretty sure combining them would be confusing, especially since the names `explanation A and B' refer to different DAGs in E1 and E2.}
    }
    \label{fig:dags-e2-explainer}
\end{figure}


\subsubsection{Modeling causal support}
We extend Griffiths and Tenenbaum's model of causal support~\cite{Griffiths2005} to accommodate more than two alternative causal explanations. 
We were interested primarily in causal support for causal explanation D, 
% \jessica{shoudl we say this earlier like briefly distinguish the four DAGs we presented beyond just saying backdoor paths?} 
\begingroup
\setlength\abovedisplayskip{3pt}
\setlength\belowdisplayskip{3pt}
    \begin{flalign*}
    \setlength\abovedisplayskip{0pt}
    \setlength\belowdisplayskip{0pt}
    \mathit{causal\_support_D} =& \log \bigg( \frac{\Pr(\mathit{model_D}|\mathit{data})}{\sum_{i=\{A,B,C\}}\Pr(\mathit{model_i}|\mathit{data})} \bigg) \\
    =& \log \bigg( \frac{\Pr(\mathit{data}|\mathit{model_D})}{\sum_{i=\{A,B,C\}}\Pr(\mathit{data}|\mathit{model_i})} \bigg) \\ 
    &+ \log \bigg( \frac{\Pr(\mathit{model_D})}{\sum_{i=\{A,B,C\}}\Pr(\mathit{model_i})} \bigg)
    \end{flalign*}
\endgroup
where $\mathit{data}$ is a data set, and models $\mathit{model_A}$, $\mathit{model_B}$, $\mathit{model_C}$, and $\mathit{model_D}$ correspond to causal explanations A through D, respectively.

Detecting confounding requires interpreting two distinct effects, the effect of gene on disease (Fig.~\ref{fig:dags-e2-explainer}, explanation B or D) and the effect of gene on treatment effectiveness (Fig.~\ref{fig:dags-e2-explainer}, explanation C or D).
% Note that in Figure~\ref{fig:dags-e2-explainer} the arrow from gene to disease was in explanations B and D, and the arrow from gene to treatment was in explanations C and D.
% Participants believe in these two distinct effects to the extent that they allocate probability to causal explanations B or D and C or D, respectively.
To study participants' sensitivity to each of these effects separately, we compared their responses to causal support for explanations B or D and causal support for explanations C or D, respectively\footnote{We define $\mathit{causal\_support_{BD}}$ and $\mathit{causal\_support_{CD}}$ similarly.}.
% and causal support for explanations C or D.
% \footnote{Causal support can be similarly defined for any subset of alternative causal explanations depending on what effects we want to operationalize belief in. \yifan{I don't understand what "operationalize belief" means. Also I think I understand why you have these subsets now. Maybe this footnote is unecessary}}.
\begingroup
\setlength\abovedisplayskip{3pt}
\setlength\belowdisplayskip{3pt}
    \begin{flalign*}
    \setlength\abovedisplayskip{0pt}
    \setlength\belowdisplayskip{0pt}
    causal\_support_{BD} =& \log \bigg( \frac{\sum_{i=\{B,D\}}\Pr(model_i|D)}{\sum_{i=\{A,C\}}\Pr(model_i|D)} \bigg) \\
    =& \log \bigg( \frac{\sum_{i=\{B,D\}}\Pr(D|model_i)}{\sum_{i=\{A,C\}}\Pr(D|model_i)} \bigg) \\ 
    &+ \log \bigg( \frac{\sum_{i=\{B,D\}}\Pr(model_i)}{\sum_{i=\{A,C\}}\Pr(model_i)} \bigg) 
    \end{flalign*}
\endgroup
% \begingroup
% \setlength\abovedisplayskip{3pt}
% \setlength\belowdisplayskip{3pt}
%     \begin{flalign*}
%     \setlength\abovedisplayskip{0pt}
%     \setlength\belowdisplayskip{0pt}
%     causal\_support_{CD} =& \log \bigg( \frac{\sum_{i=\{C,D\}}\Pr(model_i|D)}{\sum_{i=\{A,B\}}\Pr(model_i|D)} \bigg) \\
%     =& \log \bigg( \frac{\sum_{i=\{C,D\}}\Pr(D|model_i)}{\sum_{i=\{A,B\}}\Pr(D|model_i)} \bigg) \\ 
%     &+ \log \bigg( \frac{\sum_{i=\{C,D\}}\Pr(model_i)}{\sum_{i=\{A,B\}}\Pr(model_i)} \bigg)
%     \end{flalign*}
% \endgroup
% \yifan{maybe you can remove the second equation? I think it doesn't add much since I can figure out CD from DB?}
% \yifan{Format: if you are short on space, you can get rid of the alignment on the equal sign and merge the last row of the calculation}
% \yifan{Clarification: would it also be OK if I grouped AC and BD together? It's just a mathematical process right?}

To calculate likelihoods under each model $\Pr(\mathit{data}|\mathit{model_A})$, $\Pr(\mathit{data}|\mathit{model_B})$, $\Pr(\mathit{data}|\mathit{model_C})$, and $\Pr(\mathit{data}|\mathit{model_D})$, we used similar structural equations as in Experiment 1 (Fig.~\ref{fig:parameterization}), with modified formulae where people receive treatment and have the gene.
\begingroup
\setlength\abovedisplayskip{3pt}
\setlength\belowdisplayskip{3pt}
\begin{flalign*}
\setlength\abovedisplayskip{0pt}
\setlength\belowdisplayskip{0pt}
    \Pr(\mathit{Ds}|G, T) =& (\Pr(\mathit{Ds}|G) + \Pr(\mathit{Ds}) - \Pr(\mathit{Ds}|G) \cdot \Pr(\mathit{Ds})) \\
    &\cdot ((1 - \Pr(\neg \mathit{Ds}|T)) + \Pr(\neg \mathit{Ds}|T) \cdot \Pr(\neg T|G)) \\ 
    \Pr(\neg \mathit{Ds}|G, T) =& (\Pr(\mathit{Ds}|G) + \Pr(\mathit{Ds}) - \Pr(\mathit{Ds}|G) \cdot \Pr(\mathit{Ds})) \\
    &\cdot (\Pr(\neg \mathit{Ds}|T) \cdot (1 - \Pr(\neg T|G)) \\ 
    &+ (1 - \Pr(\mathit{Ds}|G)) \cdot (1 - \Pr(\mathit{Ds}))
\end{flalign*}
\endgroup
% \begingroup
% \setlength\abovedisplayskip{3pt}
% \setlength\belowdisplayskip{3pt}
% \begin{flalign*}
% \setlength\abovedisplayskip{0pt}
% \setlength\belowdisplayskip{0pt}
%     \Pr(\mathit{Ds}|G, T) =& (\textcolor{r}{\Pr(\mathit{Ds}|G)} + \textcolor{b}{\Pr(\mathit{Ds})} - \textcolor{r}{\Pr(\mathit{Ds}|G)} \cdot \textcolor{b}{\Pr(\mathit{Ds})}) \\
%     &\cdot ((1 - \textcolor{g}{\Pr(\neg \mathit{Ds}|T))} + \textcolor{g}{\Pr(\neg \mathit{Ds}|T)} \cdot \textcolor{p}{\Pr(\neg T|G)}) \\ 
%     \Pr(\neg \mathit{Ds}|G, T) =& (\textcolor{r}{\Pr(\mathit{Ds}|G)} + \textcolor{b}{\Pr(\mathit{Ds})} - \textcolor{r}{\Pr(\mathit{Ds}|G)} \cdot \textcolor{b}{\Pr(\mathit{Ds})}) \\
%     &\cdot (\textcolor{g}{\Pr(\neg \mathit{Ds}|T)} \cdot (1 - \textcolor{p}{\Pr(\neg T|G)}) \\ 
%     &+ (1 - \textcolor{r}{\Pr(\mathit{Ds}|G)}) \cdot (1 - \textcolor{b}{\Pr(\mathit{Ds})})
% \end{flalign*}
% \endgroup
% \yifan{nit: this D (for disease) collides with the previous D from the ABCD models; makes the notation slightly harder to parse.} \alex{This is definitely a problem.} \yifan{You can use a stylized font, like $\mathbb{ABCD}$ for the models?}
These models had four parameters: $\Pr(\mathit{Ds}|G)$ the probability of disease given that one has the gene; $\Pr(\mathit{Ds})$ the base rate of disease due to unexplained causes; $\Pr(\neg \mathit{Ds}|T)$ the probability that treatment prevents disease; and $\Pr(\neg T|G)$ the probability that the gene prevents treatment from working.
% These models had four parameters: $\textcolor{r}{\Pr(\mathit{Ds}|G)}$ the probability of disease given that one has the gene; $\textcolor{b}{\Pr(\mathit{Ds})}$ the base rate of disease due to unexplained causes; $\textcolor{g}{\Pr(\neg \mathit{Ds}|T)}$ the probability that treatment prevents disease; and $\textcolor{p}{\Pr(\neg T|G)}$ the probability that the gene prevents treatment from working.
As in Experiment 1, we estimated the log likelihood of each data set we showed participants under each model using Monte Carlo integration and sampling parameter values based on the assumptions of each model (see Section 3.1.3). 
Under $model_A$ we sampled $\Pr(\mathit{Ds})$ and $\Pr(\neg \mathit{Ds}|T)$ in our Monte Carlo simulation and fixed the gene effects $\Pr(\mathit{Ds}|G)$ and $\Pr(\neg T|G)$ at zero. 
Under $model_B$ we sampled $\Pr(\mathit{Ds})$, $\Pr(\mathit{Ds}|G)$, and $\Pr(\neg \mathit{Ds}|T)$ and fixed the gene effect on treatment $\Pr(\neg T|G)$ at zero. 
Under $model_C$ we sampled $\Pr(\mathit{Ds})$, $\Pr(\neg T|G)$, and $\Pr(\neg \mathit{Ds}|T)$ and fixed the gene effect on disease $\Pr(\mathit{Ds}|G)$ at zero.
% Under $model_A$ we sampled $\textcolor{b}{\Pr(\mathit{Ds})}$ and $\textcolor{g}{\Pr(\neg \mathit{Ds}|T)}$ in our Monte Carlo simulation and fixed the gene effects $\textcolor{r}{\Pr(\mathit{Ds}|G)}$ and $\textcolor{p}{\Pr(\neg T|G)}$ at zero. 
% Under $model_B$ we sampled $\textcolor{b}{\Pr(\mathit{Ds})}$, $\textcolor{r}{\Pr(\mathit{Ds}|G)}$, and $\textcolor{g}{\Pr(\neg \mathit{Ds}|T)}$ and fixed the gene effect on treatment $\textcolor{p}{\Pr(\neg T|G)}$ at zero. 
% Under $model_C$ we sampled $\textcolor{b}{\Pr(\mathit{Ds})}$, $\textcolor{p}{\Pr(\neg T|G)}$, and $\textcolor{g}{\Pr(\neg \mathit{Ds}|T)}$ and fixed the gene effect on disease $\textcolor{r}{\Pr(\mathit{Ds}|G)}$ at zero.
Under $model_D$ we sampled all four parameters to represent confounding.
% Simulating these causal explanations enabled us to calculate their compatibility with the data we showed participants.

We assume a uniform prior to create a benchmark for our task based on a Bayesian update.
% , as we did in Experiment 1.
Unlike in Experiment 1, however, the \textit{log prior ratio} ($\mathit{lpr_D}$) was non-zero when we calculated causal support.
\begingroup
\setlength\abovedisplayskip{3pt}
\setlength\belowdisplayskip{3pt}
    \begin{flalign*}
    \setlength\abovedisplayskip{0pt}
    \setlength\belowdisplayskip{0pt}
    \mathit{lpr_D} &= \log \bigg( \frac{\Pr(\mathit{model_D})}{\sum_{i=\{A,B,C\}}\Pr(\mathit{model_i})} \bigg) 
    = \log \bigg( \frac{0.25}{0.75} \bigg) = -1.099
    \end{flalign*}
\endgroup
This represents the assumption that $\Pr(\mathit{model_A}) = \Pr(\mathit{model_B}) = \Pr(\mathit{model_C}) = \Pr(\mathit{model_D}) = 0.25$, meaning that 25\% was the normative prior probability for each causal explanation.
% which means that 25\% was the normative probability allocation to explanation D in cases when the log likelihood ratio was zero.
For $\mathit{causal\_support_{BD}}$ and $\mathit{causal\_support_{CD}}$ on the other hand, $\mathit{lpr_{BD}} = \mathit{lpr_{CD}} = \mathrm{logit}(0.5) = 0$ such that the priors factored out of these expressions.
In each case, we assumed a uniform prior, but we combined these probabilities differently depending on what effect(s) we calculated causal support for.
% \yifan{I follow the direct calculations but not the implications. Is this why AB and CD have to be bundled together? Does the lpr has to be 0? What if the priors are somehow not uniformly distributed?} \jessica{agree this part is a little tricky to trace}

% These calculations extend the formalism of causal support, demonstrating how it can be applied to arbitrarily many alternative explanations that analysts might consider in real-world data analysis, and how causal support can be used to express different queries against analysts' beliefs as represented by their elicited Dirichlet distribution. 
% In principle, priors do not need to be uniform if, e.g., an analyst has \textit{a priori} knowledge of the data generating process. 
% Any application of causal support should incorporate priors as we demonstrate here, whether those priors are informed by domain knowledge or uninformed and uniform as they our in our study and in Griffiths and Tenenbaum~\cite{Griffiths2005}.


\subsubsection{Experimental design and stimuli}
We manipulated both the visualizations participants used for the task (between-subjects) and the data that we showed participants.
In Experiment 2, we generate stimuli that span a range of ground truth causal support for confounding.
We designed our stimuli to vary in three data attributes---delta p disease, delta p treatment, and sample size---which signaled whether gene was a confounding factor.
\textit{Delta p disease} described the difference in the proportion of people with disease in each data set depending on whether they had the gene.
Negative values of delta p disease indicated evidence that the gene caused disease, whereas values near zero indicated evidence against a gene effect on disease.
\textit{Delta p treatment} described the difference in the proportion of people with disease within the treatment group depending on whether they had the gene.
Negative values of delta p treatment indicated evidence that the gene stopped the treatment from preventing disease, whereas values near zero indicated evidence against a gene effect on treatment.
\textit{Sample size} was the number of people in each data set we showed chart users.

% Each participant in Experiment 2 judged 18 data sets with a visualization condition randomly assigned between-subjects.

We showed 18 data conditions generated from unique combinations of three factors: \textit{probability that gene causes disease} (3 levels: $\{0, 0.35, 0.7\}$), \textit{probability that gene prevents treatment from working} (3 levels: $\{0, 0.35, 0.7\}$), and \textit{sample size} (2 levels: $\{100, 1000\}$).
% We generated the data conditions shown on each trial from unique combinations of three factors: \textit{probability that the gene causes disease} (3 levels: $\{0, 0.35, 0.7\}$), \textit{probability that the gene prevents treatment from working} (3 levels: $\{0, 0.35, 0.7\}$), and \textit{sample size} (2 levels: $\{100, 1000\}$).
As in Experiment 1, we simulated many data sets for each data condition, and we counterbalanced quantiles of sampling error across participants (see Section 3.1.4).
These within-subjects manipulations result in 18 sets of realistic-looking count data per participant.
% These within-subjects manipulations result in fake data sets that show evidence spanning a range of ground truth causal support for confounding.

We showed participants one attention check trial, chosen to maximize causal support for confounding. We presented this attention check on the 10th of 19 total trials and used it for our exclusion criterion.


\subsubsection{Performance evaluation}
Again, we used linear in log odds (LLO) models~\cite{Gonzalez1999,Zhang2012} to describe discrepancies between perceived and normative causal support.

\noindent
\textbf{Perceived causal support.}
We estimated \textit{perceived causal support} by transforming participants' probability allocations into log response ratios representing belief in confounding ($\mathit{lrr_D}$), and the component effects of a confounding relationship---the gene effects on disease ($\mathit{llr_{BD}}$) and treatment effectiveness ($\mathit{llr_{CD}}$), respectively\footnote{We define $\mathit{llr_{BD}}$ and $\mathit{llr_{CD}}$ similarly.},
\begingroup
\setlength\abovedisplayskip{3pt}
\setlength\belowdisplayskip{3pt}
    \begin{flalign*}
    \setlength\abovedisplayskip{0pt}
    \setlength\belowdisplayskip{0pt}
    \mathit{lrr_D} &= \log \bigg( \frac{\mathit{response_D}}{\sum_{i=\{A,B,C\}}\mathit{response_i}} \bigg) \\
    \mathit{lrr_{BD}} &= \log \bigg( \frac{\sum_{i=\{B,D\}}\mathit{response_i}}{\sum_{i=\{A,C\}}\mathit{response_i}} \bigg) %\\
    % lrr_{CD} &= \log \bigg( \frac{\sum_{i=\{C,D\}}response_i / 100}{\sum_{i=\{A,B\}}response_i / 100} \bigg)
    \end{flalign*}
\endgroup
where $\mathit{response_A}$, $\mathit{response_B}$, $\mathit{response_C}$, and $\mathit{response_D}$ were participants' probability allocations to causal explanations A through D, respectively, on each trial.
We primarily compared perceived causal support for confounding ($\mathit{lrr_D}$) to normative causal support for confounding ($\mathit{causal\_support_D}$).
However, we also separately examined participants' sensitivity both of the distinct effects that constitute a confounding relationship  (Fig.~\ref{fig:dags-e2-explainer}, the highlighted arrows in the DAGs) by comparing $\mathit{lrr_{BD}}$ to $\mathit{causal\_support_{BD}}$ and $\mathit{lrr_{CD}}$ to $\mathit{causal\_support_{CD}}$.


\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/e2-interactions_final.png}
    \setlength{\abovecaptionskip}{-10pt}
    \setlength{\belowcaptionskip}{-17pt}
    \caption{Sensitivity (y-axes) conditioned on three attributes of visual signal for confounding (rows, x-axes) and visualization conditions (columns).
    % \yifan{I'm not sure how the visualization is intended to work with the rows of small multiples here. I searched the text and didn't find an explanation, so I would benefit from a different description (other than a repeat of the chart title). Also prob should move this up the page.}
    }
    \label{fig:e2-interactions}
\end{figure*}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/e2-main-effects_slopes.png}
    \setlength{\abovecaptionskip}{-10pt}
    \setlength{\belowcaptionskip}{-17pt}
    \caption{Linear in log odds (LLO) slopes per visualization condition.
    }
    \label{fig:e2-slopes}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/e2-main-effects_intercepts.png}
    \setlength{\abovecaptionskip}{-10pt}
    \setlength{\belowcaptionskip}{-17pt}
    \caption{LLO intercepts per visualization condition.
    }
    \label{fig:e2-intercepts}
\end{figure}


\noindent
\textbf{Model specification.}
We needed three inferential models because we had three dependent variables, representing perceived causal support for confounding ($\mathit{lrr_D}$) and perceived causal support for the two constituent effects of confounding ($\mathit{lrr_{BD}}$ and $\mathit{lrr_{CD}}$).
Here, we show only the models on $\mathit{lrr_D}$ and  $\mathit{lrr_{BD}}$ because the models on $\mathit{lrr_{CD}}$ and $\mathit{lrr_{BD}}$ are identical in form, with $\mathit{causal\_support_{CD}}$ and $\mathit{delta\_p\_t}$ replacing $\mathit{causal\_support_{BD}}$ and $\mathit{delta\_p\_d}$ as predictors:
% We used these models\footnote{The models on $\mathit{lrr_{CD}}$ and $\mathit{lrr_{BD}}$ are identical in form, with $\mathit{causal\_support_{CD}}$ and $\mathit{delta\_p\_t}$ replacing $\mathit{causal\_support_{BD}}$ and $\mathit{delta\_p\_d}$ as predictors.}:
% a primary model on causal support for confounding and two secondary models examining causal support for the gene effect on disease and treatment effectiveness, respectively: 
% \yifan{Clarify: I don't understand why three models are needed, instead just the primary model.} \jessica{same here, it feels liek there are steps missing in the explanation that will be very hard for readers to figure out themeselves}
\begingroup
\setlength\abovedisplayskip{3pt}
\setlength\belowdisplayskip{3pt}
    \begin{flalign*}
    \setlength\abovedisplayskip{0pt}
    \setlength\belowdisplayskip{0pt}
    \mathit{lrr_D} \sim &\mathrm{Normal}(\mu_D, \sigma_D) \\[-2pt]
    \mu_D = &\mathit{causal\_support_D}*\mathit{delta\_p\_d}*\mathit{delta\_p\_t}*n*\mathit{vis} \\[-2pt]
    &+ \big(\mathit{causal\_support_D}*\mathit{delta\_p\_d} %\\[-2pt]
    + \mathit{causal\_support_D}*\mathit{delta\_p\_t} \\[-2pt]
    &+ \mathit{causal\_support_D}*n\big|\mathit{worker\_i}d\big) \\
    \mathit{lrr_{BD}} \sim &\mathrm{Normal}(\mathit{\mu_{BD}}, \mathit{\sigma_{BD}}) \\[-2pt]
    \mathit{\mu_{BD}} = &\mathit{causal\_support_{BD}}*\mathit{delta\_p\_d}*n*\mathit{vis} \\[-2pt]
    &+ \big(\mathit{causal\_support_{BD}}\big|\mathit{worker\_id}\big) %\\
    % lrr_{CD} \sim &\mathrm{Normal}(\mu_{CD}, \sigma_{CD}) \\[-2pt]
    % \mu_{CD} = &causal\_support_{CD}*delta\_p\_t*n*vis \\[-2pt]
    % &+ \big(causal\_support_{CD}\big|worker\_id\big)
    \end{flalign*}
\endgroup
% \yifan{Clarification: I'm not following why you are grouping CD and AB together at this current stage. Is there no $causal\_support_{A}$ just by itself?}
where $\mathit{lrr_D}$, $\mathit{lrr_{BD}}$, and $\mathit{lrr_{CD}}$ were perceived causal support for a confounding, the gene effect on disease, and the gene effect on treatment, respectively, $\mathit{causal\_support_D}$, $\mathit{causal\_support_{BD}}$, and $\mathit{causal\_support_{CD}}$ were our normative benchmarks corresponding to each log response ratio, $\mathit{delta\_p\_d}$ was the difference in the proportion of people with disease given gene versus no gene, $\mathit{delta\_p\_t}$ was the difference in the proportion of people with disease among those in the treatment group given gene versus no gene, $n$ was the sample size as a factor, $\mathit{vis}$ was a dummy variable for visualization condition, and $\mathit{worker\_id}$ was a unique identifier for each participant.

We primarily modeled effects on mean perceived causal support $\mu_D$, $\mathit{\mu_{BD}}$, and $\mathit{\mu_{CD}}$, but our models also learned residual standard deviations of perceived causal support $\sigma_D$, $\mathit{\sigma_{BD}}$, and $\mathit{\sigma_{CD}}$.
These residual standard deviations and the random effects in each model helped us separate patterns in responses from noise and individual differences.
In the first model, we used the term $\mathit{causal\_support_D}*\mathit{delta\_p\_d}*\mathit{delta\_p\_t}*n*\mathit{vis}$ to learn how sensitivity to causal support for confounding varies as a function of sample size $n$ and visualization condition $\mathit{vis}$. 
In the second and third models, we used the terms $\mathit{causal\_support_{BD}}*\mathit{delta\_p\_d}*n*\mathit{vis}$ and $\mathit{causal\_support_{CD}}*\mathit{delta\_p\_t}*n*\mathit{vis}$ to learn how sensitive users in each visualization condition were to the visual signal for the gene effects on disease $\mathit{delta\_p\_d}$ and treatment $\mathit{delta\_p\_t}$, respectively.


\subsubsection{Participants}
% We recruited participants on Amazon Mechanical Turk using the same qualifications as in Experiment 1.
We used a similar approach to power analysis as in Experiment 1 to determine a target sample size of of 500 participants after exclusions.
We recruited a total of 703 participants, and after exclusions we used data from 519 participants in our analysis. 
% Again, we slightly overshot our target sample size because we ran data collection in batches of participants, and we could not anticipate perfectly how many we would exclude. \yifan{Squeeze: prev sentence could go if short for space.} \jessica{agree}
Although we preregistered that we would exclude participants who allocated less than 25\% probability to confounding on an attention check trial where confounding was very likely (see Section 4.1.3), this criterion would have excluded 39\% of our sample.
We relaxed the cutoff to less than 20\% probability of confounding to allow for additional response error, resulting in a 26\% exclusion rate.
% \yifan{Exp 1's attention check was within 5\% of the target range?} This resulted in an exclusion rate of 26\% similar to Experiment 1.
% All participants were paid regardless of exclusions.
We paid participants \$3.04 for 14 minutes on average.

==> archived/submission/6_e2-results.tex <==



\subsection{Results}
We use a linear in log odds (LLO) model to describe performance in terms of \textit{sensitivity} to ground truth causal support and \textit{bias} in probability allocations when all four causal explanations are equally likely.

\noindent
\textbf{Sensitivity.} 
A LLO slope of one indicates ideal sensitivity to the log likelihood of the data given a set of causal explanations
% that users' probability allocations change in one-to-one correspondence with the log likelihood of the data given a set of causal explanations.
Similar to Experiment 1, slopes in all visualization conditions are closer to zero than one (Fig.~\ref{fig:e2-slopes}), indicating under-sensitivity to the ground truth.

Interacting with filterbars seems to improve sensitivity, while interacting with aggbars seems to decrease sensitivity, although these differences are not reliable.
It is somewhat surprising to see a similar pattern of results for interactive visualizations in both experiments.
We expected that interactive visualizations might be more helpful for detecting confounding (Experiment 2) than for detecting a treatment effect (Experiment 1).
The confounding detection task requires users to look for more complex counterfactual patterns in order to distinguish between competing causal explanations, and the ability to manipulate data aggregation and filtering should enable users to query visualizations for these patterns.
% We expected that interactive visualizations might be more helpful for detecting confounding (Experiment 2) than for detecting a treatment effect (Experiment 1) because manipulating data aggregation and filtering might reveal or reify counterfactual patterns. \jessica{prev sentence not completely clear}
When we analyze interaction logs (see Supplemental Materials), we see that filterbars users interacted with the visualizations more frequently and created more task-relevant views of the data than aggbars users, which may help to explain why interacting with filterbars was somewhat more helpful than interacting with aggbars.

\noindent
\textbf{Visual signal effects on sensitivity.}
We examine sensitivity in each visualization condition to the three visual signals for confounding in our task (delta p disease, delta p treatment, and sample size; see Section 4.1.3).
% For Experiment 2, the signal breaks down into three components: delta p disease, delta p treatment, and sample size (see Section 4.1.3). \yifan{not sure what the prev sentence is adding in this context. seems fine without?}
% \textit{Delta p disease} describes the difference in the proportion of people with disease in each data set depending on whether they have the gene.
% Negative values of delta p disease indicate evidence that the gene causes disease, whereas values near zero indicate evidence against a gene effect on disease.
% \textit{Delta p treatment} describes the difference in the proportion of people with disease within the treatment group depending on whether they have the gene.
% Negative values of delta p treatment indicate evidence that the gene stop the treatment from preventing disease, whereas values near zero indicate evidence against a gene effect on treatment.
% \textit{Sample size} is the number of people in each data set we showed chart users.
Normatively, slopes are one regardless of these visual signals.

Figure~\ref{fig:e2-interactions} shows users are more sensitive to causal support at values of delta p disease and delta p treatment near zero, with the exception of filterbars users who don't interact.
This pattern is consistent with the findings of Experiment 1 in that chart users respond more to evidence against a given causal effect than evidence in favor of an effect.

In Figure~\ref{fig:e2-interactions}, we also see that users of every visualization but filterbars are more sensitive when sample size is smaller. 
This pattern is consistent with prior work~\cite{Benjamin2016,Kim2019} and the results of Experiment 1.
%as well as prior work showing that people tend to underestimate sample size and underweight evidence from large samples in Bayesian update~\cite{Benjamin2016} including when making estimates from visualizations~\cite{Kim2019}.

\noindent
\textbf{Bias.}
LLO intercepts describe bias in probability allocations when the data are equally likely under each alternative causal explanation.
We derive expected probability allocated to explanation D based on LLO intercepts and compare this to the normative benchmark of 25\%.

Figure~\ref{fig:e2-intercepts} shows that, with all visualizations but text tables, users underestimate the probability of confounding in the absence of signal.
The fact that biases for each visualization condition differ between Experiments 1 and 2 suggests that these results are task-specific.
Future work should study reasons for these biases and what visual analytics software can do to help calibrate analysts' probability allocations. 
% \yifan{made a jump between biases and priors, prob just keep bias discussion or elaborate a bit more.}

==> archived/submission/7_discussion.tex <==
\section{Discussion}
We demonstrate the utility of causal support for studying inferences with visualizations.
% , and we learn about ways that users struggle to make causal inferences with common visualizations of count data.
Our evaluation approach successfully measures some expected patterns in the quality of chart users' causal inferences.
For example, filterbars users should not have been able to perform either task without interacting because the visual signals required to perform the tasks were hidden behind interactions.
Our method shows that filterbars users were completely insensitive to the signal in data when they did not interact with the visualizations.
Similarly, our models corroborate findings from prior work suggesting that chart users underweight sample size when making inferences~\cite{Benjamin2016,Kim2019}.
Findings like these reassure us that causal support can help us understand how users struggle to use visualizations to evaluate causal hypotheses.
% \yifan{perhaps a nod to the intro's \emph{"study the utility of causalsupport and (2) evaluate how well visualization and interaction designscommon in visual analytics software support causal inferences"} here as opposed to directly jumping to the evaluation itself?}
% \jessica{Also maybe establish we think causal support was useful here (ie we saw some expected directions of effects? not sure), before saying things that assume it worked}

Our findings point to unsolved design challenges for supporting causal inferences with visual analytics (VA) tools.
Contrary to what we might expect given the emphasis of visualization research on evaluating encodings and interaction techniques, using different encodings for count data doesn’t appear to improve sensitivity to evidence for causal inferences beyond text contingency tables.
Similarly, common interaction techniques in VA tools, such as manipulating data aggregation or cross-filtering coordinated multiple views, don’t seem to improve causal inferences beyond what users can achieve with simpler static visualizations.
% \yifan{nit: "help that much" colloquial.} \jessica{help bring analysts inferences closer to causal support?}
Interacting with visualizations seems to help or hurt sensitivity depending on how deliberately signal-seeking users are and whether interacting is necessary in order to expose the visual signal in the data. 
This suggests that VA tools designed to optimize easy exposure of data are not sufficient for supporting causal inferences. 
% \yifan{Clarify: what is data exposure? avoid novel nouns?}

We also find systematic biases in the way that chart users respond to specific visual signals in charts.
\textit{Chart users seem ubiquitously more sensitive to falsifying evidence than they are to verifying evidence}.
This may reflect a cognitive bias where analysts are more responsive to \textit{discrepancies}, between observed data and the counterfactual patterns expected under a given causal explanation, than they are to \textit{similarities} between observed data and counterfactual patterns.
% \yifan{prev sentence hard to follow}
Interestingly, this bias may be somewhat rational to the extent that verifying an inference
% the logic of verification \jessica{could we say, 'verifying an inference' to be clearer?} 
is probabilistic, whereas the logic of falsification is deductive and thus ``more powerful'' in that it can definitively rule out an explanation~\cite{Popper1959}. 

\textit{Insensitivity to sample size remains a major challenge for informal statistical inferences}, and it appears not to be sufficiently addressed by common chart types for showing count data.
Even icon arrays, which emphasize sample size as the number of equal-sized dots, don't seem to mitigate this problem.
As suggested by prior work~\cite{Benjamin2016,Kim2019}, this may be due to a combination of perceptual underestimation of sample size and cognitive bias against claiming certainty in inferences.

Consistent with an aversion to believing causal relationships exist, we find that chart users tend to underestimate the probability of a given arrow in a DAG. 
Specifically, in the absence of any signal for differentiating between causal explanations, chart users allocate more probability to explanations that posit fewer causal relationships, rather than allocating probability uniformly across alternatives.
Though this tendency interacts with task and visualization format in ways that warrant further study, it may reflect an overall cognitive bias toward believing in simpler causal explanations with fewer assumptions.
% \yifan{you can prob get some cogsci citations to back up this hypothesis}

\subsection{Limitations}
The primary limitation of this work is that we recruited participants on Mechanical Turk, who may differ from the user population for VA tools.
Real data analysts may be more sensitive to causal support than crowdworkers to the extent that they may use VA tools more deliberately, though we suspect the overall patterns of biases that we find will persist in some form across user populations and causal inference tasks.
We set out to run a proof-of-concept study establishing causal support as an evaluation method for VA tools.
To the extent that real data analysts give less noisy responses than crowdworkers, the evaluation approach we demonstrate should be helpful in evaluating current practices or novel interfaces with smaller pools of participants.


\subsection{Improving visual analytics for causal inference}
A theme in visual causal inference is that analysts do not always know what to look for in the data~\cite{Batanero1996,Yen2019}.
Causal inferences differentiating between possible data generating processes (DGPs) rely on comparisons between the patterns in observed data and counterfactual patterns that should only manifest under a specific DGP~\cite{Greenland1999,Pearl2018}. %\yifan{add citation}
Users of visual analytics software may find causal inferences very challenging insofar as they fail to \textit{imagine} counterfactual predictions from alternative DGPs.

Prior work in statistics and visualization argues for \textit{model checks} that make comparisons between data and model predictions explicit~\cite{gelman2003,gelman2004exploratory,hullman2020theories}.
For example, workflows in Bayesian statistics frequently employ prior and posterior predictive checks~\cite{Gabry2019}.%, where analysts pass draws from a prior or posterior distribution through a model in order to generate counterfactual predictions.
Visualizing model predictions alongside 
% the empirical distribution of the 
empirical data could support causal inference by externalizing discrepancies and similarities between observed and expected patterns.
% Such model checks may 
% improve performance on causal inference tasks
% support causal inferences insofar as they externalize the required comparisons, expressing information that is otherwise only in the imagination of the analyst.

We envision a workflow for VA software where analysts cycle between to interactively specifying models (e.g.,~\cite{Kraska2018}) and generating model checks to gauge model compatibility with their data. 
This echos calls to make models themselves a primary goal of visual data analysis~\cite{Andrienko2018}.
Causal support solves an important problem in realizing this vision, defining a ``good'' model check as one which support sensitive inferences among a set of candidate data generating models. 
Though it may be difficult to come up with an exhaustive set of models for many real world applications, we think that this approach would be fruitful even with a relatively simple set of models that a knowledgeable analyst might provisionally entertain.
Causal support cannot guard against an analyst ignoring possible models, but it can be used to evaluate visualization and interaction designs intended to help analyst collate and compare alternative models.

% Future work should investigate how to construct these visual model checks to support greater sensitivity to the signal in charts and how to incorporate them into VA software.
% The present study suggests a path toward realizing these goals.
% We demonstrate how causal support can be used to operationalize the signal in a chart for the purpose of making causal inferences.
% Our approach to operationalizing the signal in charts for causal inferences requires a set of possible data generating models.
% Though it may be difficult to come up with an exhaustive set of models for many real world applications, we think that this approach would be fruitful even with a relatively simple set of models that a knowledgeable analyst might provisionally entertain.
% Although causal support cannot guard against an analyst ignoring possible models, it can be used to evaluate visualization and interaction designs intended to support targeted counterfactual comparisons.

% \jessica{I think you can shorten this, the Northstar reference eg seems a little too much to introduce at the end of discussion:} 
% Many challenges of integrating model checks into VA systems revolve around how to extend existing workflows to support user interactions with statistical models.
% For example, Northstar~\cite{Kraska2018}, a proof-of-concept in this design space, uses machine learning models to provide automated assistance for inferences in VA.
% Among its many features, Northstar provides interaction techniques for subsetting the data to make models aware of distinctions that seem important to the analyst.
% We envision a future where widely-used VA software affords iteration between interactive model construction (e.g.,~\cite{Kraska2018}) and model checks, making models themselves a primary goal of visual data analysis~\cite{Andrienko2018}.
% Within model-based VA systems, causal support could serve as a basis for mixed-initiative tools that help users collate and compare alternative models.


\section{Conclusion}
We contribute two crowdsourced experiments demonstrating an approach to evaluating causal inferences with visual analytics (VA) tools.
No visualization or interaction designs we tested lead to reliably better causal inferences than text contingency tables, suggesting that common VA tools designed for data exposure may not be sufficient for supporting causal inferences.
We point to perceptual and cognitive biases which seem to make causal inferences difficult for chart users, including the tendencies to underweight both evidence verifying a causal relationship and evidence from large samples.
We discuss how formal models of causal support, such as the ones we demonstrate in our study, can be used to evaluate VA systems that place an emphasis on helping users reason about possible data generating processes.

==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)

